Towards Refining Developer Questions using LLM-Based Named Entity Recognition for Developer Chatroom Conversations

In software engineering chatrooms, communication is often hindered by imprecise questions that cannot be answered. Recognizing key entities can be essential for improving question clarity and facilitating better exchange. However, existing research using natural language processing techniques often overlooks these software-specific nuances. In this paper, we introduce Software-specific Named Entity Recognition, Intent Detection, and Resolution Classification (SENIR), a labeling approach that leverages a Large Language Model to annotate entities, intents, and resolution status in developer chatroom conversations. To offer quantitative guidance for improving question clarity and resolvability, we build a resolution prediction model that leverages SENIR's entity and intent labels along with additional predictive features. We evaluate SENIR on the DISCO dataset using a subset of annotated chatroom dialogues. SENIR achieves an 86% F-score for entity recognition, a 71% F-score for intent detection, and an 89% F-score for resolution status classification. Furthermore, our resolution prediction model, tested with various sampling strategies (random undersampling and oversampling with SMOTE) and evaluation methods (5-fold cross-validation, 10-fold cross-validation, and bootstrapping), demonstrates AUC values ranging from 0.7 to 0.8. Key factors influencing resolution include positive sentiment and entities such as Programming Language and User Variable across multiple intents, while diagnostic entities are more relevant in error-related questions. Moreover, resolution rates vary significantly by intent: questions about API Usage and API Change achieve higher resolution rates, whereas Discrepancy and Review have lower resolution rates. A Chi-Square analysis confirms the statistical significance of these differences.

==> tablets/best_worst_combinations.tex <==

\begin{table}
\centering
\begin{tabular}{llllllll}
Entities Combination                        & Success Rate & Number of Successful Combinations & Total Number of Combinations & Max Entities & Min Entities & Median Entities & Average Entities  \\
VERSION, LIBRARY\_CLASS                     & 70           & 7                                 & 10                           & 24           & 7            & 11              & 12.6              \\
VERSION, FILE\_TYPE                         & 65           & 13                                & 20                           & 24           & 2            & 7.5             & 8.85              \\
VERSION, DEVICE                             & 64.28571429  & 9                                 & 14                           & 24           & 4            & 8               & 10.07142857       \\
VERSION, FILE\_NAME                         & 60.71428571  & 17                                & 28                           & 24           & 3            & 7               & 8.142857143       \\
LIBRARY, LIBRARY\_VARIABLE                  & 60           & 6                                 & 10                           & 19           & 7            & 8.5             & 10.4              \\
APPLICATION, LIBRARY\_FUNCTION              & 59.09090909  & 13                                & 22                           & 11           & 3            & 7               & 6.954545455       \\
LIBRARY\_CLASS, FILE\_TYPE                  & 55.55555556  & 10                                & 18                           & 24           & 6            & 9.5             & 10.33333333       \\
USER\_NAME, LIBRARY\_FUNCTION               & 54.54545455  & 6                                 & 11                           & 11           & 3            & 7               & 6.727272727       \\
APPLICATION, VALUE                          & 54.16666667  & 13                                & 24                           & 24           & 3            & 7               & 7.166666667       \\
DEVICE, LIBRARY\_FUNCTION                   & 53.84615385  & 7                                 & 13                           & 19           & 4            & 6               & 7.384615385       \\
LIBRARY\_CLASS, FILE\_NAME                  & 53.33333333  & 8                                 & 15                           & 24           & 6            & 10              & 10.6              \\
ERROR\_NAME, DATA\_TYPE                     & 52.38095238  & 11                                & 21                           & 24           & 2            & 8               & 8.476190476       \\
OPERATION\_SYSTEM, DEVICE                   & 50           & 10                                & 20                           & 24           & 3            & 5               & 8.15              \\
USER\_NAME, IN\_LINE\_CODE                  & 50           & 7                                 & 14                           & 24           & 2            & 4.5             & 5.928571429       \\
DATA\_TYPE, FILE\_NAME                      & 50           & 12                                & 24                           & 24           & 3            & 8.5             & 8.666666667       \\
LIBRARY\_CLASS, USER\_FUNCTION\_NAME        & 50           & 5                                 & 10                           & 24           & 7            & 10              & 11.4              \\
FILE\_TYPE, KEYBOARD\_INPUT                 & 50           & 6                                 & 12                           & 24           & 4            & 9.5             & 9.583333333       \\
APPLICATION, LIBRARY                        & 49.05660377  & 26                                & 53                           & 24           & 2            & 5               & 5.509433962       \\
ERROR\_NAME, FILE\_TYPE                     & 48.14814815  & 13                                & 27                           & 24           & 4            & 7               & 8.185185185       \\
APPLICATION, IN\_LINE\_CODE                 & 47.05882353  & 8                                 & 17                           & 24           & 4            & 7               & 7.352941176       \\
ERROR\_NAME, VALUE                          & 47.05882353  & 16                                & 34                           & 24           & 2            & 5.5             & 7.088235294       \\
USER\_NAME, VALUE                           & 47.05882353  & 8                                 & 17                           & 24           & 2            & 5               & 6.176470588       \\
PROGRAMMING\_LANGUAGE, LIBRARY\_VARIABLE    & 46.66666667  & 7                                 & 15                           & 19           & 2            & 8               & 8.4               \\
ALGORITHM, IN\_LINE\_CODE                   & 45.45454545  & 5                                 & 11                           & 24           & 2            & 7               & 9                 \\
USER\_NAME, DATA\_TYPE                      & 45.45454545  & 5                                 & 11                           & 24           & 4            & 5               & 7.181818182       \\
OPERATION\_SYSTEM, FILE\_TYPE               & 45           & 9                                 & 20                           & 24           & 2            & 5               & 7.15              \\
OPERATION\_SYSTEM, IN\_LINE\_CODE           & 44.44444444  & 8                                 & 18                           & 24           & 2            & 6               & 8.555555556       \\
ERROR\_NAME, DATA\_STRUCTURE                & 44           & 11                                & 25                           & 24           & 4            & 7               & 8.64              \\
DATA\_STRUCTURE, FILE\_NAME                 & 43.75        & 14                                & 32                           & 24           & 3            & 8               & 8.25              \\
APPLICATION, ERROR\_NAME                    & 42.85714286  & 6                                 & 14                           & 24           & 2            & 4               & 6.357142857       \\
DEVICE, DATA\_TYPE                          & 42.85714286  & 6                                 & 14                           & 24           & 4            & 7.5             & 9.571428571       \\
DATA\_TYPE, IN\_LINE\_CODE                  & 42.85714286  & 15                                & 35                           & 24           & 3            & 6               & 7.485714286       \\
LIBRARY\_CLASS, VALUE                       & 42.85714286  & 6                                 & 14                           & 24           & 5            & 9               & 11                \\
LIBRARY\_FUNCTION, VALUE                    & 42.85714286  & 27                                & 63                           & 19           & 3            & 7               & 6.825396825       \\
DATA\_TYPE, LIBRARY\_FUNCTION               & 42.1875      & 27                                & 64                           & 19           & 3            & 7               & 7.09375           \\
VERSION, OPERATION\_SYSTEM                  & 42.10526316  & 8                                 & 19                           & 24           & 2            & 5               & 8.052631579       \\
LIBRARY\_FUNCTION, FILE\_TYPE               & 41.81818182  & 23                                & 55                           & 14           & 4            & 7               & 7.745454545       \\
ALGORITHM, OPERATION\_SYSTEM                & 41.66666667  & 5                                 & 12                           & 24           & 3            & 5               & 8.5               \\
ALGORITHM, DATA\_TYPE                       & 41.66666667  & 10                                & 24                           & 24           & 2            & 5               & 6.791666667       \\
DEVICE, USER\_FUNCTION\_NAME                & 41.66666667  & 5                                 & 12                           & 24           & 4            & 7               & 9.166666667       \\
FILE\_NAME, KEYBOARD\_INPUT                 & 41.66666667  & 5                                 & 12                           & 24           & 3            & 9.5             & 9.333333333       \\
DATA\_STRUCTURE, VALUE                      & 41.46341463  & 17                                & 41                           & 24           & 2            & 7               & 7.487804878       \\
FILE\_TYPE, FILE\_NAME                      & 41.25        & 33                                & 80                           & 24           & 2            & 7               & 7.05              \\
LIBRARY\_VARIABLE                           & 41.17647059  & 7                                 & 17                           & 19           & 2            & 8               & 7.882352941       \\
HTML\_TAG\_NAME                             & 41.17647059  & 7                                 & 17                           & 24           & 1            & 5               & 6.941176471       \\
OPERATION\_SYSTEM, DATA\_STRUCTURE          & 41.17647059  & 7                                 & 17                           & 24           & 3            & 6               & 8                 \\
USER\_NAME, LIBRARY                         & 41.17647059  & 7                                 & 17                           & 24           & 3            & 6               & 6.705882353       \\
USER\_NAME, DATA\_STRUCTURE                 & 40.90909091  & 9                                 & 22                           & 24           & 2            & 5               & 5.863636364       \\
PROGRAMMING\_LANGUAGE, DATA\_STRUCTURE      & 40.85365854  & 134                               & 328                          & 24           & 2            & 4               & 4.649390244       \\
PROGRAMMING\_LANGUAGE, ERROR\_NAME          & 40.81632653  & 40                                & 98                           & 24           & 2            & 5               & 5.734693878       \\
LIBRARY\_FUNCTION                           & 40.75630252  & 97                                & 238                          & 19           & 1            & 5               & 5.676470588       \\
VERSION, LIBRARY\_FUNCTION                  & 40.74074074  & 11                                & 27                           & 19           & 3            & 7               & 7.777777778       \\
DATA\_STRUCTURE, LIBRARY\_FUNCTION          & 40.22988506  & 35                                & 87                           & 19           & 3            & 6               & 6.747126437       \\
APPLICATION, VERSION                        & 40           & 12                                & 30                           & 24           & 2            & 5               & 6.2               \\
VERSION, LIBRARY                            & 40           & 20                                & 50                           & 24           & 2            & 5.5             & 6.8               \\
VERSION, VALUE                              & 40           & 6                                 & 15                           & 24           & 3            & 9               & 10.33333333       \\
ERROR\_NAME, USER\_VARIABLE                 & 40           & 18                                & 45                           & 24           & 2            & 6               & 7.266666667       \\
LIBRARY, UI\_ELEMENT                        & 40           & 4                                 & 10                           & 24           & 3            & 8.5             & 10.2              \\
LIBRARY\_FUNCTION, FILE\_NAME               & 40           & 18                                & 45                           & 14           & 4            & 8               & 7.977777778       \\
FILE\_TYPE, UI\_ELEMENT                     & 40           & 4                                 & 10                           & 24           & 4            & 9               & 10                \\
DATA\_STRUCTURE, DATA\_TYPE                 & 39.79591837  & 39                                & 98                           & 24           & 2            & 6               & 6.081632653       \\
PROGRAMMING\_LANGUAGE, LIBRARY\_FUNCTION    & 39.71962617  & 85                                & 214                          & 19           & 2            & 6               & 5.822429907       \\
LIBRARY, VALUE                              & 39.65517241  & 23                                & 58                           & 24           & 2            & 7               & 7.465517241       \\
ALGORITHM, DATA\_STRUCTURE                  & 39.47368421  & 15                                & 38                           & 24           & 2            & 5               & 5.973684211       \\
DATA\_TYPE, FILE\_TYPE                      & 39.39393939  & 13                                & 33                           & 24           & 2            & 7               & 7.515151515       \\
DEVICE, LIBRARY                             & 39.13043478  & 9                                 & 23                           & 24           & 4            & 8               & 8.869565217       \\
FILE\_TYPE, IN\_LINE\_CODE                  & 38.88888889  & 14                                & 36                           & 24           & 3            & 6               & 7                 \\
LIBRARY, LIBRARY\_CLASS                     & 38.63636364  & 17                                & 44                           & 24           & 3            & 7               & 7.727272727       \\
PROGRAMMING\_LANGUAGE, HTML\_TAG\_NAME      & 38.46153846  & 5                                 & 13                           & 24           & 2            & 7               & 8.307692308       \\
OPERATION\_SYSTEM, USER\_FUNCTION\_NAME     & 38.46153846  & 5                                 & 13                           & 24           & 4            & 6               & 8.461538462       \\
DEVICE, FILE\_TYPE                          & 38.46153846  & 5                                 & 13                           & 24           & 4            & 8               & 9.692307692       \\
ERROR\_NAME, LIBRARY\_CLASS                 & 38.46153846  & 5                                 & 13                           & 24           & 5            & 7               & 10.07692308       \\
DATA\_TYPE, VALUE                           & 38.46153846  & 15                                & 39                           & 24           & 2            & 6               & 6.974358974       \\
LIBRARY, FILE\_TYPE                         & 38.46153846  & 30                                & 78                           & 24           & 3            & 7               & 7.41025641        \\
LIBRARY, LIBRARY\_FUNCTION                  & 38.4057971   & 53                                & 138                          & 19           & 2            & 6               & 6.405797101       \\
DATA\_STRUCTURE                             & 38.35294118  & 163                               & 425                          & 24           & 1            & 4               & 4.150588235       \\
DATA\_STRUCTURE, FILE\_TYPE                 & 38.29787234  & 18                                & 47                           & 24           & 3            & 7               & 7.255319149       \\
USER\_VARIABLE, LIBRARY\_FUNCTION           & 38.28125     & 49                                & 128                          & 19           & 3            & 6               & 6.5703125         \\
USER\_VARIABLE, VALUE                       & 38.20224719  & 34                                & 89                           & 24           & 3            & 6               & 6.752808989       \\
PROGRAMMING\_LANGUAGE, DEVICE               & 38.18181818  & 21                                & 55                           & 24           & 2            & 5               & 6.254545455       \\
LIBRARY\_CLASS, LIBRARY\_FUNCTION           & 37.93103448  & 11                                & 29                           & 19           & 3            & 7               & 7.896551724       \\
ERROR\_NAME, LIBRARY                        & 37.5         & 15                                & 40                           & 24           & 3            & 7               & 8.025             \\
ERROR\_NAME, FILE\_NAME                     & 37.5         & 12                                & 32                           & 24           & 3            & 7               & 7.84375           \\
LIBRARY\_CLASS, USER\_VARIABLE              & 37.5         & 9                                 & 24                           & 24           & 4            & 9               & 9.875             \\
ERROR\_NAME, LIBRARY\_FUNCTION              & 37.14285714  & 13                                & 35                           & 19           & 4            & 7               & 7.571428571       \\
DATA\_TYPE, LIBRARY                         & 37.09677419  & 23                                & 62                           & 24           & 3            & 7               & 7.580645161       \\
LIBRARY\_FUNCTION, USER\_FUNCTION\_NAME     & 37.09677419  & 23                                & 62                           & 12           & 4            & 7               & 7.032258065       \\
PROGRAMMING\_LANGUAGE, LIBRARY\_CLASS       & 36.95652174  & 17                                & 46                           & 24           & 3            & 7               & 7.826086957       \\
USER\_VARIABLE, KEYBOARD\_INPUT             & 36.84210526  & 7                                 & 19                           & 24           & 3            & 6               & 8.210526316       \\
PROGRAMMING\_LANGUAGE, FILE\_TYPE           & 36.64596273  & 59                                & 161                          & 24           & 2            & 5               & 5.677018634       \\
DATA\_STRUCTURE, LIBRARY                    & 36.52173913  & 42                                & 115                          & 24           & 2            & 6               & 6.356521739       \\
ERROR\_NAME                                 & 36.36363636  & 52                                & 143                          & 24           & 1            & 4               & 4.678321678       \\
DEVICE, ERROR\_NAME                         & 36.36363636  & 4                                 & 11                           & 24           & 3            & 5               & 8.727272727       \\
ERROR\_NAME, USER\_NAME                     & 36.36363636  & 4                                 & 11                           & 24           & 2            & 5               & 6.727272727       \\
USER\_NAME, FILE\_TYPE                      & 36.36363636  & 4                                 & 11                           & 24           & 3            & 7               & 8                 \\
DATA\_TYPE, KEYBOARD\_INPUT                 & 36.36363636  & 4                                 & 11                           & 24           & 5            & 7               & 9.818181818       \\
DATA\_TYPE                                  & 35.71428571  & 85                                & 238                          & 24           & 1            & 4               & 4.617647059       \\
PROGRAMMING\_LANGUAGE, DATA\_TYPE           & 35.71428571  & 65                                & 182                          & 24           & 2            & 4               & 5.131868132       \\
USER\_NAME, USER\_FUNCTION\_NAME            & 35.71428571  & 5                                 & 14                           & 24           & 3            & 6               & 6.785714286       \\
DATA\_TYPE, USER\_VARIABLE                  & 35.48387097  & 33                                & 93                           & 24           & 2            & 6               & 6.387096774       \\
APPLICATION, DATA\_STRUCTURE                & 35.29411765  & 24                                & 68                           & 24           & 2            & 4               & 5.176470588       \\
VERSION, ERROR\_NAME                        & 35.29411765  & 6                                 & 17                           & 24           & 2            & 5               & 8                 \\
ALGORITHM, VALUE                            & 35.29411765  & 6                                 & 17                           & 24           & 3            & 7               & 8.352941176       \\
APPLICATION, DATA\_TYPE                     & 35           & 7                                 & 20                           & 24           & 3            & 6               & 7.05              \\
FILE\_TYPE                                  & 34.75935829  & 65                                & 187                          & 24           & 1            & 5               & 5.417112299       \\
LIBRARY\_CLASS                              & 34.69387755  & 17                                & 49                           & 24           & 2            & 7               & 7.489795918       \\
VERSION, DATA\_STRUCTURE                    & 34.61538462  & 9                                 & 26                           & 24           & 3            & 7               & 8.269230769       \\
USER\_VARIABLE, IN\_LINE\_CODE              & 34.48275862  & 30                                & 87                           & 24           & 2            & 5               & 6.218390805       \\
DEVICE                                      & 34.375       & 22                                & 64                           & 24           & 2            & 5               & 5.9375            \\
FILE\_TYPE, VALUE                           & 34.375       & 11                                & 32                           & 24           & 3            & 7               & 8.1875            \\
PROGRAMMING\_LANGUAGE                       & 33.76700177  & 571                               & 1691                         & 24           & 1            & 2               & 2.897102306       \\
PROGRAMMING\_LANGUAGE, IN\_LINE\_CODE       & 33.75796178  & 53                                & 157                          & 24           & 2            & 4               & 5.178343949       \\
IN\_LINE\_CODE                              & 33.48837209  & 72                                & 215                          & 24           & 1            & 4               & 4.627906977       \\
VALUE                                       & 33.33333333  & 65                                & 195                          & 24           & 1            & 5               & 5.2               \\
APPLICATION, FILE\_TYPE                     & 33.33333333  & 8                                 & 24                           & 24           & 3            & 6.5             & 7.083333333       \\
PROGRAMMING\_LANGUAGE, VALUE                & 33.33333333  & 52                                & 156                          & 24           & 2            & 5               & 5.58974359        \\
VERSION, USER\_NAME                         & 33.33333333  & 4                                 & 12                           & 24           & 3            & 5               & 7.5               \\
VERSION, DATA\_TYPE                         & 33.33333333  & 6                                 & 18                           & 24           & 3            & 7.5             & 8.611111111       \\
OPERATION\_SYSTEM, FILE\_NAME               & 33.33333333  & 5                                 & 15                           & 24           & 3            & 8               & 9.333333333       \\
ERROR\_NAME, USER\_FUNCTION\_NAME           & 33.33333333  & 6                                 & 18                           & 24           & 4            & 8.5             & 9                 \\
DATA\_STRUCTURE, USER\_FUNCTION\_NAME       & 33.33333333  & 26                                & 78                           & 24           & 2            & 6               & 6.320512821       \\
DATA\_STRUCTURE, IN\_LINE\_CODE             & 33.33333333  & 16                                & 48                           & 24           & 3            & 6               & 7.041666667       \\
LIBRARY, FILE\_NAME                         & 33.33333333  & 24                                & 72                           & 24           & 3            & 7               & 7.583333333       \\
USER\_FUNCTION\_NAME, FILE\_TYPE            & 33.33333333  & 13                                & 39                           & 24           & 4            & 8               & 8.179487179       \\
USER\_VARIABLE, FILE\_TYPE                  & 32.87671233  & 24                                & 73                           & 24           & 3            & 7               & 7.273972603       \\
PROGRAMMING\_LANGUAGE, USER\_VARIABLE       & 32.8358209   & 132                               & 402                          & 24           & 2            & 4               & 4.875621891       \\
PROGRAMMING\_LANGUAGE, VERSION              & 32.63157895  & 31                                & 95                           & 24           & 2            & 4               & 5.452631579       \\
LIBRARY\_FUNCTION, IN\_LINE\_CODE           & 32.60869565  & 15                                & 46                           & 19           & 3            & 6               & 6.739130435       \\
PROGRAMMING\_LANGUAGE, KEYBOARD\_INPUT      & 32.43243243  & 12                                & 37                           & 24           & 2            & 6               & 7                 \\
USER\_VARIABLE                              & 32.18623482  & 159                               & 494                          & 24           & 1            & 4               & 4.591093117       \\
APPLICATION                                 & 32.12121212  & 106                               & 330                          & 24           & 1            & 3               & 3.242424242       \\
APPLICATION, PROGRAMMING\_LANGUAGE          & 32.05741627  & 67                                & 209                          & 24           & 2            & 3               & 3.76076555        \\
DATA\_STRUCTURE, USER\_VARIABLE             & 31.6091954   & 55                                & 174                          & 24           & 2            & 5               & 5.614942529       \\
PROGRAMMING\_LANGUAGE, UI\_ELEMENT          & 31.57894737  & 6                                 & 19                           & 24           & 2            & 5               & 7.947368421       \\
VALUE, IN\_LINE\_CODE                       & 31.48148148  & 17                                & 54                           & 24           & 2            & 6               & 6.62962963        \\
ALGORITHM                                   & 31.40495868  & 38                                & 121                          & 24           & 1            & 4               & 4.231404959       \\
DATA\_TYPE, USER\_FUNCTION\_NAME            & 31.37254902  & 16                                & 51                           & 24           & 3            & 7               & 6.823529412       \\
PROGRAMMING\_LANGUAGE, LIBRARY              & 31.36645963  & 101                               & 322                          & 24           & 2            & 5               & 5.139751553       \\
LIBRARY                                     & 31.31868132  & 114                               & 364                          & 24           & 1            & 4               & 4.945054945       \\
LIBRARY, KEYBOARD\_INPUT                    & 31.25        & 5                                 & 16                           & 24           & 5            & 9               & 10                \\
FILE\_NAME, VALUE                           & 31.25        & 10                                & 32                           & 24           & 2            & 7.5             & 8.28125           \\
VERSION                                     & 31.06060606  & 41                                & 132                          & 24           & 1            & 4               & 4.772727273       \\
PROGRAMMING\_LANGUAGE, ALGORITHM            & 30.92783505  & 30                                & 97                           & 24           & 2            & 4               & 4.618556701       \\
APPLICATION, ALGORITHM                      & 30.76923077  & 8                                 & 26                           & 24           & 2            & 4               & 5.115384615       \\
PROGRAMMING\_LANGUAGE, FILE\_NAME           & 30.76923077  & 52                                & 169                          & 24           & 2            & 5               & 5.485207101       \\
ALGORITHM, USER\_NAME                       & 30.76923077  & 4                                 & 13                           & 24           & 3            & 4               & 5.846153846       \\
USER\_VARIABLE, OUTPUT\_BLOCK               & 30.76923077  & 4                                 & 13                           & 24           & 5            & 8               & 10.61538462       \\
OPERATION\_SYSTEM, VALUE                    & 30.43478261  & 7                                 & 23                           & 24           & 2            & 6               & 7.826086957       \\
PROGRAMMING\_LANGUAGE, OPERATION\_SYSTEM    & 30.26315789  & 23                                & 76                           & 24           & 2            & 4               & 5.236842105       \\
APPLICATION, USER\_FUNCTION\_NAME           & 30           & 9                                 & 30                           & 24           & 2            & 5               & 6.233333333       \\
APPLICATION, WEBSITE                        & 30           & 3                                 & 10                           & 24           & 2            & 6               & 7                 \\
LIBRARY\_VARIABLE, USER\_VARIABLE           & 30           & 3                                 & 10                           & 19           & 3            & 8.5             & 9.4               \\
FILE\_NAME                                  & 29.78723404  & 56                                & 188                          & 24           & 1            & 5               & 5.292553191       \\
VERSION, IN\_LINE\_CODE                     & 29.41176471  & 5                                 & 17                           & 24           & 3            & 7               & 8.411764706       \\
PROGRAMMING\_LANGUAGE, USER\_NAME           & 29.29292929  & 29                                & 99                           & 24           & 2            & 3               & 4.03030303        \\
FILE\_NAME, IN\_LINE\_CODE                  & 28.94736842  & 11                                & 38                           & 24           & 3            & 6               & 7.184210526       \\
PROGRAMMING\_LANGUAGE, OUTPUT\_BLOCK        & 28.57142857  & 4                                 & 14                           & 24           & 5            & 8.5             & 10.57142857       \\
OPERATION\_SYSTEM, ERROR\_NAME              & 28.57142857  & 4                                 & 14                           & 24           & 3            & 7               & 8.5               \\
OPERATION\_SYSTEM, USER\_VARIABLE           & 28.57142857  & 6                                 & 21                           & 24           & 3            & 6               & 8.19047619        \\
DEVICE, VALUE                               & 28.57142857  & 4                                 & 14                           & 24           & 4            & 8               & 10.35714286       \\
DEVICE, IN\_LINE\_CODE                      & 28.57142857  & 4                                 & 14                           & 24           & 4            & 7.5             & 10                \\
DATA\_STRUCTURE, LIBRARY\_CLASS             & 28.57142857  & 6                                 & 21                           & 24           & 4            & 8               & 9.047619048       \\
DATA\_TYPE, LIBRARY\_CLASS                  & 28.57142857  & 4                                 & 14                           & 24           & 2            & 8               & 9.857142857       \\
USER\_VARIABLE, FILE\_NAME                  & 28.57142857  & 18                                & 63                           & 24           & 3            & 7               & 7.634920635       \\
USER\_FUNCTION\_NAME, VALUE                 & 28.26086957  & 13                                & 46                           & 24           & 4            & 6.5             & 7.326086957       \\
ERROR\_NAME, IN\_LINE\_CODE                 & 28.125       & 9                                 & 32                           & 24           & 3            & 6               & 7.5               \\
LIBRARY, USER\_VARIABLE                     & 28.05755396  & 39                                & 139                          & 24           & 2            & 6               & 6.575539568       \\
OUTPUT\_BLOCK                               & 27.77777778  & 5                                 & 18                           & 24           & 2            & 7.5             & 9.444444444       \\
DEVICE, DATA\_STRUCTURE                     & 27.77777778  & 5                                 & 18                           & 24           & 2            & 7               & 8.5               \\
DEVICE, FILE\_NAME                          & 27.77777778  & 5                                 & 18                           & 24           & 4            & 8               & 9.111111111       \\
OPERATION\_SYSTEM                           & 27.61904762  & 29                                & 105                          & 24           & 1            & 4               & 4.619047619       \\
ALGORITHM, LIBRARY\_FUNCTION                & 27.27272727  & 3                                 & 11                           & 19           & 4            & 7               & 8.090909091       \\
OPERATION\_SYSTEM, LIBRARY                  & 27.27272727  & 6                                 & 22                           & 24           & 3            & 7               & 8.5               \\
USER\_VARIABLE, UI\_ELEMENT                 & 27.27272727  & 3                                 & 11                           & 24           & 3            & 9               & 10.72727273       \\
USER\_FUNCTION\_NAME, IN\_LINE\_CODE        & 27.27272727  & 12                                & 44                           & 24           & 3            & 6               & 7.068181818       \\
DATA\_STRUCTURE, KEYBOARD\_INPUT            & 26.66666667  & 4                                 & 15                           & 24           & 3            & 6               & 7.666666667       \\
LIBRARY, USER\_FUNCTION\_NAME               & 26.66666667  & 20                                & 75                           & 24           & 3            & 7               & 7.106666667       \\
LIBRARY, IN\_LINE\_CODE                     & 26.66666667  & 12                                & 45                           & 24           & 3            & 7               & 7.933333333       \\
LIBRARY\_CLASS, IN\_LINE\_CODE              & 26.66666667  & 4                                 & 15                           & 24           & 5            & 8               & 10.06666667       \\
ALGORITHM, LIBRARY                          & 26.31578947  & 5                                 & 19                           & 24           & 3            & 5               & 7.842105263       \\
APPLICATION, USER\_VARIABLE                 & 26.15384615  & 17                                & 65                           & 24           & 2            & 5               & 5.538461538       \\
PROGRAMMING\_LANGUAGE, USER\_FUNCTION\_NAME & 25.38071066  & 50                                & 197                          & 24           & 2            & 5               & 5.446700508       \\
KEYBOARD\_INPUT                             & 25           & 12                                & 48                           & 24           & 1            & 5               & 6.145833333       \\
VERSION, ALGORITHM                          & 25           & 4                                 & 16                           & 24           & 3            & 4.5             & 7.5               \\
OPERATION\_SYSTEM, DATA\_TYPE               & 25           & 4                                 & 16                           & 24           & 3            & 6               & 8.75              \\
DEVICE, USER\_VARIABLE                      & 25           & 5                                 & 20                           & 24           & 3            & 6.5             & 8.3               \\
USER\_VARIABLE, USER\_FUNCTION\_NAME        & 24.69879518  & 41                                & 166                          & 24           & 2            & 5               & 5.722891566       \\
USER\_FUNCTION\_NAME                        & 24.56140351  & 56                                & 228                          & 24           & 2            & 5               & 5.254385965       \\
VERSION, USER\_VARIABLE                     & 24.3902439   & 10                                & 41                           & 24           & 2            & 5               & 7.097560976       \\
USER\_FUNCTION\_NAME, FILE\_NAME            & 24.3902439   & 10                                & 41                           & 24           & 3            & 8               & 8                 \\
UI\_ELEMENT                                 & 24           & 6                                 & 25                           & 24           & 1            & 5               & 6.88              \\
USER\_NAME, USER\_VARIABLE                  & 23.52941176  & 8                                 & 34                           & 24           & 2            & 5               & 5.617647059       \\
USER\_NAME                                  & 23.4939759   & 39                                & 166                          & 24           & 1            & 3               & 3.277108434       \\
APPLICATION, DEVICE                         & 23.07692308  & 3                                 & 13                           & 24           & 2            & 4               & 6.076923077       \\
VERSION, USER\_FUNCTION\_NAME               & 23.07692308  & 3                                 & 13                           & 24           & 3            & 5               & 8.538461538       \\
USER\_FUNCTION\_NAME, KEYBOARD\_INPUT       & 23.07692308  & 3                                 & 13                           & 24           & 4            & 7               & 8.692307692       \\
ALGORITHM, USER\_VARIABLE                   & 22.85714286  & 8                                 & 35                           & 24           & 3            & 5               & 6.542857143       \\
APPLICATION, USER\_NAME                     & 20.93023256  & 9                                 & 43                           & 24           & 2            & 3               & 4.488372093       \\
APPLICATION, OPERATION\_SYSTEM              & 20           & 4                                 & 20                           & 24           & 2            & 4               & 5.3               \\
LIBRARY\_FUNCTION, KEYBOARD\_INPUT          & 20           & 3                                 & 15                           & 19           & 5            & 7               & 8.066666667       \\
FILE\_TYPE, WEBSITE                         & 20           & 2                                 & 10                           & 24           & 3            & 6               & 7.3               \\
IN\_LINE\_CODE, OUTPUT\_BLOCK               & 20           & 3                                 & 15                           & 24           & 2            & 8               & 10.13333333       \\
WEBSITE                                     & 19.60784314  & 10                                & 51                           & 24           & 1            & 3               & 3.882352941       \\
OPERATION\_SYSTEM, LIBRARY\_FUNCTION        & 18.75        & 3                                 & 16                           & 19           & 3            & 5.5             & 6.625             \\
USER\_NAME, FILE\_NAME                      & 18.75        & 3                                 & 16                           & 24           & 2            & 5               & 6.25              \\
VALUE, KEYBOARD\_INPUT                      & 18.75        & 3                                 & 16                           & 24           & 4            & 6.5             & 9                 \\
IN\_LINE\_CODE, KEYBOARD\_INPUT             & 18.75        & 3                                 & 16                           & 24           & 2            & 6.5             & 8.5625            \\
ALGORITHM, USER\_FUNCTION\_NAME             & 17.64705882  & 3                                 & 17                           & 24           & 2            & 7               & 7.764705882       \\
APPLICATION, FILE\_NAME                     & 17.24137931  & 5                                 & 29                           & 24           & 3            & 5               & 6.275862069       \\
PROGRAMMING\_LANGUAGE, WEBSITE              & 17.07317073  & 7                                 & 41                           & 24           & 2            & 3               & 4.268292683      
\end{tabular}
\end{table}

==> tablets/intent_API_CHANGE_upto2_combinations_success_rate.tex <==
\begin{table}
\centering
\caption{Entity Combinations in API CHANGE intent}
\label{tab:intent_API_CHANGE_upto2_combinations_success_rate}

\begin{tabular}{llllllll}
Entities Combination                     & Success Rate & Number of Successful Combinations & Total Number of Combinations & Max Entities & Min Entities & Median Entities & Average Entities  \\
PROGRAMMING\_LANGUAGE, LIBRARY\_FUNCTION & 63.64        & 7                                 & 11                           & 11           & 3            & 4               & 4.91              \\
LIBRARY\_FUNCTION                        & 58.33        & 7                                 & 12                           & 11           & 2            & 3.5             & 4.67              \\
FILE\_NAME                               & 42.11        & 8                                 & 19                           & 10           & 2            & 3               & 4.58              \\
PROGRAMMING\_LANGUAGE, FILE\_NAME        & 41.18        & 7                                 & 17                           & 10           & 2            & 4               & 4.82              \\
OPERATION\_SYSTEM                        & 40.00        & 4                                 & 10                           & 4            & 2            & 2.5             & 2.60              \\
USER\_VARIABLE                           & 36.36        & 4                                 & 11                           & 11           & 2            & 4               & 4.64              \\
LIBRARY                                  & 33.33        & 10                                & 30                           & 10           & 1            & 3               & 3.90              \\
FILE\_TYPE                               & 33.33        & 4                                 & 12                           & 11           & 3            & 6               & 6.08              \\
PROGRAMMING\_LANGUAGE, FILE\_TYPE        & 33.33        & 4                                 & 12                           & 11           & 3            & 6               & 6.08              \\
PROGRAMMING\_LANGUAGE, LIBRARY           & 32.00        & 8                                 & 25                           & 10           & 2            & 4               & 4.32              \\
VALUE                                    & 30.00        & 3                                 & 10                           & 11           & 1            & 4               & 4.90              \\
PROGRAMMING\_LANGUAGE, USER\_VARIABLE    & 30.00        & 3                                 & 10                           & 11           & 2            & 4               & 4.90              \\
ERROR\_NAME                              & 27.78        & 5                                 & 18                           & 10           & 1            & 3               & 3.94              \\
PROGRAMMING\_LANGUAGE, ERROR\_NAME       & 27.27        & 3                                 & 11                           & 10           & 2            & 4               & 5.18              \\
APPLICATION                              & 25.93        & 7                                 & 27                           & 11           & 1            & 2               & 2.85              \\
APPLICATION, PROGRAMMING\_LANGUAGE       & 25.00        & 5                                 & 20                           & 11           & 2            & 2.5             & 3.25              \\
PROGRAMMING\_LANGUAGE                    & 24.60        & 31                                & 126                          & 11           & 1            & 2               & 2.43              \\
VERSION                                  & 14.29        & 4                                 & 28                           & 11           & 1            & 2               & 2.82              \\
USER\_NAME                               & 14.29        & 2                                 & 14                           & 11           & 1            & 3               & 3.21              \\
PROGRAMMING\_LANGUAGE, VERSION           & 14.29        & 2                                 & 14                           & 11           & 2            & 3               & 4.36              \\
PROGRAMMING\_LANGUAGE, USER\_NAME        & 0.00         & 0                                 & 10                           & 11           & 2            & 3               & 3.90             
\end{tabular}
\end{table}

==> tablets/intent_API_USAGE_upto2_combinations_success_rate.tex <==
\begin{table}
\centering
\caption{Entity Combinations in API USAGE intent}
\label{tab:intent_API_USAGE_upto2_combinations_success_rate}

\begin{tabular}{llllllll}
Entities Combination                        & Success Rate & Number of Successful Combinations & Total Number of Combinations & Max Entities & Min Entities & Median Entities & Average Entities  \\
DATA\_STRUCTURE, OUTPUT\_BLOCK              & 75.00        & 9                                 & 12                           & 24           & 3            & 17.5            & 15.58             \\
ALGORITHM, ERROR\_NAME                      & 66.67        & 8                                 & 12                           & 24           & 3            & 11.5            & 12.25             \\
DATA\_TYPE, UI\_ELEMENT                     & 63.64        & 7                                 & 11                           & 24           & 8            & 17              & 17.27             \\
USER\_NAME, LIBRARY\_FUNCTION               & 63.16        & 12                                & 19                           & 22           & 4            & 7               & 8.68              \\
DATA\_TYPE, OUTPUT\_BLOCK                   & 61.54        & 8                                 & 13                           & 24           & 8            & 17              & 15.46             \\
UI\_ELEMENT, OUTPUT\_BLOCK                  & 60.00        & 6                                 & 10                           & 24           & 5            & 17.5            & 16.50             \\
VERSION, DATA\_STRUCTURE                    & 56.00        & 14                                & 25                           & 24           & 3            & 9               & 11.24             \\
UI\_ELEMENT, IN\_LINE\_CODE                 & 55.56        & 10                                & 18                           & 24           & 4            & 14              & 12.56             \\
DEVICE, OUTPUT\_BLOCK                       & 54.55        & 6                                 & 11                           & 24           & 11           & 18              & 17.73             \\
LIBRARY\_CLASS, WEBSITE                     & 54.55        & 6                                 & 11                           & 24           & 4            & 18              & 16.73             \\
WEBSITE, IN\_LINE\_CODE                     & 54.55        & 6                                 & 11                           & 24           & 4            & 18              & 16.73             \\
WEBSITE, KEYBOARD\_INPUT                    & 54.55        & 6                                 & 11                           & 24           & 7            & 18              & 17.73             \\
USER\_NAME, DATA\_STRUCTURE                 & 54.29        & 19                                & 35                           & 24           & 3            & 6               & 7.43              \\
VERSION, OUTPUT\_BLOCK                      & 53.85        & 7                                 & 13                           & 24           & 3            & 17              & 14.08             \\
LIBRARY\_FUNCTION, WEBSITE                  & 53.85        & 7                                 & 13                           & 22           & 5            & 12              & 12.77             \\
DATA\_STRUCTURE, UI\_ELEMENT                & 53.33        & 8                                 & 15                           & 24           & 2            & 17              & 14.33             \\
DEVICE, IN\_LINE\_CODE                      & 52.17        & 12                                & 23                           & 24           & 4            & 11              & 12.48             \\
PROGRAMMING\_LANGUAGE, LIBRARY\_CLASS       & 51.16        & 44                                & 86                           & 24           & 2            & 6.5             & 7.59              \\
PROGRAMMING\_LANGUAGE, USER\_CLASS          & 50.00        & 9                                 & 18                           & 24           & 3            & 6               & 9.78              \\
VERSION, DEVICE                             & 50.00        & 13                                & 26                           & 24           & 3            & 8               & 11.08             \\
OPERATION\_SYSTEM, USER\_NAME               & 50.00        & 9                                 & 18                           & 24           & 3            & 5.5             & 8.22              \\
OPERATION\_SYSTEM, UI\_ELEMENT              & 50.00        & 6                                 & 12                           & 24           & 4            & 17.5            & 15.67             \\
DEVICE, LIBRARY\_FUNCTION                   & 50.00        & 14                                & 28                           & 22           & 4            & 8               & 9.86              \\
ERROR\_NAME, LIBRARY\_CLASS                 & 50.00        & 7                                 & 14                           & 24           & 5            & 12              & 13.79             \\
DATA\_STRUCTURE, HTML\_TAG\_NAME            & 50.00        & 5                                 & 10                           & 24           & 6            & 17.5            & 16.70             \\
LIBRARY\_CLASS, UI\_ELEMENT                 & 50.00        & 5                                 & 10                           & 24           & 9            & 18              & 17.70             \\
LIBRARY\_CLASS, IN\_LINE\_CODE              & 50.00        & 13                                & 26                           & 24           & 3            & 9               & 11.81             \\
UI\_ELEMENT, WEBSITE                        & 50.00        & 7                                 & 14                           & 24           & 3            & 17              & 13.93             \\
UI\_ELEMENT, KEYBOARD\_INPUT                & 50.00        & 6                                 & 12                           & 24           & 2            & 17.5            & 16.08             \\
WEBSITE, HTML\_TAG\_NAME                    & 50.00        & 5                                 & 10                           & 24           & 2            & 17.5            & 16.30             \\
LIBRARY\_CLASS, USER\_VARIABLE              & 48.89        & 22                                & 45                           & 24           & 3            & 8               & 9.51              \\
DATA\_STRUCTURE, LIBRARY\_CLASS             & 48.48        & 16                                & 33                           & 24           & 5            & 9               & 11.15             \\
LIBRARY\_CLASS                              & 48.39        & 45                                & 93                           & 24           & 2            & 6               & 7.46              \\
ALGORITHM, DEVICE                           & 48.00        & 12                                & 25                           & 24           & 4            & 6               & 10.00             \\
LIBRARY\_CLASS, FILE\_TYPE                  & 48.00        & 12                                & 25                           & 24           & 4            & 9               & 11.76             \\
DEVICE, ERROR\_NAME                         & 47.62        & 10                                & 21                           & 24           & 4            & 8               & 10.52             \\
LIBRARY, LIBRARY\_CLASS                     & 47.50        & 38                                & 80                           & 24           & 3            & 7               & 7.85              \\
DEVICE, USER\_NAME                          & 47.37        & 9                                 & 19                           & 24           & 3            & 5               & 8.74              \\
DEVICE, KEYBOARD\_INPUT                     & 47.37        & 9                                 & 19                           & 24           & 4            & 17              & 13.53             \\
ERROR\_NAME, USER\_NAME                     & 47.37        & 9                                 & 19                           & 24           & 3            & 6               & 8.00              \\
DATA\_TYPE, LIBRARY\_CLASS                  & 47.22        & 17                                & 36                           & 24           & 2            & 9               & 10.42             \\
USER\_CLASS, USER\_VARIABLE                 & 47.06        & 8                                 & 17                           & 24           & 3            & 6               & 10.12             \\
HTML\_TAG\_NAME                             & 46.67        & 7                                 & 15                           & 24           & 1            & 16              & 11.93             \\
VERSION, ALGORITHM                          & 46.67        & 7                                 & 15                           & 24           & 4            & 11              & 11.80             \\
VERSION, DATA\_TYPE                         & 46.67        & 7                                 & 15                           & 24           & 7            & 17              & 14.67             \\
USER\_FUNCTION\_NAME, OUTPUT\_BLOCK         & 46.67        & 7                                 & 15                           & 24           & 6            & 14              & 14.13             \\
LIBRARY\_CLASS, USER\_FUNCTION\_NAME        & 46.43        & 13                                & 28                           & 24           & 5            & 9               & 11.18             \\
OPERATION\_SYSTEM, LIBRARY\_CLASS           & 46.15        & 6                                 & 13                           & 24           & 6            & 16              & 15.00             \\
OPERATION\_SYSTEM, WEBSITE                  & 46.15        & 6                                 & 13                           & 24           & 4            & 17              & 15.23             \\
FILE\_NAME, OUTPUT\_BLOCK                   & 46.15        & 6                                 & 13                           & 24           & 4            & 11              & 13.38             \\
WEBSITE, VALUE                              & 46.15        & 6                                 & 13                           & 24           & 4            & 17              & 14.77             \\
PROGRAMMING\_LANGUAGE, DATA\_STRUCTURE      & 46.11        & 160                               & 347                          & 24           & 2            & 4               & 4.79              \\
VERSION, USER\_VARIABLE                     & 45.95        & 17                                & 37                           & 24           & 3            & 7               & 9.27              \\
VERSION, IN\_LINE\_CODE                     & 45.71        & 16                                & 35                           & 24           & 2            & 7               & 8.94              \\
PROGRAMMING\_LANGUAGE, HTML\_TAG\_NAME      & 45.45        & 5                                 & 11                           & 24           & 4            & 17              & 15.55             \\
VERSION, UI\_ELEMENT                        & 45.45        & 5                                 & 11                           & 24           & 5            & 17              & 16.00             \\
USER\_CLASS                                 & 45.00        & 9                                 & 20                           & 24           & 2            & 6               & 9.80              \\
DATA\_STRUCTURE, KEYBOARD\_INPUT            & 45.00        & 9                                 & 20                           & 24           & 3            & 13.5            & 12.45             \\
LIBRARY, OUTPUT\_BLOCK                      & 45.00        & 9                                 & 20                           & 24           & 5            & 11              & 13.10             \\
DATA\_STRUCTURE, WEBSITE                    & 44.44        & 8                                 & 18                           & 24           & 4            & 16.5            & 13.78             \\
OPERATION\_SYSTEM, DEVICE                   & 44.00        & 22                                & 50                           & 24           & 2            & 5               & 7.60              \\
OPERATION\_SYSTEM, ERROR\_NAME              & 44.00        & 11                                & 25                           & 24           & 3            & 6               & 8.60              \\
OPERATION\_SYSTEM, LIBRARY\_FUNCTION        & 44.00        & 11                                & 25                           & 22           & 2            & 7               & 9.00              \\
DEVICE, DATA\_TYPE                          & 44.00        & 11                                & 25                           & 24           & 3            & 11              & 11.96             \\
VERSION, USER\_FUNCTION\_NAME               & 43.75        & 7                                 & 16                           & 24           & 3            & 14              & 12.94             \\
OPERATION\_SYSTEM, KEYBOARD\_INPUT          & 43.75        & 7                                 & 16                           & 24           & 3            & 13.5            & 12.94             \\
DATA\_STRUCTURE, USER\_CLASS                & 43.75        & 7                                 & 16                           & 24           & 2            & 7.5             & 11.13             \\
DATA\_TYPE, WEBSITE                         & 43.75        & 7                                 & 16                           & 24           & 3            & 16.5            & 13.44             \\
FILE\_NAME, UI\_ELEMENT                     & 43.75        & 7                                 & 16                           & 24           & 4            & 10.5            & 12.69             \\
DEVICE, VALUE                               & 43.48        & 10                                & 23                           & 24           & 3            & 8               & 11.39             \\
VERSION, FILE\_TYPE                         & 43.24        & 16                                & 37                           & 24           & 4            & 7               & 9.32              \\
DATA\_STRUCTURE                             & 43.02        & 194                               & 451                          & 24           & 1            & 4               & 4.35              \\
PROGRAMMING\_LANGUAGE, OUTPUT\_BLOCK        & 42.86        & 12                                & 28                           & 24           & 2            & 9               & 10.93             \\
DEVICE, WEBSITE                             & 42.86        & 6                                 & 14                           & 24           & 4            & 17.5            & 15.21             \\
ERROR\_NAME, USER\_FUNCTION\_NAME           & 42.86        & 12                                & 28                           & 24           & 3            & 7               & 9.64              \\
FILE\_TYPE, OUTPUT\_BLOCK                   & 42.86        & 6                                 & 14                           & 24           & 5            & 11.5            & 13.57             \\
DEVICE, DATA\_STRUCTURE                     & 42.31        & 11                                & 26                           & 24           & 2            & 10              & 11.85             \\
OPERATION\_SYSTEM, VALUE                    & 42.11        & 8                                 & 19                           & 24           & 3            & 8               & 10.95             \\
DEVICE, LIBRARY                             & 42.11        & 24                                & 57                           & 24           & 3            & 6               & 8.30              \\
PROGRAMMING\_LANGUAGE, LIBRARY\_VARIABLE    & 41.67        & 5                                 & 12                           & 22           & 2            & 8.5             & 9.50              \\
VERSION, WEBSITE                            & 41.67        & 5                                 & 12                           & 24           & 5            & 17.5            & 15.58             \\
ERROR\_NAME, DATA\_STRUCTURE                & 41.67        & 10                                & 24                           & 24           & 4            & 6               & 9.33              \\
LIBRARY\_CLASS, LIBRARY\_FUNCTION           & 41.46        & 17                                & 41                           & 22           & 3            & 8               & 8.85              \\
VERSION, LIBRARY\_FUNCTION                  & 41.38        & 12                                & 29                           & 18           & 3            & 7               & 8.83              \\
OPERATION\_SYSTEM, IN\_LINE\_CODE           & 41.38        & 12                                & 29                           & 24           & 3            & 6               & 9.52              \\
ERROR\_NAME, USER\_VARIABLE                 & 41.33        & 31                                & 75                           & 24           & 3            & 6               & 7.00              \\
DEVICE, LIBRARY\_CLASS                      & 41.18        & 7                                 & 17                           & 24           & 5            & 16              & 14.29             \\
DATA\_STRUCTURE, FILE\_TYPE                 & 40.91        & 27                                & 66                           & 24           & 2            & 6               & 7.98              \\
IN\_LINE\_CODE, OUTPUT\_BLOCK               & 40.91        & 9                                 & 22                           & 24           & 3            & 9.5             & 11.73             \\
DATA\_STRUCTURE, USER\_VARIABLE             & 40.56        & 73                                & 180                          & 24           & 2            & 5               & 5.98              \\
APPLICATION, WEBSITE                        & 40.00        & 8                                 & 20                           & 24           & 2            & 5               & 8.00              \\
DATA\_STRUCTURE, FILE\_NAME                 & 40.00        & 18                                & 45                           & 24           & 3            & 7               & 8.93              \\
DATA\_TYPE, KEYBOARD\_INPUT                 & 40.00        & 8                                 & 20                           & 24           & 6            & 13.5            & 13.60             \\
LIBRARY, LIBRARY\_VARIABLE                  & 40.00        & 4                                 & 10                           & 22           & 6            & 9               & 10.70             \\
LIBRARY\_FUNCTION, OUTPUT\_BLOCK            & 40.00        & 6                                 & 15                           & 22           & 7            & 11              & 12.27             \\
VERSION, FILE\_NAME                         & 39.47        & 15                                & 38                           & 24           & 3            & 7               & 8.45              \\
APPLICATION, DATA\_STRUCTURE                & 39.39        & 26                                & 66                           & 24           & 2            & 5               & 6.35              \\
ALGORITHM, IN\_LINE\_CODE                   & 39.13        & 9                                 & 23                           & 24           & 2            & 7               & 9.87              \\
DATA\_TYPE, FILE\_NAME                      & 38.71        & 12                                & 31                           & 24           & 4            & 9               & 10.48             \\
PROGRAMMING\_LANGUAGE, DATA\_TYPE           & 38.57        & 86                                & 223                          & 24           & 2            & 5               & 5.68              \\
VERSION, LIBRARY\_CLASS                     & 38.46        & 5                                 & 13                           & 24           & 7            & 17              & 15.08             \\
DEVICE, FILE\_NAME                          & 38.46        & 10                                & 26                           & 24           & 3            & 7.5             & 10.58             \\
APPLICATION, ALGORITHM                      & 37.50        & 9                                 & 24                           & 24           & 2            & 5               & 7.88              \\
USER\_NAME, DATA\_TYPE                      & 37.50        & 6                                 & 16                           & 24           & 3            & 6               & 9.94              \\
VALUE, OUTPUT\_BLOCK                        & 37.50        & 6                                 & 16                           & 24           & 5            & 13              & 13.88             \\
DATA\_TYPE, IN\_LINE\_CODE                  & 37.29        & 22                                & 59                           & 24           & 2            & 8               & 8.93              \\
OUTPUT\_BLOCK                               & 37.14        & 13                                & 35                           & 24           & 1            & 8               & 9.83              \\
PROGRAMMING\_LANGUAGE, DEVICE               & 37.09        & 56                                & 151                          & 24           & 2            & 4               & 5.50              \\
USER\_NAME, VALUE                           & 37.04        & 10                                & 27                           & 24           & 3            & 5               & 7.56              \\
DATA\_TYPE, FILE\_TYPE                      & 36.96        & 17                                & 46                           & 24           & 3            & 8               & 9.22              \\
PROGRAMMING\_LANGUAGE, VERSION              & 36.92        & 48                                & 130                          & 24           & 2            & 5               & 5.83              \\
APPLICATION, VERSION                        & 36.84        & 14                                & 38                           & 24           & 2            & 5               & 6.84              \\
VERSION, LIBRARY                            & 36.84        & 21                                & 57                           & 24           & 3            & 6               & 8.11              \\
ALGORITHM, LIBRARY\_FUNCTION                & 36.84        & 7                                 & 19                           & 18           & 4            & 6               & 7.58              \\
USER\_NAME, FILE\_NAME                      & 36.84        & 7                                 & 19                           & 24           & 2            & 5               & 7.63              \\
OUTPUT\_BLOCK, KEYBOARD\_INPUT              & 36.84        & 7                                 & 19                           & 24           & 4            & 11              & 13.05             \\
FILE\_TYPE, FILE\_NAME                      & 36.52        & 42                                & 115                          & 24           & 2            & 6               & 6.89              \\
ALGORITHM, LIBRARY\_CLASS                   & 36.36        & 4                                 & 11                           & 24           & 5            & 17              & 16.27             \\
ALGORITHM, WEBSITE                          & 36.36        & 4                                 & 11                           & 24           & 5            & 16              & 13.82             \\
ERROR\_NAME, WEBSITE                        & 36.36        & 4                                 & 11                           & 24           & 3            & 7               & 12.27             \\
LIBRARY\_CLASS, KEYBOARD\_INPUT             & 36.36        & 4                                 & 11                           & 24           & 7            & 18              & 17.09             \\
DATA\_TYPE                                  & 36.23        & 100                               & 276                          & 24           & 1            & 4               & 5.21              \\
USER\_NAME, USER\_VARIABLE                  & 36.21        & 21                                & 58                           & 24           & 2            & 5.5             & 6.45              \\
DATA\_TYPE, LIBRARY\_FUNCTION               & 36.11        & 26                                & 72                           & 22           & 3            & 7               & 7.97              \\
LIBRARY\_VARIABLE                           & 35.71        & 5                                 & 14                           & 22           & 2            & 7.5             & 8.71              \\
VERSION, USER\_NAME                         & 35.71        & 5                                 & 14                           & 24           & 3            & 6               & 9.71              \\
VERSION, KEYBOARD\_INPUT                    & 35.71        & 5                                 & 14                           & 24           & 7            & 17              & 15.86             \\
OPERATION\_SYSTEM, USER\_VARIABLE           & 35.59        & 21                                & 59                           & 24           & 2            & 6               & 7.19              \\
OPERATION\_SYSTEM, USER\_FUNCTION\_NAME     & 35.48        & 11                                & 31                           & 24           & 2            & 6               & 8.71              \\
DEVICE, UI\_ELEMENT                         & 35.29        & 6                                 & 17                           & 24           & 4            & 17              & 13.41             \\
VERSION                                     & 35.26        & 55                                & 156                          & 24           & 1            & 4               & 5.35              \\
DEVICE, USER\_FUNCTION\_NAME                & 35.14        & 13                                & 37                           & 24           & 3            & 6               & 9.08              \\
DATA\_TYPE, USER\_VARIABLE                  & 35.09        & 40                                & 114                          & 24           & 2            & 6               & 6.95              \\
DEVICE                                      & 35.00        & 63                                & 180                          & 24           & 1            & 4               & 5.23              \\
APPLICATION, FILE\_NAME                     & 34.78        & 16                                & 46                           & 24           & 2            & 5               & 6.70              \\
DATA\_TYPE, LIBRARY                         & 34.78        & 32                                & 92                           & 24           & 3            & 7               & 7.76              \\
LIBRARY\_CLASS, FILE\_NAME                  & 34.78        & 8                                 & 23                           & 24           & 6            & 9               & 11.91             \\
PROGRAMMING\_LANGUAGE, LIBRARY\_FUNCTION    & 34.77        & 105                               & 302                          & 22           & 2            & 5               & 5.62              \\
USER\_FUNCTION\_NAME, KEYBOARD\_INPUT       & 34.62        & 9                                 & 26                           & 24           & 3            & 7.5             & 10.85             \\
LIBRARY, LIBRARY\_FUNCTION                  & 34.59        & 64                                & 185                          & 22           & 3            & 6               & 6.42              \\
DATA\_STRUCTURE, DATA\_TYPE                 & 34.55        & 38                                & 110                          & 24           & 2            & 5               & 6.92              \\
OPERATION\_SYSTEM, DATA\_TYPE               & 34.48        & 10                                & 29                           & 24           & 3            & 6               & 9.72              \\
DATA\_STRUCTURE, IN\_LINE\_CODE             & 34.48        & 20                                & 58                           & 24           & 2            & 7               & 8.60              \\
PROGRAMMING\_LANGUAGE                       & 34.45        & 955                               & 2772                         & 24           & 1            & 2               & 2.87              \\
VERSION, OPERATION\_SYSTEM                  & 34.29        & 12                                & 35                           & 24           & 3            & 6               & 8.34              \\
APPLICATION, VALUE                          & 34.21        & 13                                & 38                           & 24           & 3            & 7               & 8.37              \\
DEVICE, USER\_VARIABLE                      & 33.96        & 18                                & 53                           & 24           & 3            & 6               & 8.36              \\
LIBRARY\_FUNCTION                           & 33.85        & 110                               & 325                          & 22           & 2            & 5               & 5.58              \\
PROGRAMMING\_LANGUAGE, IN\_LINE\_CODE       & 33.59        & 86                                & 256                          & 24           & 2            & 5               & 5.63              \\
VERSION, ERROR\_NAME                        & 33.33        & 12                                & 36                           & 24           & 3            & 6               & 8.00              \\
VERSION, VALUE                              & 33.33        & 6                                 & 18                           & 24           & 5            & 11              & 12.83             \\
OPERATION\_SYSTEM, DATA\_STRUCTURE          & 33.33        & 12                                & 36                           & 24           & 3            & 5               & 8.69              \\
ERROR\_NAME, DATA\_TYPE                     & 33.33        & 6                                 & 18                           & 24           & 3            & 8               & 11.06             \\
DATA\_STRUCTURE, LIBRARY                    & 33.33        & 36                                & 108                          & 24           & 2            & 6               & 7.29              \\
DATA\_STRUCTURE, USER\_FUNCTION\_NAME       & 33.33        & 25                                & 75                           & 24           & 2            & 6               & 7.65              \\
LIBRARY\_FUNCTION, UI\_ELEMENT              & 33.33        & 5                                 & 15                           & 22           & 3            & 12              & 12.60             \\
LIBRARY\_FUNCTION, IN\_LINE\_CODE           & 33.33        & 26                                & 78                           & 22           & 3            & 7               & 7.72              \\
USER\_FUNCTION\_NAME, WEBSITE               & 33.33        & 5                                 & 15                           & 24           & 3            & 8               & 12.40             \\
ERROR\_NAME, LIBRARY\_FUNCTION              & 32.50        & 13                                & 40                           & 22           & 2            & 6.5             & 7.03              \\
IN\_LINE\_CODE                              & 32.38        & 102                               & 315                          & 24           & 1            & 5               & 5.24              \\
USER\_FUNCTION\_NAME, FILE\_NAME            & 32.35        & 11                                & 34                           & 24           & 3            & 7.5             & 9.44              \\
ALGORITHM, OPERATION\_SYSTEM                & 32.26        & 10                                & 31                           & 24           & 3            & 5               & 8.00              \\
DEVICE, FILE\_TYPE                          & 32.26        & 10                                & 31                           & 24           & 3            & 7               & 9.55              \\
PROGRAMMING\_LANGUAGE, USER\_VARIABLE       & 32.22        & 213                               & 661                          & 24           & 2            & 4               & 4.75              \\
PROGRAMMING\_LANGUAGE, ERROR\_NAME          & 32.16        & 55                                & 171                          & 24           & 2            & 5               & 5.41              \\
ALGORITHM, LIBRARY                          & 32.14        & 9                                 & 28                           & 24           & 4            & 6               & 9.29              \\
ALGORITHM, VALUE                            & 32.14        & 9                                 & 28                           & 24           & 3            & 7               & 9.07              \\
USER\_VARIABLE, OUTPUT\_BLOCK               & 31.82        & 7                                 & 22                           & 24           & 5            & 9               & 11.41             \\
ERROR\_NAME, FILE\_TYPE                     & 31.58        & 12                                & 38                           & 24           & 3            & 7               & 8.82              \\
USER\_NAME, WEBSITE                         & 31.58        & 6                                 & 19                           & 24           & 2            & 5               & 8.84              \\
ALGORITHM                                   & 31.25        & 40                                & 128                          & 24           & 1            & 4               & 5.16              \\
PROGRAMMING\_LANGUAGE, KEYBOARD\_INPUT      & 31.25        & 25                                & 80                           & 24           & 2            & 6               & 7.05              \\
USER\_NAME, UI\_ELEMENT                     & 31.25        & 5                                 & 16                           & 24           & 3            & 5               & 9.00              \\
LIBRARY, IN\_LINE\_CODE                     & 31.13        & 33                                & 106                          & 24           & 2            & 7               & 7.73              \\
OPERATION\_SYSTEM, FILE\_NAME               & 31.03        & 9                                 & 29                           & 24           & 3            & 6               & 8.86              \\
USER\_VARIABLE                              & 31.01        & 236                               & 761                          & 24           & 1            & 4               & 4.61              \\
PROGRAMMING\_LANGUAGE, ALGORITHM            & 31.00        & 31                                & 100                          & 24           & 2            & 5               & 5.69              \\
PROGRAMMING\_LANGUAGE, FILE\_TYPE           & 30.91        & 98                                & 317                          & 24           & 2            & 4               & 5.09              \\
ALGORITHM, FILE\_TYPE                       & 30.77        & 4                                 & 13                           & 24           & 3            & 13              & 12.15             \\
DATA\_STRUCTURE, LIBRARY\_FUNCTION          & 30.77        & 24                                & 78                           & 22           & 2            & 7               & 7.72              \\
VALUE, IN\_LINE\_CODE                       & 30.77        & 28                                & 91                           & 24           & 2            & 6               & 7.54              \\
PROGRAMMING\_LANGUAGE, FILE\_NAME           & 30.74        & 71                                & 231                          & 24           & 2            & 5               & 5.54              \\
USER\_VARIABLE, IN\_LINE\_CODE              & 30.66        & 42                                & 137                          & 24           & 2            & 5               & 6.64              \\
FILE\_NAME                                  & 30.50        & 79                                & 259                          & 24           & 1            & 5               & 5.37              \\
USER\_VARIABLE, KEYBOARD\_INPUT             & 30.43        & 14                                & 46                           & 24           & 2            & 6               & 8.61              \\
PROGRAMMING\_LANGUAGE, LIBRARY              & 30.40        & 176                               & 579                          & 24           & 2            & 4               & 4.77              \\
USER\_VARIABLE, LIBRARY\_FUNCTION           & 30.36        & 51                                & 168                          & 22           & 3            & 6               & 6.43              \\
LIBRARY, FILE\_TYPE                         & 30.28        & 33                                & 109                          & 24           & 2            & 6               & 7.43              \\
ALGORITHM, USER\_NAME                       & 30.00        & 3                                 & 10                           & 24           & 2            & 5.5             & 9.50              \\
ERROR\_NAME, OUTPUT\_BLOCK                  & 30.00        & 3                                 & 10                           & 24           & 6            & 18              & 15.80             \\
USER\_NAME, IN\_LINE\_CODE                  & 30.00        & 9                                 & 30                           & 24           & 3            & 4               & 6.70              \\
ERROR\_NAME                                 & 29.86        & 63                                & 211                          & 24           & 1            & 4               & 4.91              \\
PROGRAMMING\_LANGUAGE, WEBSITE              & 29.85        & 20                                & 67                           & 24           & 2            & 4               & 6.45              \\
LIBRARY\_FUNCTION, USER\_FUNCTION\_NAME     & 29.85        & 20                                & 67                           & 22           & 3            & 7               & 7.78              \\
LIBRARY                                     & 29.84        & 191                               & 640                          & 24           & 1            & 4               & 4.62              \\
KEYBOARD\_INPUT                             & 29.81        & 31                                & 104                          & 24           & 1            & 5               & 6.33              \\
APPLICATION, IN\_LINE\_CODE                 & 29.73        & 11                                & 37                           & 24           & 3            & 6               & 7.97              \\
OPERATION\_SYSTEM, FILE\_TYPE               & 29.73        & 11                                & 37                           & 24           & 2            & 5               & 7.51              \\
FILE\_TYPE                                  & 29.54        & 109                               & 369                          & 24           & 1            & 4               & 4.90              \\
IN\_LINE\_CODE, KEYBOARD\_INPUT             & 29.41        & 10                                & 34                           & 24           & 2            & 8               & 10.15             \\
ALGORITHM, USER\_VARIABLE                   & 29.27        & 12                                & 41                           & 24           & 3            & 6               & 8.29              \\
ERROR\_NAME, KEYBOARD\_INPUT                & 29.17        & 7                                 & 24                           & 24           & 2            & 7               & 10.04             \\
OPERATION\_SYSTEM                           & 29.13        & 74                                & 254                          & 24           & 1            & 3.5             & 4.23              \\
PROGRAMMING\_LANGUAGE, USER\_NAME           & 29.06        & 59                                & 203                          & 24           & 2            & 4               & 4.19              \\
APPLICATION, PROGRAMMING\_LANGUAGE          & 28.64        & 122                               & 426                          & 24           & 2            & 3               & 3.79              \\
OPERATION\_SYSTEM, LIBRARY                  & 28.57        & 14                                & 49                           & 24           & 2            & 6               & 7.92              \\
LIBRARY, USER\_VARIABLE                     & 28.50        & 59                                & 207                          & 24           & 2            & 6               & 6.47              \\
PROGRAMMING\_LANGUAGE, VALUE                & 28.32        & 64                                & 226                          & 24           & 2            & 5               & 5.87              \\
APPLICATION                                 & 28.18        & 173                               & 614                          & 24           & 1            & 3               & 3.26              \\
USER\_NAME                                  & 28.09        & 75                                & 267                          & 24           & 1            & 3               & 3.79              \\
VALUE                                       & 27.99        & 75                                & 268                          & 24           & 1            & 5               & 5.59              \\
LIBRARY\_FUNCTION, FILE\_TYPE               & 27.94        & 19                                & 68                           & 22           & 2            & 7               & 7.93              \\
APPLICATION, UI\_ELEMENT                    & 27.78        & 5                                 & 18                           & 24           & 2            & 6               & 8.33              \\
VALUE, KEYBOARD\_INPUT                      & 27.59        & 8                                 & 29                           & 24           & 4            & 9               & 11.10             \\
ERROR\_NAME, LIBRARY                        & 27.38        & 23                                & 84                           & 24           & 2            & 6               & 6.89              \\
APPLICATION, DEVICE                         & 27.27        & 12                                & 44                           & 24           & 2            & 5               & 6.43              \\
PROGRAMMING\_LANGUAGE, OPERATION\_SYSTEM    & 27.22        & 49                                & 180                          & 24           & 2            & 4               & 4.77              \\
USER\_FUNCTION\_NAME, FILE\_TYPE            & 27.14        & 19                                & 70                           & 24           & 3            & 6               & 7.73              \\
USER\_FUNCTION\_NAME, IN\_LINE\_CODE        & 27.12        & 16                                & 59                           & 24           & 3            & 7               & 8.29              \\
LIBRARY, USER\_FUNCTION\_NAME               & 27.00        & 27                                & 100                          & 24           & 3            & 6               & 7.45              \\
LIBRARY\_FUNCTION, KEYBOARD\_INPUT          & 26.92        & 7                                 & 26                           & 22           & 3            & 7               & 9.62              \\
ERROR\_NAME, VALUE                          & 26.83        & 11                                & 41                           & 24           & 3            & 7               & 8.39              \\
USER\_FUNCTION\_NAME, VALUE                 & 26.76        & 19                                & 71                           & 24           & 2            & 6               & 7.70              \\
APPLICATION, LIBRARY\_CLASS                 & 26.67        & 4                                 & 15                           & 24           & 4            & 11              & 12.00             \\
LIBRARY\_FUNCTION, VALUE                    & 26.67        & 20                                & 75                           & 22           & 3            & 7               & 7.73              \\
FILE\_TYPE, WEBSITE                         & 26.67        & 4                                 & 15                           & 24           & 3            & 11              & 12.07             \\
DATA\_TYPE, USER\_FUNCTION\_NAME            & 26.47        & 18                                & 68                           & 24           & 2            & 7               & 8.00              \\
FILE\_NAME, IN\_LINE\_CODE                  & 26.47        & 18                                & 68                           & 24           & 2            & 7               & 7.71              \\
WEBSITE                                     & 26.44        & 23                                & 87                           & 24           & 1            & 4               & 5.76              \\
ERROR\_NAME, FILE\_NAME                     & 26.09        & 12                                & 46                           & 24           & 3            & 6               & 7.61              \\
FILE\_NAME, KEYBOARD\_INPUT                 & 26.09        & 6                                 & 23                           & 24           & 3            & 10              & 11.17             \\
FILE\_TYPE, IN\_LINE\_CODE                  & 26.03        & 19                                & 73                           & 24           & 3            & 7               & 7.68              \\
USER\_NAME, USER\_FUNCTION\_NAME            & 26.00        & 13                                & 50                           & 24           & 2            & 5               & 6.18              \\
APPLICATION, OPERATION\_SYSTEM              & 25.81        & 16                                & 62                           & 24           & 2            & 4               & 4.82              \\
LIBRARY, VALUE                              & 25.81        & 24                                & 93                           & 24           & 3            & 7               & 7.91              \\
APPLICATION, FILE\_TYPE                     & 25.76        & 17                                & 66                           & 24           & 2            & 5               & 6.06              \\
PROGRAMMING\_LANGUAGE, USER\_FUNCTION\_NAME & 25.75        & 77                                & 299                          & 24           & 2            & 5               & 5.46              \\
ALGORITHM, DATA\_STRUCTURE                  & 25.71        & 9                                 & 35                           & 24           & 2            & 6               & 8.43              \\
USER\_NAME, LIBRARY                         & 25.53        & 12                                & 47                           & 24           & 3            & 5               & 6.45              \\
USER\_VARIABLE, VALUE                       & 25.36        & 35                                & 138                          & 24           & 2            & 6               & 6.89              \\
LIBRARY, FILE\_NAME                         & 25.30        & 21                                & 83                           & 24           & 3            & 7               & 8.08              \\
APPLICATION, KEYBOARD\_INPUT                & 25.00        & 3                                 & 12                           & 24           & 2            & 9.5             & 10.83             \\
ALGORITHM, DATA\_TYPE                       & 25.00        & 8                                 & 32                           & 24           & 2            & 5.5             & 8.44              \\
ALGORITHM, KEYBOARD\_INPUT                  & 25.00        & 4                                 & 16                           & 24           & 2            & 8               & 11.38             \\
DATA\_STRUCTURE, VALUE                      & 25.00        & 17                                & 68                           & 24           & 2            & 7               & 7.90              \\
LIBRARY, UI\_ELEMENT                        & 25.00        & 6                                 & 24                           & 24           & 3            & 8.5             & 10.96             \\
DATA\_TYPE, VALUE                           & 24.56        & 14                                & 57                           & 24           & 2            & 7               & 8.54              \\
USER\_FUNCTION\_NAME                        & 24.50        & 86                                & 351                          & 24           & 1            & 5               & 5.19              \\
USER\_VARIABLE, USER\_FUNCTION\_NAME        & 24.42        & 63                                & 258                          & 24           & 2            & 5               & 5.67              \\
APPLICATION, LIBRARY                        & 24.30        & 26                                & 107                          & 24           & 2            & 5               & 5.79              \\
USER\_VARIABLE, FILE\_NAME                  & 24.18        & 22                                & 91                           & 24           & 2            & 6               & 7.51              \\
ALGORITHM, USER\_FUNCTION\_NAME             & 24.00        & 6                                 & 25                           & 24           & 2            & 7               & 9.60              \\
FILE\_TYPE, UI\_ELEMENT                     & 24.00        & 6                                 & 25                           & 24           & 3            & 8               & 10.16             \\
USER\_FUNCTION\_NAME, UI\_ELEMENT           & 23.81        & 5                                 & 21                           & 24           & 4            & 7               & 10.90             \\
FILE\_NAME, WEBSITE                         & 23.81        & 5                                 & 21                           & 24           & 4            & 9               & 11.00             \\
UI\_ELEMENT, VALUE                          & 23.81        & 5                                 & 21                           & 24           & 3            & 8               & 11.10             \\
USER\_NAME, FILE\_TYPE                      & 23.33        & 7                                 & 30                           & 24           & 2            & 5               & 6.77              \\
APPLICATION, DATA\_TYPE                     & 23.08        & 9                                 & 39                           & 24           & 3            & 6               & 8.26              \\
LIBRARY, KEYBOARD\_INPUT                    & 23.08        & 9                                 & 39                           & 24           & 3            & 7               & 9.97              \\
APPLICATION, LIBRARY\_FUNCTION              & 22.45        & 11                                & 49                           & 17           & 3            & 7               & 7.47              \\
USER\_VARIABLE, FILE\_TYPE                  & 22.45        & 33                                & 147                          & 24           & 3            & 5               & 6.42              \\
APPLICATION, USER\_VARIABLE                 & 22.41        & 26                                & 116                          & 24           & 2            & 5               & 5.67              \\
USER\_VARIABLE, WEBSITE                     & 22.22        & 6                                 & 27                           & 24           & 3            & 6               & 9.70              \\
FILE\_NAME, VALUE                           & 22.22        & 12                                & 54                           & 24           & 2            & 8               & 8.69              \\
USER\_VARIABLE, UI\_ELEMENT                 & 21.88        & 7                                 & 32                           & 24           & 3            & 6               & 8.81              \\
LIBRARY\_FUNCTION, FILE\_NAME               & 21.82        & 12                                & 55                           & 22           & 3            & 8               & 8.45              \\
LIBRARY\_CLASS, VALUE                       & 21.74        & 5                                 & 23                           & 24           & 4            & 9               & 11.70             \\
FILE\_TYPE, VALUE                           & 21.74        & 10                                & 46                           & 24           & 3            & 8               & 9.61              \\
APPLICATION, ERROR\_NAME                    & 21.43        & 6                                 & 28                           & 24           & 2            & 5.5             & 6.75              \\
UI\_ELEMENT                                 & 20.48        & 17                                & 83                           & 24           & 1            & 4               & 6.07              \\
ERROR\_NAME, IN\_LINE\_CODE                 & 20.45        & 9                                 & 44                           & 24           & 2            & 7               & 8.48              \\
APPLICATION, USER\_NAME                     & 18.75        & 12                                & 64                           & 24           & 2            & 4               & 4.80              \\
PROGRAMMING\_LANGUAGE, UI\_ELEMENT          & 18.06        & 13                                & 72                           & 24           & 2            & 4               & 6.26              \\
FILE\_TYPE, KEYBOARD\_INPUT                 & 17.65        & 6                                 & 34                           & 24           & 2            & 7               & 9.91              \\
LIBRARY, WEBSITE                            & 17.14        & 6                                 & 35                           & 24           & 2            & 5               & 8.91              \\
APPLICATION, USER\_FUNCTION\_NAME           & 16.95        & 10                                & 59                           & 24           & 3            & 5               & 6.73             
\end{tabular}
\end{table}

==> tablets/intent_CONCEPTUAL_upto2_combinations_success_rate.tex <==
\begin{table}
\centering
\caption{Entity Combinations in CONCEPTUAL intent}
\label{tab:intent_CONCEPTUAL_upto2_combinations_success_rate}

\begin{tabular}{llllllll}
Entities Combination                        & Success Rate & Number of Successful Combinations & Total Number of Combinations & Max Entities & Min Entities & Median Entities & Average Entities  \\
DATA\_STRUCTURE, LIBRARY\_VARIABLE          & 42.11        & 8                                 & 19                           & 24           & 4            & 9               & 12.32             \\
VERSION, LIBRARY\_VARIABLE                  & 41.67        & 5                                 & 12                           & 24           & 3            & 15              & 14.17             \\
USER\_NAME, HTML\_TAG\_NAME                 & 41.67        & 5                                 & 12                           & 24           & 2            & 22.5            & 17.50             \\
APPLICATION, LIBRARY\_CLASS                 & 40.00        & 10                                & 25                           & 24           & 4            & 9               & 12.20             \\
LIBRARY, LIBRARY\_VARIABLE                  & 40.00        & 10                                & 25                           & 24           & 4            & 9               & 11.56             \\
APPLICATION, IN\_LINE\_CODE                 & 38.64        & 17                                & 44                           & 24           & 4            & 7               & 9.25              \\
UI\_ELEMENT, HTML\_TAG\_NAME                & 38.46        & 10                                & 26                           & 24           & 3            & 17.5            & 15.23             \\
VERSION, LIBRARY\_CLASS                     & 38.24        & 13                                & 34                           & 24           & 7            & 14              & 14.88             \\
ERROR\_NAME, DATA\_TYPE                     & 37.84        & 28                                & 74                           & 24           & 2            & 7.5             & 9.09              \\
DATA\_TYPE, LIBRARY\_VARIABLE               & 36.84        & 7                                 & 19                           & 24           & 2            & 9               & 12.21             \\
APPLICATION, LIBRARY\_FUNCTION              & 36.51        & 23                                & 63                           & 24           & 2            & 7               & 7.95              \\
VERSION, FILE\_NAME                         & 36.51        & 23                                & 63                           & 24           & 3            & 8               & 10.38             \\
USER\_NAME, KEYBOARD\_INPUT                 & 36.00        & 9                                 & 25                           & 24           & 3            & 7               & 11.44             \\
LIBRARY\_VARIABLE, FILE\_NAME               & 35.71        & 5                                 & 14                           & 24           & 7            & 12.5            & 13.57             \\
ERROR\_NAME, WEBSITE                        & 35.29        & 6                                 & 17                           & 24           & 3            & 18              & 15.00             \\
LIBRARY\_VARIABLE, FILE\_TYPE               & 35.29        & 6                                 & 17                           & 24           & 6            & 9               & 12.47             \\
ERROR\_NAME, LIBRARY\_CLASS                 & 35.14        & 13                                & 37                           & 24           & 3            & 11              & 12.68             \\
OPERATION\_SYSTEM, IN\_LINE\_CODE           & 34.88        & 15                                & 43                           & 24           & 2            & 7               & 10.77             \\
VERSION, LIBRARY                            & 34.48        & 40                                & 116                          & 24           & 2            & 7               & 8.08              \\
USER\_NAME, DATA\_STRUCTURE                 & 34.33        & 23                                & 67                           & 24           & 2            & 5               & 7.27              \\
PROGRAMMING\_LANGUAGE, LIBRARY\_VARIABLE    & 33.33        & 12                                & 36                           & 24           & 2            & 8               & 10.08             \\
APPLICATION, VALUE                          & 32.35        & 22                                & 68                           & 24           & 3            & 6               & 7.74              \\
HTML\_TAG\_NAME                             & 32.26        & 20                                & 62                           & 24           & 1            & 6               & 9.13              \\
VERSION, DATA\_STRUCTURE                    & 32.26        & 20                                & 62                           & 24           & 3            & 8.5             & 10.55             \\
USER\_VARIABLE, HTML\_TAG\_NAME             & 32.26        & 10                                & 31                           & 24           & 2            & 14              & 13.52             \\
ERROR\_NAME, LIBRARY\_FUNCTION              & 32.14        & 27                                & 84                           & 24           & 3            & 8               & 8.67              \\
VERSION, DEVICE                             & 32.00        & 16                                & 50                           & 24           & 2            & 8.5             & 11.40             \\
ERROR\_NAME, DATA\_STRUCTURE                & 31.88        & 22                                & 69                           & 24           & 3            & 8               & 9.72              \\
PROGRAMMING\_LANGUAGE, DATA\_STRUCTURE      & 31.62        & 264                               & 835                          & 24           & 2            & 4               & 4.85              \\
ALGORITHM, ERROR\_NAME                      & 31.03        & 9                                 & 29                           & 24           & 2            & 7               & 11.34             \\
VERSION, LIBRARY\_FUNCTION                  & 30.56        & 22                                & 72                           & 24           & 3            & 8               & 9.42              \\
LIBRARY\_VARIABLE                           & 30.00        & 12                                & 40                           & 24           & 2            & 8               & 9.68              \\
DEVICE, USER\_CLASS                         & 30.00        & 3                                 & 10                           & 24           & 12           & 19              & 19.40             \\
LIBRARY\_VARIABLE, OUTPUT\_BLOCK            & 30.00        & 3                                 & 10                           & 22           & 6            & 17              & 15.70             \\
OPERATION\_SYSTEM, FILE\_TYPE               & 29.82        & 17                                & 57                           & 24           & 2            & 7               & 9.39              \\
DEVICE, LIBRARY\_FUNCTION                   & 29.55        & 13                                & 44                           & 24           & 3            & 8.5             & 10.61             \\
OPERATION\_SYSTEM, OUTPUT\_BLOCK            & 29.41        & 5                                 & 17                           & 24           & 3            & 18              & 17.41             \\
WEBSITE, KEYBOARD\_INPUT                    & 29.41        & 5                                 & 17                           & 24           & 2            & 20              & 16.53             \\
VERSION, FILE\_TYPE                         & 29.23        & 19                                & 65                           & 24           & 2            & 9               & 10.77             \\
LIBRARY, LIBRARY\_FUNCTION                  & 29.21        & 111                               & 380                          & 24           & 2            & 6               & 6.68              \\
OPERATION\_SYSTEM, LIBRARY\_CLASS           & 29.17        & 7                                 & 24                           & 24           & 5            & 16              & 15.83             \\
DATA\_STRUCTURE, HTML\_TAG\_NAME            & 29.17        & 7                                 & 24                           & 24           & 3            & 18.5            & 16.29             \\
DATA\_STRUCTURE, FILE\_NAME                 & 29.03        & 27                                & 93                           & 24           & 2            & 9               & 9.58              \\
PROGRAMMING\_LANGUAGE, HTML\_TAG\_NAME      & 28.89        & 13                                & 45                           & 24           & 2            & 8               & 10.96             \\
DATA\_TYPE, LIBRARY\_FUNCTION               & 28.65        & 55                                & 192                          & 24           & 3            & 7               & 7.67              \\
ERROR\_NAME, HTML\_TAG\_NAME                & 28.57        & 4                                 & 14                           & 24           & 6            & 22.5            & 19.71             \\
LIBRARY\_CLASS, HTML\_TAG\_NAME             & 28.57        & 6                                 & 21                           & 24           & 4            & 19              & 17.81             \\
LIBRARY\_VARIABLE, LIBRARY\_FUNCTION        & 28.57        & 8                                 & 28                           & 24           & 4            & 8.5             & 10.96             \\
DATA\_STRUCTURE                             & 28.41        & 317                               & 1116                         & 24           & 1            & 4               & 4.29              \\
OPERATION\_SYSTEM, DATA\_STRUCTURE          & 28.33        & 17                                & 60                           & 24           & 2            & 6               & 9.07              \\
DATA\_STRUCTURE, LIBRARY\_FUNCTION          & 28.31        & 62                                & 219                          & 24           & 3            & 7               & 7.57              \\
PROGRAMMING\_LANGUAGE, LIBRARY\_FUNCTION    & 28.03        & 178                               & 635                          & 24           & 2            & 5               & 5.78              \\
DEVICE, USER\_NAME                          & 28.00        & 7                                 & 25                           & 24           & 2            & 9               & 12.08             \\
USER\_NAME, IN\_LINE\_CODE                  & 28.00        & 14                                & 50                           & 24           & 2            & 5               & 8.14              \\
PROGRAMMING\_LANGUAGE, LIBRARY\_CLASS       & 27.96        & 52                                & 186                          & 24           & 2            & 6               & 7.57              \\
LIBRARY\_FUNCTION                           & 27.90        & 195                               & 699                          & 24           & 1            & 5               & 5.65              \\
LIBRARY, LIBRARY\_CLASS                     & 27.81        & 47                                & 169                          & 24           & 2            & 7               & 7.80              \\
OPERATION\_SYSTEM, FILE\_NAME               & 27.78        & 10                                & 36                           & 24           & 3            & 10              & 12.28             \\
LIBRARY\_CLASS, FILE\_TYPE                  & 27.54        & 19                                & 69                           & 24           & 4            & 10              & 11.52             \\
APPLICATION, LIBRARY                        & 27.52        & 41                                & 149                          & 24           & 2            & 5               & 5.91              \\
USER\_NAME, FILE\_TYPE                      & 27.45        & 14                                & 51                           & 24           & 2            & 7               & 8.75              \\
LIBRARY\_FUNCTION, FILE\_NAME               & 27.35        & 32                                & 117                          & 24           & 4            & 8               & 9.21              \\
VERSION, ERROR\_NAME                        & 27.27        & 15                                & 55                           & 24           & 2            & 8               & 10.05             \\
USER\_CLASS, KEYBOARD\_INPUT                & 27.27        & 3                                 & 11                           & 24           & 5            & 20              & 17.18             \\
WEBSITE, OUTPUT\_BLOCK                      & 27.27        & 3                                 & 11                           & 24           & 16           & 23              & 21.36             \\
DATA\_STRUCTURE, LIBRARY                    & 27.21        & 77                                & 283                          & 24           & 2            & 6               & 7.13              \\
LIBRARY, FILE\_NAME                         & 27.13        & 51                                & 188                          & 24           & 2            & 7               & 8.22              \\
LIBRARY\_CLASS, USER\_FUNCTION\_NAME        & 27.12        & 16                                & 59                           & 24           & 3            & 10              & 11.31             \\
ALGORITHM, DEVICE                           & 26.92        & 7                                 & 26                           & 24           & 3            & 9               & 12.69             \\
UI\_ELEMENT, KEYBOARD\_INPUT                & 26.92        & 7                                 & 26                           & 24           & 2            & 18              & 15.35             \\
DATA\_STRUCTURE, FILE\_TYPE                 & 26.85        & 40                                & 149                          & 24           & 2            & 7               & 8.39              \\
ALGORITHM, DATA\_TYPE                       & 26.83        & 22                                & 82                           & 24           & 2            & 6               & 7.76              \\
LIBRARY\_CLASS, LIBRARY\_FUNCTION           & 26.73        & 27                                & 101                          & 24           & 3            & 8               & 9.12              \\
APPLICATION, OUTPUT\_BLOCK                  & 26.67        & 4                                 & 15                           & 24           & 3            & 8               & 13.20             \\
OPERATION\_SYSTEM, HTML\_TAG\_NAME          & 26.67        & 4                                 & 15                           & 24           & 5            & 22              & 19.20             \\
USER\_NAME, OUTPUT\_BLOCK                   & 26.67        & 4                                 & 15                           & 24           & 3            & 18              & 14.93             \\
LIBRARY\_VARIABLE, VALUE                    & 26.67        & 4                                 & 15                           & 24           & 4            & 14              & 13.80             \\
LIBRARY\_CLASS                              & 26.60        & 54                                & 203                          & 24           & 1            & 6               & 7.42              \\
ERROR\_NAME, USER\_VARIABLE                 & 26.59        & 46                                & 173                          & 24           & 2            & 5               & 6.82              \\
ERROR\_NAME, FILE\_TYPE                     & 26.51        & 22                                & 83                           & 24           & 3            & 7               & 9.27              \\
DATA\_STRUCTURE, DATA\_TYPE                 & 26.50        & 75                                & 283                          & 24           & 2            & 6               & 6.83              \\
APPLICATION, DATA\_TYPE                     & 26.39        & 19                                & 72                           & 24           & 2            & 6               & 7.69              \\
DATA\_TYPE, FILE\_NAME                      & 26.39        & 19                                & 72                           & 24           & 3            & 9               & 10.47             \\
VERSION, USER\_VARIABLE                     & 26.37        & 24                                & 91                           & 24           & 2            & 7               & 9.10              \\
APPLICATION, DATA\_STRUCTURE                & 26.32        & 35                                & 133                          & 24           & 2            & 5               & 6.13              \\
OPERATION\_SYSTEM, DATA\_TYPE               & 26.32        & 15                                & 57                           & 24           & 3            & 6               & 9.81              \\
DATA\_TYPE, USER\_CLASS                     & 26.32        & 5                                 & 19                           & 24           & 3            & 14              & 13.32             \\
LIBRARY\_CLASS, LIBRARY\_VARIABLE           & 26.32        & 5                                 & 19                           & 24           & 8            & 14              & 14.11             \\
USER\_FUNCTION\_NAME, HTML\_TAG\_NAME       & 26.32        & 5                                 & 19                           & 24           & 5            & 17              & 16.53             \\
PROGRAMMING\_LANGUAGE, DATA\_TYPE           & 26.29        & 153                               & 582                          & 24           & 2            & 4               & 5.31              \\
ERROR\_NAME, LIBRARY                        & 26.27        & 31                                & 118                          & 24           & 3            & 7               & 8.23              \\
OPERATION\_SYSTEM, USER\_NAME               & 25.93        & 7                                 & 27                           & 24           & 2            & 5               & 10.07             \\
LIBRARY, HTML\_TAG\_NAME                    & 25.93        & 7                                 & 27                           & 24           & 2            & 16              & 14.93             \\
PROGRAMMING\_LANGUAGE, VERSION              & 25.91        & 71                                & 274                          & 24           & 2            & 4               & 5.68              \\
DATA\_TYPE, IN\_LINE\_CODE                  & 25.90        & 36                                & 139                          & 24           & 2            & 7               & 8.22              \\
FILE\_TYPE, FILE\_NAME                      & 25.81        & 64                                & 248                          & 24           & 2            & 7               & 7.49              \\
APPLICATION, VERSION                        & 25.68        & 19                                & 74                           & 24           & 2            & 5               & 7.22              \\
PROGRAMMING\_LANGUAGE, ERROR\_NAME          & 25.56        & 92                                & 360                          & 24           & 2            & 4               & 5.29              \\
DATA\_TYPE                                  & 25.52        & 198                               & 776                          & 24           & 1            & 4               & 4.76              \\
USER\_VARIABLE, LIBRARY\_FUNCTION           & 25.42        & 91                                & 358                          & 24           & 2            & 6               & 6.82              \\
OPERATION\_SYSTEM, LIBRARY                  & 25.33        & 19                                & 75                           & 24           & 3            & 6               & 8.51              \\
ERROR\_NAME, VALUE                          & 25.24        & 26                                & 103                          & 24           & 2            & 6               & 7.76              \\
VERSION, OPERATION\_SYSTEM                  & 25.00        & 16                                & 64                           & 24           & 2            & 7               & 9.13              \\
VERSION, DATA\_TYPE                         & 25.00        & 14                                & 56                           & 24           & 3            & 9               & 11.16             \\
VERSION, USER\_CLASS                        & 25.00        & 3                                 & 12                           & 24           & 5            & 19              & 18.08             \\
OPERATION\_SYSTEM, DEVICE                   & 25.00        & 19                                & 76                           & 24           & 2            & 6               & 8.74              \\
OPERATION\_SYSTEM, ERROR\_NAME              & 25.00        & 12                                & 48                           & 24           & 2            & 7               & 9.79              \\
LIBRARY\_CLASS, USER\_CLASS                 & 25.00        & 3                                 & 12                           & 24           & 10           & 19              & 18.58             \\
LIBRARY\_CLASS, UI\_ELEMENT                 & 25.00        & 7                                 & 28                           & 24           & 4            & 17.5            & 16.32             \\
LIBRARY\_CLASS, WEBSITE                     & 25.00        & 4                                 & 16                           & 24           & 4            & 21              & 18.81             \\
USER\_CLASS, OUTPUT\_BLOCK                  & 25.00        & 3                                 & 12                           & 24           & 6            & 19              & 17.50             \\
LIBRARY\_FUNCTION, HTML\_TAG\_NAME          & 25.00        & 5                                 & 20                           & 24           & 5            & 17              & 16.10             \\
FILE\_NAME, KEYBOARD\_INPUT                 & 25.00        & 9                                 & 36                           & 24           & 3            & 11              & 12.97             \\
DATA\_TYPE, LIBRARY                         & 24.87        & 48                                & 193                          & 24           & 3            & 7               & 7.86              \\
VERSION                                     & 24.86        & 89                                & 358                          & 24           & 1            & 4               & 4.97              \\
LIBRARY, VALUE                              & 24.71        & 42                                & 170                          & 24           & 2            & 7               & 8.21              \\
LIBRARY\_FUNCTION, FILE\_TYPE               & 24.71        & 42                                & 170                          & 24           & 3            & 7               & 8.31              \\
DATA\_STRUCTURE, LIBRARY\_CLASS             & 24.64        & 17                                & 69                           & 24           & 4            & 9               & 10.96             \\
DEVICE, DATA\_TYPE                          & 24.56        & 14                                & 57                           & 24           & 2            & 8               & 10.84             \\
ERROR\_NAME                                 & 24.55        & 124                               & 505                          & 24           & 1            & 4               & 4.48              \\
DEVICE, DATA\_STRUCTURE                     & 24.53        & 13                                & 53                           & 24           & 2            & 8               & 11.08             \\
LIBRARY\_CLASS, FILE\_NAME                  & 24.53        & 13                                & 53                           & 24           & 5            & 10              & 12.43             \\
FILE\_NAME                                  & 24.49        & 119                               & 486                          & 24           & 1            & 5               & 5.68              \\
PROGRAMMING\_LANGUAGE, LIBRARY              & 24.44        & 249                               & 1019                         & 24           & 2            & 4               & 4.96              \\
LIBRARY, FILE\_TYPE                         & 24.28        & 59                                & 243                          & 24           & 3            & 7               & 7.84              \\
LIBRARY\_FUNCTION, VALUE                    & 24.28        & 42                                & 173                          & 24           & 2            & 7               & 7.65              \\
PROGRAMMING\_LANGUAGE, FILE\_NAME           & 24.24        & 104                               & 429                          & 24           & 2            & 5               & 5.90              \\
PROGRAMMING\_LANGUAGE                       & 24.06        & 1682                              & 6992                         & 24           & 1            & 2               & 2.51              \\
DEVICE, LIBRARY\_CLASS                      & 24.00        & 6                                 & 25                           & 24           & 3            & 18              & 16.36             \\
LIBRARY\_CLASS, USER\_VARIABLE              & 24.00        & 24                                & 100                          & 24           & 3            & 8               & 9.70              \\
LIBRARY\_CLASS, OUTPUT\_BLOCK               & 24.00        & 6                                 & 25                           & 24           & 8            & 18              & 16.64             \\
LIBRARY\_CLASS, KEYBOARD\_INPUT             & 24.00        & 6                                 & 25                           & 24           & 5            & 18              & 16.60             \\
LIBRARY\_VARIABLE, USER\_VARIABLE           & 24.00        & 6                                 & 25                           & 24           & 3            & 9               & 10.96             \\
FILE\_NAME, HTML\_TAG\_NAME                 & 24.00        & 6                                 & 25                           & 24           & 2            & 16              & 14.96             \\
LIBRARY                                     & 23.97        & 273                               & 1139                         & 24           & 1            & 4               & 4.80              \\
USER\_NAME, DATA\_TYPE                      & 23.91        & 11                                & 46                           & 24           & 2            & 5               & 8.67              \\
VERSION, USER\_FUNCTION\_NAME               & 23.81        & 10                                & 42                           & 24           & 3            & 10.5            & 11.55             \\
VERSION, UI\_ELEMENT                        & 23.81        & 5                                 & 21                           & 24           & 4            & 19              & 16.67             \\
FILE\_TYPE, HTML\_TAG\_NAME                 & 23.81        & 5                                 & 21                           & 24           & 6            & 19              & 17.00             \\
APPLICATION, FILE\_TYPE                     & 23.66        & 22                                & 93                           & 24           & 2            & 6               & 7.08              \\
LIBRARY\_VARIABLE, USER\_FUNCTION\_NAME     & 23.53        & 4                                 & 17                           & 24           & 4            & 11              & 12.18             \\
PROGRAMMING\_LANGUAGE, FILE\_TYPE           & 23.51        & 126                               & 536                          & 24           & 2            & 5               & 5.78              \\
FILE\_TYPE                                  & 23.44        & 147                               & 627                          & 24           & 1            & 5               & 5.48              \\
USER\_NAME, FILE\_NAME                      & 23.40        & 11                                & 47                           & 24           & 2            & 5               & 8.45              \\
DEVICE, LIBRARY                             & 23.38        & 18                                & 77                           & 24           & 3            & 8               & 9.58              \\
DATA\_STRUCTURE, USER\_FUNCTION\_NAME       & 23.36        & 50                                & 214                          & 24           & 2            & 6               & 7.08              \\
DEVICE, KEYBOARD\_INPUT                     & 23.33        & 7                                 & 30                           & 24           & 3            & 14              & 13.80             \\
ERROR\_NAME, FILE\_NAME                     & 23.33        & 21                                & 90                           & 24           & 2            & 7               & 8.78              \\
ALGORITHM, DATA\_STRUCTURE                  & 23.15        & 25                                & 108                          & 24           & 2            & 5               & 6.88              \\
VERSION, KEYBOARD\_INPUT                    & 23.08        & 6                                 & 26                           & 24           & 3            & 16.5            & 15.04             \\
OPERATION\_SYSTEM, LIBRARY\_FUNCTION        & 23.08        & 12                                & 52                           & 24           & 2            & 6               & 8.88              \\
DEVICE, WEBSITE                             & 23.08        & 3                                 & 13                           & 24           & 8            & 23              & 20.23             \\
USER\_NAME, LIBRARY\_FUNCTION               & 23.08        & 9                                 & 39                           & 24           & 3            & 7               & 9.23              \\
USER\_NAME, UI\_ELEMENT                     & 23.08        & 6                                 & 26                           & 24           & 2            & 7.5             & 11.50             \\
DATA\_TYPE, OUTPUT\_BLOCK                   & 23.08        & 9                                 & 39                           & 24           & 5            & 10              & 12.92             \\
DATA\_STRUCTURE, USER\_VARIABLE             & 22.99        & 103                               & 448                          & 24           & 2            & 5               & 5.99              \\
DATA\_TYPE, USER\_VARIABLE                  & 22.93        & 72                                & 314                          & 24           & 2            & 6               & 6.55              \\
FILE\_TYPE, KEYBOARD\_INPUT                 & 22.92        & 11                                & 48                           & 24           & 2            & 8               & 11.40             \\
PROGRAMMING\_LANGUAGE, IN\_LINE\_CODE       & 22.81        & 117                               & 513                          & 24           & 2            & 5               & 5.50              \\
USER\_FUNCTION\_NAME, FILE\_NAME            & 22.77        & 23                                & 101                          & 24           & 3            & 8               & 9.39              \\
IN\_LINE\_CODE                              & 22.73        & 153                               & 673                          & 24           & 1            & 4               & 5.00              \\
VERSION, OUTPUT\_BLOCK                      & 22.73        & 5                                 & 22                           & 24           & 5            & 18              & 16.23             \\
ERROR\_NAME, UI\_ELEMENT                    & 22.73        & 5                                 & 22                           & 24           & 5            & 18.5            & 15.55             \\
WEBSITE, IN\_LINE\_CODE                     & 22.73        & 5                                 & 22                           & 24           & 2            & 17              & 13.86             \\
HTML\_TAG\_NAME, IN\_LINE\_CODE             & 22.73        & 5                                 & 22                           & 24           & 5            & 19              & 16.77             \\
USER\_FUNCTION\_NAME, FILE\_TYPE            & 22.58        & 28                                & 124                          & 24           & 3            & 8               & 9.10              \\
VERSION, IN\_LINE\_CODE                     & 22.22        & 12                                & 54                           & 24           & 3            & 8               & 10.70             \\
DEVICE, HTML\_TAG\_NAME                     & 22.22        & 4                                 & 18                           & 24           & 5            & 19.5            & 18.61             \\
DEVICE, IN\_LINE\_CODE                      & 22.22        & 10                                & 45                           & 24           & 3            & 8               & 11.89             \\
DATA\_STRUCTURE, WEBSITE                    & 22.22        & 6                                 & 27                           & 24           & 2            & 8               & 12.85             \\
WEBSITE, HTML\_TAG\_NAME                    & 22.22        & 4                                 & 18                           & 24           & 4            & 19              & 16.89             \\
HTML\_TAG\_NAME, OUTPUT\_BLOCK              & 22.22        & 4                                 & 18                           & 24           & 8            & 19.5            & 18.44             \\
LIBRARY\_FUNCTION, USER\_FUNCTION\_NAME     & 22.02        & 37                                & 168                          & 24           & 3            & 7               & 7.88              \\
LIBRARY\_CLASS, VALUE                       & 22.00        & 11                                & 50                           & 24           & 4            & 11              & 12.54             \\
PROGRAMMING\_LANGUAGE, VALUE                & 21.82        & 122                               & 559                          & 24           & 2            & 5               & 5.52              \\
DATA\_TYPE, FILE\_TYPE                      & 21.82        & 24                                & 110                          & 24           & 2            & 8               & 9.16              \\
USER\_VARIABLE, VALUE                       & 21.75        & 72                                & 331                          & 24           & 2            & 6               & 6.57              \\
ALGORITHM, OPERATION\_SYSTEM                & 21.74        & 10                                & 46                           & 24           & 2            & 6               & 8.85              \\
USER\_VARIABLE, OUTPUT\_BLOCK               & 21.67        & 13                                & 60                           & 24           & 3            & 8               & 10.55             \\
PROGRAMMING\_LANGUAGE, OPERATION\_SYSTEM    & 21.64        & 58                                & 268                          & 24           & 2            & 4               & 5.29              \\
USER\_VARIABLE, FILE\_TYPE                  & 21.60        & 54                                & 250                          & 24           & 2            & 7               & 7.58              \\
DEVICE, USER\_FUNCTION\_NAME                & 21.57        & 11                                & 51                           & 24           & 4            & 8               & 10.90             \\
APPLICATION                                 & 21.54        & 252                               & 1170                         & 24           & 1            & 2               & 2.99              \\
DATA\_STRUCTURE, IN\_LINE\_CODE             & 21.48        & 32                                & 149                          & 24           & 3            & 7               & 8.01              \\
VERSION, USER\_NAME                         & 21.43        & 6                                 & 28                           & 24           & 2            & 7.5             & 10.46             \\
ALGORITHM, WEBSITE                          & 21.43        & 3                                 & 14                           & 24           & 2            & 19              & 14.71             \\
DEVICE, UI\_ELEMENT                         & 21.43        & 6                                 & 28                           & 24           & 3            & 14              & 13.86             \\
FILE\_TYPE, IN\_LINE\_CODE                  & 21.43        & 27                                & 126                          & 24           & 2            & 7               & 8.62              \\
VALUE                                       & 21.31        & 156                               & 732                          & 24           & 1            & 4               & 5.06              \\
APPLICATION, PROGRAMMING\_LANGUAGE          & 21.28        & 169                               & 794                          & 24           & 2            & 3               & 3.47              \\
LIBRARY, UI\_ELEMENT                        & 21.28        & 10                                & 47                           & 24           & 3            & 10              & 11.68             \\
APPLICATION, ALGORITHM                      & 21.21        & 14                                & 66                           & 24           & 2            & 4               & 6.52              \\
ALGORITHM, LIBRARY                          & 21.15        & 11                                & 52                           & 24           & 2            & 7               & 8.88              \\
DATA\_TYPE, KEYBOARD\_INPUT                 & 21.15        & 11                                & 52                           & 24           & 3            & 8               & 11.00             \\
LIBRARY, USER\_VARIABLE                     & 21.14        & 85                                & 402                          & 24           & 2            & 6               & 6.80              \\
DATA\_TYPE, WEBSITE                         & 21.05        & 4                                 & 19                           & 24           & 3            & 18              & 16.11             \\
FILE\_TYPE, VALUE                           & 21.01        & 25                                & 119                          & 24           & 2            & 8               & 9.36              \\
DATA\_TYPE, LIBRARY\_CLASS                  & 20.97        & 13                                & 62                           & 24           & 2            & 8.5             & 11.16             \\
DATA\_STRUCTURE, VALUE                      & 20.89        & 33                                & 158                          & 24           & 2            & 6               & 7.69              \\
USER\_NAME, LIBRARY                         & 20.88        & 19                                & 91                           & 24           & 2            & 5               & 6.77              \\
PROGRAMMING\_LANGUAGE, USER\_VARIABLE       & 20.84        & 283                               & 1358                         & 24           & 2            & 4               & 4.79              \\
DEVICE, OUTPUT\_BLOCK                       & 20.83        & 5                                 & 24                           & 24           & 6            & 16.5            & 15.71             \\
DATA\_TYPE, HTML\_TAG\_NAME                 & 20.83        & 5                                 & 24                           & 24           & 5            & 18.5            & 16.00             \\
LIBRARY\_FUNCTION, IN\_LINE\_CODE           & 20.78        & 32                                & 154                          & 24           & 3            & 7               & 7.92              \\
LIBRARY, KEYBOARD\_INPUT                    & 20.75        & 11                                & 53                           & 24           & 4            & 8               & 11.13             \\
ALGORITHM, FILE\_TYPE                       & 20.69        & 6                                 & 29                           & 24           & 3            & 9               & 11.69             \\
OPERATION\_SYSTEM, KEYBOARD\_INPUT          & 20.69        & 6                                 & 29                           & 24           & 5            & 12              & 13.55             \\
DATA\_TYPE, UI\_ELEMENT                     & 20.69        & 6                                 & 29                           & 24           & 4            & 17              & 15.52             \\
PROGRAMMING\_LANGUAGE, KEYBOARD\_INPUT      & 20.56        & 37                                & 180                          & 24           & 2            & 5               & 6.69              \\
VERSION, ALGORITHM                          & 20.51        & 8                                 & 39                           & 24           & 2            & 7               & 10.18             \\
ERROR\_NAME, USER\_NAME                     & 20.51        & 8                                 & 39                           & 24           & 2            & 5               & 8.77              \\
PROGRAMMING\_LANGUAGE, USER\_NAME           & 20.50        & 90                                & 439                          & 24           & 2            & 3               & 3.95              \\
USER\_VARIABLE, IN\_LINE\_CODE              & 20.46        & 62                                & 303                          & 24           & 2            & 6               & 6.50              \\
USER\_VARIABLE, FILE\_NAME                  & 20.43        & 38                                & 186                          & 24           & 3            & 7               & 8.17              \\
DATA\_TYPE, VALUE                           & 20.37        & 33                                & 162                          & 24           & 2            & 6               & 7.36              \\
VALUE, IN\_LINE\_CODE                       & 20.28        & 43                                & 212                          & 24           & 2            & 6               & 7.22              \\
USER\_VARIABLE                              & 20.21        & 334                               & 1653                         & 24           & 1            & 4               & 4.53              \\
PROGRAMMING\_LANGUAGE, ALGORITHM            & 20.07        & 56                                & 279                          & 24           & 2            & 4               & 4.92              \\
OPERATION\_SYSTEM, WEBSITE                  & 20.00        & 3                                 & 15                           & 24           & 4            & 22              & 17.87             \\
DEVICE, ERROR\_NAME                         & 20.00        & 9                                 & 45                           & 24           & 3            & 9               & 10.89             \\
ERROR\_NAME, USER\_CLASS                    & 20.00        & 2                                 & 10                           & 24           & 5            & 19              & 16.30             \\
ERROR\_NAME, IN\_LINE\_CODE                 & 20.00        & 19                                & 95                           & 24           & 2            & 6               & 8.12              \\
LIBRARY, USER\_CLASS                        & 20.00        & 4                                 & 20                           & 24           & 5            & 10.5            & 12.85             \\
LIBRARY, OUTPUT\_BLOCK                      & 20.00        & 7                                 & 35                           & 24           & 5            & 12              & 14.03             \\
USER\_CLASS, UI\_ELEMENT                    & 20.00        & 2                                 & 10                           & 24           & 8            & 20              & 19.60             \\
LIBRARY\_VARIABLE, IN\_LINE\_CODE           & 20.00        & 3                                 & 15                           & 24           & 4            & 15              & 13.93             \\
HTML\_TAG\_NAME, VALUE                      & 20.00        & 6                                 & 30                           & 24           & 2            & 14.5            & 14.00             \\
HTML\_TAG\_NAME, KEYBOARD\_INPUT            & 20.00        & 4                                 & 20                           & 24           & 6            & 19.5            & 18.10             \\
FILE\_NAME, VALUE                           & 19.80        & 20                                & 101                          & 24           & 2            & 8               & 9.71              \\
OPERATION\_SYSTEM, VALUE                    & 19.74        & 15                                & 76                           & 24           & 2            & 6               & 8.14              \\
LIBRARY, USER\_FUNCTION\_NAME               & 19.71        & 41                                & 208                          & 24           & 3            & 7               & 7.72              \\
LIBRARY\_CLASS, IN\_LINE\_CODE              & 19.64        & 11                                & 56                           & 24           & 4            & 10              & 11.82             \\
VERSION, VALUE                              & 19.61        & 10                                & 51                           & 24           & 2            & 9               & 11.35             \\
DATA\_STRUCTURE, OUTPUT\_BLOCK              & 19.44        & 7                                 & 36                           & 24           & 5            & 12              & 13.14             \\
OPERATION\_SYSTEM                           & 19.40        & 77                                & 397                          & 24           & 1            & 3               & 4.37              \\
ALGORITHM                                   & 19.23        & 75                                & 390                          & 24           & 1            & 3               & 4.26              \\
OPERATION\_SYSTEM, UI\_ELEMENT              & 19.23        & 5                                 & 26                           & 24           & 2            & 8.5             & 12.65             \\
WEBSITE, VALUE                              & 19.23        & 5                                 & 26                           & 24           & 3            & 9.5             & 12.85             \\
APPLICATION, USER\_VARIABLE                 & 19.11        & 30                                & 157                          & 24           & 2            & 5               & 6.26              \\
LIBRARY, IN\_LINE\_CODE                     & 19.11        & 30                                & 157                          & 24           & 3            & 7               & 8.36              \\
USER\_NAME                                  & 19.05        & 129                               & 677                          & 24           & 1            & 3               & 3.26              \\
VERSION, WEBSITE                            & 19.05        & 4                                 & 21                           & 24           & 3            & 17              & 14.29             \\
UI\_ELEMENT, WEBSITE                        & 19.05        & 4                                 & 21                           & 24           & 3            & 18              & 15.29             \\
PROGRAMMING\_LANGUAGE, DEVICE               & 19.03        & 43                                & 226                          & 24           & 2            & 4               & 6.00              \\
KEYBOARD\_INPUT                             & 18.94        & 43                                & 227                          & 24           & 1            & 5               & 6.04              \\
DEVICE, FILE\_NAME                          & 18.87        & 10                                & 53                           & 24           & 4            & 9               & 11.47             \\
ALGORITHM, OUTPUT\_BLOCK                    & 18.75        & 3                                 & 16                           & 24           & 2            & 17              & 14.69             \\
USER\_CLASS, IN\_LINE\_CODE                 & 18.75        & 3                                 & 16                           & 24           & 5            & 15              & 14.69             \\
PROGRAMMING\_LANGUAGE, USER\_CLASS          & 18.60        & 8                                 & 43                           & 24           & 2            & 6               & 8.77              \\
PROGRAMMING\_LANGUAGE, WEBSITE              & 18.60        & 24                                & 129                          & 24           & 2            & 4               & 5.67              \\
FILE\_NAME, IN\_LINE\_CODE                  & 18.58        & 21                                & 113                          & 24           & 3            & 7               & 8.58              \\
OPERATION\_SYSTEM, USER\_FUNCTION\_NAME     & 18.52        & 10                                & 54                           & 24           & 2            & 6.5             & 9.63              \\
ALGORITHM, VALUE                            & 18.46        & 12                                & 65                           & 24           & 2            & 6               & 7.94              \\
DEVICE                                      & 18.32        & 50                                & 273                          & 24           & 1            & 4               & 5.56              \\
APPLICATION, USER\_FUNCTION\_NAME           & 18.18        & 14                                & 77                           & 24           & 2            & 6               & 7.32              \\
ALGORITHM, FILE\_NAME                       & 18.18        & 4                                 & 22                           & 24           & 2            & 9.5             & 13.09             \\
USER\_NAME, VALUE                           & 18.18        & 14                                & 77                           & 24           & 2            & 5               & 6.99              \\
DATA\_TYPE, USER\_FUNCTION\_NAME            & 18.18        & 30                                & 165                          & 24           & 2            & 6               & 7.61              \\
IN\_LINE\_CODE, OUTPUT\_BLOCK               & 18.18        & 12                                & 66                           & 24           & 2            & 8               & 10.56             \\
DEVICE, FILE\_TYPE                          & 18.03        & 11                                & 61                           & 24           & 3            & 9               & 10.87             \\
LIBRARY\_FUNCTION, OUTPUT\_BLOCK            & 17.95        & 7                                 & 39                           & 24           & 5            & 9               & 11.87             \\
WEBSITE                                     & 17.86        & 30                                & 168                          & 24           & 1            & 3               & 4.88              \\
OUTPUT\_BLOCK                               & 17.71        & 17                                & 96                           & 24           & 2            & 7               & 9.16              \\
ALGORITHM, LIBRARY\_FUNCTION                & 17.65        & 6                                 & 34                           & 24           & 3            & 7.5             & 9.97              \\
LIBRARY\_FUNCTION, WEBSITE                  & 17.65        & 3                                 & 17                           & 24           & 3            & 16              & 14.71             \\
ERROR\_NAME, USER\_FUNCTION\_NAME           & 17.33        & 13                                & 75                           & 24           & 3            & 7               & 9.00              \\
OPERATION\_SYSTEM, USER\_VARIABLE           & 17.24        & 15                                & 87                           & 24           & 2            & 6               & 8.28              \\
LIBRARY\_FUNCTION, UI\_ELEMENT              & 17.24        & 5                                 & 29                           & 24           & 4            & 12              & 13.72             \\
USER\_NAME, WEBSITE                         & 17.14        & 6                                 & 35                           & 24           & 2            & 5               & 8.77              \\
FILE\_TYPE, OUTPUT\_BLOCK                   & 17.07        & 7                                 & 41                           & 24           & 5            & 11              & 12.80             \\
USER\_NAME, USER\_FUNCTION\_NAME            & 16.92        & 11                                & 65                           & 24           & 2            & 5               & 6.92              \\
USER\_VARIABLE, KEYBOARD\_INPUT             & 16.81        & 19                                & 113                          & 24           & 3            & 6               & 7.78              \\
APPLICATION, USER\_NAME                     & 16.67        & 21                                & 126                          & 24           & 2            & 3               & 4.81              \\
USER\_NAME, LIBRARY\_CLASS                  & 16.67        & 4                                 & 24                           & 24           & 2            & 10              & 12.63             \\
USER\_CLASS, FILE\_TYPE                     & 16.67        & 3                                 & 18                           & 24           & 3            & 13              & 14.39             \\
UI\_ELEMENT, OUTPUT\_BLOCK                  & 16.67        & 4                                 & 24                           & 24           & 6            & 18              & 16.08             \\
VALUE, OUTPUT\_BLOCK                        & 16.67        & 8                                 & 48                           & 24           & 3            & 9.5             & 12.33             \\
OUTPUT\_BLOCK, KEYBOARD\_INPUT              & 16.67        & 6                                 & 36                           & 24           & 4            & 13              & 13.47             \\
PROGRAMMING\_LANGUAGE, OUTPUT\_BLOCK        & 16.46        & 13                                & 79                           & 24           & 3            & 8               & 9.78              \\
PROGRAMMING\_LANGUAGE, USER\_FUNCTION\_NAME & 16.43        & 103                               & 627                          & 24           & 2            & 5               & 5.57              \\
DATA\_STRUCTURE, KEYBOARD\_INPUT            & 16.33        & 8                                 & 49                           & 24           & 3            & 7               & 11.00             \\
FILE\_NAME, UI\_ELEMENT                     & 16.22        & 6                                 & 37                           & 24           & 4            & 11              & 13.19             \\
APPLICATION, FILE\_NAME                     & 16.00        & 12                                & 75                           & 24           & 3            & 5               & 7.29              \\
USER\_FUNCTION\_NAME, VALUE                 & 15.93        & 29                                & 182                          & 24           & 2            & 6               & 7.46              \\
ALGORITHM, IN\_LINE\_CODE                   & 15.91        & 7                                 & 44                           & 24           & 2            & 6.5             & 9.20              \\
USER\_FUNCTION\_NAME                        & 15.90        & 118                               & 742                          & 24           & 1            & 5               & 5.34              \\
APPLICATION, KEYBOARD\_INPUT                & 15.79        & 3                                 & 19                           & 24           & 2            & 8               & 11.63             \\
APPLICATION, OPERATION\_SYSTEM              & 15.71        & 11                                & 70                           & 24           & 2            & 4               & 5.86              \\
LIBRARY\_FUNCTION, KEYBOARD\_INPUT          & 15.69        & 8                                 & 51                           & 24           & 4            & 8               & 10.49             \\
FILE\_NAME, OUTPUT\_BLOCK                   & 15.63        & 5                                 & 32                           & 24           & 5            & 13.5            & 14.31             \\
USER\_CLASS                                 & 15.38        & 8                                 & 52                           & 24           & 1            & 5               & 8.12              \\
DATA\_STRUCTURE, UI\_ELEMENT                & 15.38        & 6                                 & 39                           & 24           & 2            & 11              & 13.21             \\
PROGRAMMING\_LANGUAGE, UI\_ELEMENT          & 15.32        & 19                                & 124                          & 24           & 2            & 5               & 7.26              \\
VALUE, KEYBOARD\_INPUT                      & 15.28        & 11                                & 72                           & 24           & 2            & 7               & 9.82              \\
ERROR\_NAME, KEYBOARD\_INPUT                & 15.15        & 5                                 & 33                           & 24           & 3            & 7               & 11.94             \\
LIBRARY, WEBSITE                            & 15.15        & 5                                 & 33                           & 24           & 3            & 7               & 10.55             \\
DEVICE, VALUE                               & 15.09        & 8                                 & 53                           & 24           & 3            & 8               & 11.02             \\
USER\_VARIABLE, USER\_FUNCTION\_NAME        & 14.69        & 83                                & 565                          & 24           & 2            & 5               & 5.80              \\
FILE\_TYPE, UI\_ELEMENT                     & 14.58        & 7                                 & 48                           & 24           & 4            & 9.5             & 11.96             \\
APPLICATION, UI\_ELEMENT                    & 14.29        & 5                                 & 35                           & 24           & 2            & 6               & 8.89              \\
USER\_CLASS, LIBRARY\_FUNCTION              & 14.29        & 2                                 & 14                           & 24           & 5            & 9               & 11.64             \\
USER\_CLASS, USER\_FUNCTION\_NAME           & 14.29        & 4                                 & 28                           & 24           & 3            & 7.5             & 10.96             \\
USER\_FUNCTION\_NAME, IN\_LINE\_CODE        & 14.18        & 19                                & 134                          & 24           & 3            & 7               & 7.99              \\
UI\_ELEMENT                                 & 14.01        & 22                                & 157                          & 24           & 1            & 5               & 6.60              \\
APPLICATION, ERROR\_NAME                    & 14.00        & 7                                 & 50                           & 24           & 2            & 6               & 7.80              \\
USER\_NAME, USER\_VARIABLE                  & 13.82        & 17                                & 123                          & 24           & 2            & 5               & 5.98              \\
DATA\_STRUCTURE, USER\_CLASS                & 13.64        & 3                                 & 22                           & 24           & 3            & 8               & 11.91             \\
IN\_LINE\_CODE, KEYBOARD\_INPUT             & 13.58        & 11                                & 81                           & 24           & 2            & 7               & 9.27              \\
UI\_ELEMENT, IN\_LINE\_CODE                 & 13.51        & 5                                 & 37                           & 24           & 3            & 11              & 13.35             \\
ALGORITHM, LIBRARY\_CLASS                   & 13.33        & 2                                 & 15                           & 24           & 5            & 20              & 17.67             \\
DEVICE, USER\_VARIABLE                      & 12.94        & 11                                & 85                           & 24           & 2            & 7               & 9.00              \\
APPLICATION, DEVICE                         & 12.90        & 8                                 & 62                           & 24           & 2            & 5               & 7.16              \\
ALGORITHM, USER\_NAME                       & 12.82        & 5                                 & 39                           & 24           & 2            & 4               & 7.23              \\
USER\_CLASS, USER\_VARIABLE                 & 12.50        & 5                                 & 40                           & 24           & 2            & 6               & 8.95              \\
FILE\_TYPE, WEBSITE                         & 12.12        & 4                                 & 33                           & 24           & 2            & 7               & 11.52             \\
ERROR\_NAME, OUTPUT\_BLOCK                  & 12.00        & 3                                 & 25                           & 24           & 4            & 15              & 14.12             \\
UI\_ELEMENT, VALUE                          & 11.86        & 7                                 & 59                           & 24           & 3            & 8               & 11.02             \\
VERSION, HTML\_TAG\_NAME                    & 11.76        & 2                                 & 17                           & 24           & 3            & 20              & 18.65             \\
APPLICATION, WEBSITE                        & 11.11        & 4                                 & 36                           & 24           & 2            & 4.5             & 7.50              \\
USER\_FUNCTION\_NAME, KEYBOARD\_INPUT       & 10.96        & 8                                 & 73                           & 24           & 3            & 6               & 8.79              \\
ALGORITHM, USER\_VARIABLE                   & 10.53        & 14                                & 133                          & 24           & 2            & 5               & 6.63              \\
USER\_FUNCTION\_NAME, OUTPUT\_BLOCK         & 10.53        & 4                                 & 38                           & 24           & 3            & 9               & 11.74             \\
ALGORITHM, HTML\_TAG\_NAME                  & 10.00        & 1                                 & 10                           & 24           & 15           & 23              & 21.90             \\
ALGORITHM, KEYBOARD\_INPUT                  & 10.00        & 3                                 & 30                           & 24           & 3            & 7               & 11.43             \\
USER\_VARIABLE, UI\_ELEMENT                 & 9.86         & 7                                 & 71                           & 24           & 2            & 6               & 9.01              \\
USER\_FUNCTION\_NAME, UI\_ELEMENT           & 9.76         & 4                                 & 41                           & 24           & 3            & 8               & 10.88             \\
FILE\_NAME, WEBSITE                         & 9.68         & 3                                 & 31                           & 24           & 3            & 8               & 11.84             \\
APPLICATION, HTML\_TAG\_NAME                & 9.09         & 1                                 & 11                           & 24           & 4            & 20              & 17.55             \\
ALGORITHM, USER\_FUNCTION\_NAME             & 9.09         & 6                                 & 66                           & 24           & 2            & 7               & 8.45              \\
USER\_CLASS, FILE\_NAME                     & 9.09         & 1                                 & 11                           & 24           & 8            & 20              & 18.27             \\
USER\_CLASS, VALUE                          & 7.69         & 1                                 & 13                           & 24           & 5            & 18              & 16.15             \\
USER\_FUNCTION\_NAME, WEBSITE               & 6.90         & 2                                 & 29                           & 24           & 3            & 7               & 11.45             \\
ALGORITHM, UI\_ELEMENT                      & 6.25         & 1                                 & 16                           & 24           & 3            & 19.5            & 15.31             \\
USER\_VARIABLE, WEBSITE                     & 5.56         & 2                                 & 36                           & 24           & 3            & 7               & 10.67            
\end{tabular}
\end{table}

==> tablets/intent_DISCREPANCY_upto2_combinations_success_rate.tex <==
\begin{table}
\centering
\caption{Entity Combinations in DISCREPANCY intent}
\label{tab:intent_DISCREPANCY_upto2_combinations_success_rate}

\begin{tabular}{llllllll}
Entities Combination                        & Success Rate & Number of Successful Combinations & Total Number of Combinations & Max Entities & Min Entities & Median Entities & Average Entities  \\
USER\_VARIABLE, LIBRARY\_FUNCTION           & 39.1         & 45                                & 115                          & 25           & 3            & 6               & 6.91              \\
LIBRARY\_CLASS, LIBRARY\_FUNCTION           & 38.7         & 12                                & 31                           & 25           & 4            & 7               & 8.94              \\
APPLICATION, FILE\_TYPE                     & 38.5         & 10                                & 26                           & 25           & 3            & 6.5             & 7.96              \\
USER\_NAME, LIBRARY\_FUNCTION               & 37.5         & 6                                 & 16                           & 25           & 4            & 7               & 9.06              \\
LIBRARY\_CLASS, USER\_VARIABLE              & 37.0         & 10                                & 27                           & 25           & 5            & 8               & 9.89              \\
USER\_NAME, USER\_VARIABLE                  & 36.1         & 13                                & 36                           & 25           & 2            & 5               & 6.19              \\
LIBRARY\_CLASS, FILE\_TYPE                  & 35.0         & 7                                 & 20                           & 25           & 6            & 11              & 11.55             \\
DATA\_STRUCTURE, LIBRARY\_FUNCTION          & 34.8         & 23                                & 66                           & 25           & 3            & 7               & 7.29              \\
LIBRARY\_FUNCTION, VALUE                    & 34.8         & 24                                & 69                           & 25           & 2            & 7               & 7.51              \\
OPERATION\_SYSTEM, FILE\_NAME               & 33.3         & 6                                 & 18                           & 25           & 4            & 9.5             & 11.50             \\
DATA\_STRUCTURE, USER\_VARIABLE             & 33.0         & 34                                & 103                          & 25           & 2            & 5               & 6.36              \\
PROGRAMMING\_LANGUAGE, LIBRARY\_FUNCTION    & 33.0         & 66                                & 200                          & 25           & 2            & 6               & 6.11              \\
PROGRAMMING\_LANGUAGE, DATA\_STRUCTURE      & 32.3         & 50                                & 155                          & 25           & 2            & 5               & 5.90              \\
LIBRARY, USER\_VARIABLE                     & 31.9         & 37                                & 116                          & 25           & 3            & 7               & 7.02              \\
LIBRARY\_FUNCTION                           & 31.8         & 71                                & 223                          & 25           & 2            & 6               & 6.00              \\
DATA\_TYPE, LIBRARY\_FUNCTION               & 31.1         & 14                                & 45                           & 25           & 4            & 7               & 7.69              \\
DATA\_STRUCTURE, FILE\_NAME                 & 31.0         & 9                                 & 29                           & 25           & 2            & 8               & 8.93              \\
APPLICATION, USER\_NAME                     & 30.8         & 8                                 & 26                           & 25           & 2            & 4               & 5.92              \\
DATA\_STRUCTURE                             & 30.4         & 58                                & 191                          & 25           & 1            & 5               & 5.47              \\
LIBRARY, FILE\_TYPE                         & 30.2         & 19                                & 63                           & 25           & 3            & 8               & 8.37              \\
LIBRARY\_FUNCTION, USER\_FUNCTION\_NAME     & 29.6         & 16                                & 54                           & 25           & 4            & 7               & 8.11              \\
LIBRARY\_FUNCTION, FILE\_NAME               & 29.3         & 12                                & 41                           & 25           & 4            & 8               & 8.95              \\
LIBRARY\_CLASS                              & 29.1         & 16                                & 55                           & 25           & 2            & 7               & 8.13              \\
DATA\_TYPE, USER\_VARIABLE                  & 29.1         & 16                                & 55                           & 25           & 3            & 6               & 7.42              \\
OPERATION\_SYSTEM, USER\_VARIABLE           & 28.9         & 11                                & 38                           & 25           & 2            & 6               & 7.66              \\
LIBRARY\_FUNCTION, FILE\_TYPE               & 28.9         & 13                                & 45                           & 25           & 4            & 8               & 9.07              \\
PROGRAMMING\_LANGUAGE, LIBRARY\_CLASS       & 28.8         & 15                                & 52                           & 25           & 2            & 7               & 8.13              \\
APPLICATION, USER\_FUNCTION\_NAME           & 28.6         & 6                                 & 21                           & 25           & 4            & 6               & 8.19              \\
LIBRARY\_CLASS, USER\_FUNCTION\_NAME        & 28.6         & 4                                 & 14                           & 25           & 6            & 8               & 11.50             \\
USER\_NAME, VALUE                           & 28.0         & 7                                 & 25                           & 25           & 2            & 5               & 7.48              \\
DATA\_STRUCTURE, USER\_FUNCTION\_NAME       & 27.8         & 15                                & 54                           & 25           & 3            & 7               & 7.52              \\
LIBRARY\_CLASS, FILE\_NAME                  & 27.8         & 5                                 & 18                           & 25           & 5            & 10.5            & 11.22             \\
LIBRARY, LIBRARY\_FUNCTION                  & 27.6         & 32                                & 116                          & 25           & 3            & 6.5             & 6.86              \\
FILE\_TYPE, IN\_LINE\_CODE                  & 27.5         & 14                                & 51                           & 25           & 3            & 7               & 8.39              \\
LIBRARY\_FUNCTION, IN\_LINE\_CODE           & 27.1         & 16                                & 59                           & 25           & 3            & 7               & 8.03              \\
LIBRARY, LIBRARY\_CLASS                     & 27.1         & 13                                & 48                           & 25           & 3            & 7               & 7.85              \\
VERSION, FILE\_NAME                         & 26.3         & 10                                & 38                           & 25           & 4            & 7.5             & 9.21              \\
USER\_FUNCTION\_NAME, FILE\_TYPE            & 26.3         & 10                                & 38                           & 25           & 4            & 8.5             & 9.47              \\
USER\_FUNCTION\_NAME, FILE\_NAME            & 26.3         & 10                                & 38                           & 25           & 5            & 8               & 9.39              \\
FILE\_TYPE, FILE\_NAME                      & 26.1         & 23                                & 88                           & 25           & 2            & 7               & 7.49              \\
APPLICATION, VALUE                          & 26.1         & 6                                 & 23                           & 25           & 3            & 6               & 7.83              \\
LIBRARY, FILE\_NAME                         & 26.1         & 18                                & 69                           & 25           & 3            & 7               & 7.84              \\
PROGRAMMING\_LANGUAGE, FILE\_TYPE           & 26.0         & 34                                & 131                          & 25           & 2            & 6               & 6.85              \\
OPERATION\_SYSTEM, LIBRARY\_FUNCTION        & 25.9         & 7                                 & 27                           & 25           & 3            & 5               & 7.89              \\
ERROR\_NAME, DATA\_STRUCTURE                & 25.9         & 14                                & 54                           & 25           & 3            & 6               & 7.35              \\
LIBRARY, VALUE                              & 25.9         & 21                                & 81                           & 25           & 3            & 7               & 7.62              \\
PROGRAMMING\_LANGUAGE, USER\_VARIABLE       & 25.7         & 93                                & 362                          & 25           & 2            & 5               & 5.35              \\
PROGRAMMING\_LANGUAGE, LIBRARY              & 25.6         & 72                                & 281                          & 25           & 2            & 5               & 5.51              \\
USER\_VARIABLE, VALUE                       & 25.5         & 28                                & 110                          & 25           & 3            & 6               & 6.85              \\
USER\_VARIABLE                              & 25.2         & 114                               & 452                          & 25           & 1            & 5               & 4.94              \\
LIBRARY                                     & 25.2         & 78                                & 310                          & 25           & 1            & 5               & 5.45              \\
FILE\_TYPE                                  & 25.0         & 39                                & 156                          & 25           & 1            & 6               & 6.47              \\
VERSION, USER\_VARIABLE                     & 25.0         & 9                                 & 36                           & 25           & 3            & 7.5             & 9.11              \\
VERSION, USER\_FUNCTION\_NAME               & 25.0         & 5                                 & 20                           & 25           & 3            & 9.5             & 11.10             \\
OPERATION\_SYSTEM, FILE\_TYPE               & 25.0         & 5                                 & 20                           & 25           & 3            & 8.5             & 10.50             \\
LIBRARY\_CLASS, IN\_LINE\_CODE              & 25.0         & 5                                 & 20                           & 25           & 6            & 10.5            & 11.25             \\
FILE\_NAME                                  & 24.9         & 52                                & 209                          & 25           & 1            & 5               & 5.73              \\
USER\_VARIABLE, IN\_LINE\_CODE              & 24.7         & 23                                & 93                           & 25           & 2            & 6               & 6.72              \\
PROGRAMMING\_LANGUAGE, FILE\_NAME           & 24.7         & 43                                & 174                          & 25           & 2            & 5               & 5.98              \\
DATA\_STRUCTURE, DATA\_TYPE                 & 24.5         & 13                                & 53                           & 25           & 2            & 7               & 7.89              \\
APPLICATION, FILE\_NAME                     & 24.3         & 9                                 & 37                           & 25           & 3            & 6               & 7.30              \\
USER\_VARIABLE, FILE\_NAME                  & 24.0         & 18                                & 75                           & 25           & 3            & 7               & 7.65              \\
OPERATION\_SYSTEM, IN\_LINE\_CODE           & 23.8         & 5                                 & 21                           & 25           & 3            & 7               & 9.62              \\
VALUE, IN\_LINE\_CODE                       & 23.6         & 21                                & 89                           & 25           & 3            & 6               & 6.72              \\
DATA\_STRUCTURE, LIBRARY                    & 23.5         & 16                                & 68                           & 25           & 3            & 7               & 7.43              \\
DATA\_STRUCTURE, FILE\_TYPE                 & 23.5         & 8                                 & 34                           & 25           & 4            & 8               & 9.21              \\
LIBRARY, USER\_FUNCTION\_NAME               & 23.4         & 15                                & 64                           & 25           & 4            & 7               & 7.97              \\
VERSION, LIBRARY                            & 23.3         & 14                                & 60                           & 25           & 3            & 7               & 7.43              \\
ERROR\_NAME, LIBRARY\_CLASS                 & 23.3         & 7                                 & 30                           & 25           & 5            & 7.5             & 9.63              \\
FILE\_TYPE, VALUE                           & 23.3         & 10                                & 43                           & 25           & 3            & 8               & 8.79              \\
HTML\_TAG\_NAME                             & 23.1         & 3                                 & 13                           & 25           & 2            & 12              & 12.15             \\
PROGRAMMING\_LANGUAGE                       & 22.8         & 291                               & 1277                         & 25           & 1            & 3               & 3.49              \\
ERROR\_NAME, FILE\_TYPE                     & 22.8         & 18                                & 79                           & 25           & 2            & 6               & 7.53              \\
USER\_NAME, USER\_FUNCTION\_NAME            & 22.7         & 5                                 & 22                           & 25           & 3            & 4.5             & 7.27              \\
USER\_VARIABLE, FILE\_TYPE                  & 22.7         & 15                                & 66                           & 25           & 2            & 8               & 8.24              \\
VERSION, FILE\_TYPE                         & 22.6         & 7                                 & 31                           & 25           & 4            & 8               & 9.84              \\
VERSION, DATA\_STRUCTURE                    & 22.2         & 4                                 & 18                           & 25           & 3            & 7.5             & 10.22             \\
USER\_NAME, LIBRARY                         & 22.2         & 4                                 & 18                           & 25           & 2            & 7               & 7.94              \\
DATA\_STRUCTURE, LIBRARY\_CLASS             & 22.2         & 4                                 & 18                           & 25           & 5            & 8.5             & 11.17             \\
VALUE                                       & 22.0         & 55                                & 250                          & 25           & 1            & 5               & 5.48              \\
ERROR\_NAME, LIBRARY\_FUNCTION              & 22.0         & 20                                & 91                           & 25           & 2            & 6               & 6.85              \\
VERSION, VALUE                              & 21.7         & 5                                 & 23                           & 25           & 3            & 8               & 10.30             \\
FILE\_NAME, IN\_LINE\_CODE                  & 21.7         & 13                                & 60                           & 25           & 3            & 7               & 7.83              \\
VERSION, ERROR\_NAME                        & 21.6         & 16                                & 74                           & 25           & 3            & 6               & 7.27              \\
PROGRAMMING\_LANGUAGE, VALUE                & 21.5         & 42                                & 195                          & 25           & 2            & 5               & 5.97              \\
DEVICE, FILE\_NAME                          & 21.4         & 6                                 & 28                           & 25           & 3            & 7.5             & 9.57              \\
DATA\_TYPE, LIBRARY\_CLASS                  & 21.4         & 3                                 & 14                           & 25           & 6            & 11              & 12.36             \\
LIBRARY\_CLASS, VALUE                       & 21.4         & 3                                 & 14                           & 25           & 6            & 10              & 12.07             \\
PROGRAMMING\_LANGUAGE, VERSION              & 21.3         & 23                                & 108                          & 25           & 2            & 6               & 6.41              \\
APPLICATION, PROGRAMMING\_LANGUAGE          & 21.3         & 33                                & 155                          & 25           & 2            & 4               & 4.44              \\
USER\_FUNCTION\_NAME                        & 21.3         & 43                                & 202                          & 25           & 1            & 5               & 5.90              \\
OPERATION\_SYSTEM, VALUE                    & 21.2         & 7                                 & 33                           & 25           & 3            & 7               & 8.52              \\
DATA\_TYPE, USER\_FUNCTION\_NAME            & 21.2         & 7                                 & 33                           & 25           & 3            & 7               & 8.73              \\
APPLICATION                                 & 21.1         & 49                                & 232                          & 25           & 1            & 3               & 3.84              \\
USER\_NAME, IN\_LINE\_CODE                  & 21.1         & 4                                 & 19                           & 25           & 2            & 6               & 8.47              \\
PROGRAMMING\_LANGUAGE, USER\_NAME           & 20.9         & 19                                & 91                           & 25           & 2            & 4               & 4.67              \\
APPLICATION, LIBRARY\_FUNCTION              & 20.8         & 5                                 & 24                           & 25           & 2            & 7               & 7.96              \\
ERROR\_NAME, USER\_VARIABLE                 & 20.6         & 41                                & 199                          & 25           & 2            & 5               & 5.72              \\
VERSION                                     & 20.4         & 28                                & 137                          & 25           & 1            & 5               & 5.70              \\
USER\_NAME                                  & 20.3         & 31                                & 153                          & 25           & 1            & 3               & 3.88              \\
PROGRAMMING\_LANGUAGE, DATA\_TYPE           & 20.2         & 20                                & 99                           & 25           & 2            & 6               & 6.38              \\
IN\_LINE\_CODE                              & 20.2         & 46                                & 228                          & 25           & 1            & 5               & 5.43              \\
APPLICATION, WEBSITE                        & 20.0         & 2                                 & 10                           & 25           & 3            & 4               & 8.80              \\
VERSION, LIBRARY\_FUNCTION                  & 20.0         & 6                                 & 30                           & 25           & 4            & 7               & 8.97              \\
OPERATION\_SYSTEM, USER\_NAME               & 20.0         & 2                                 & 10                           & 25           & 3            & 5.5             & 10.70             \\
USER\_NAME, DATA\_STRUCTURE                 & 20.0         & 2                                 & 10                           & 25           & 5            & 6.5             & 11.10             \\
USER\_NAME, WEBSITE                         & 20.0         & 3                                 & 15                           & 25           & 2            & 5               & 7.87              \\
USER\_VARIABLE, OUTPUT\_BLOCK               & 20.0         & 3                                 & 15                           & 25           & 4            & 11              & 11.73             \\
ERROR\_NAME, FILE\_NAME                     & 19.8         & 23                                & 116                          & 25           & 2            & 6               & 6.59              \\
FILE\_NAME, VALUE                           & 19.6         & 10                                & 51                           & 25           & 3            & 7               & 8.25              \\
PROGRAMMING\_LANGUAGE, USER\_FUNCTION\_NAME & 19.4         & 35                                & 180                          & 25           & 2            & 5               & 6.07              \\
DATA\_TYPE                                  & 19.3         & 22                                & 114                          & 25           & 2            & 6               & 6.17              \\
APPLICATION, USER\_VARIABLE                 & 19.1         & 9                                 & 47                           & 25           & 2            & 5               & 6.32              \\
ERROR\_NAME, USER\_NAME                     & 19.1         & 9                                 & 47                           & 25           & 2            & 5               & 6.13              \\
VERSION, DEVICE                             & 19.0         & 4                                 & 21                           & 25           & 2            & 9               & 10.33             \\
LIBRARY, IN\_LINE\_CODE                     & 19.0         & 12                                & 63                           & 25           & 3            & 7               & 7.95              \\
USER\_VARIABLE, USER\_FUNCTION\_NAME        & 18.8         & 29                                & 154                          & 25           & 2            & 6               & 6.23              \\
ERROR\_NAME, USER\_FUNCTION\_NAME           & 18.8         & 16                                & 85                           & 25           & 3            & 6               & 7.00              \\
ERROR\_NAME                                 & 18.8         & 120                               & 639                          & 25           & 1            & 4               & 4.05              \\
PROGRAMMING\_LANGUAGE, ERROR\_NAME          & 18.8         & 83                                & 442                          & 25           & 2            & 4               & 4.79              \\
DEVICE, USER\_VARIABLE                      & 18.8         & 6                                 & 32                           & 25           & 3            & 7               & 8.50              \\
PROGRAMMING\_LANGUAGE, IN\_LINE\_CODE       & 18.6         & 33                                & 177                          & 25           & 2            & 5               & 5.85              \\
APPLICATION, DATA\_STRUCTURE                & 18.5         & 5                                 & 27                           & 25           & 2            & 6               & 6.96              \\
PROGRAMMING\_LANGUAGE, DEVICE               & 18.3         & 17                                & 93                           & 25           & 2            & 5               & 5.99              \\
OPERATION\_SYSTEM                           & 18.2         & 27                                & 148                          & 25           & 1            & 4               & 4.80              \\
OPERATION\_SYSTEM, LIBRARY\_CLASS           & 18.2         & 2                                 & 11                           & 25           & 6            & 12              & 13.09             \\
OPERATION\_SYSTEM, USER\_FUNCTION\_NAME     & 18.2         & 4                                 & 22                           & 25           & 2            & 7               & 9.95              \\
DEVICE, FILE\_TYPE                          & 18.2         & 4                                 & 22                           & 25           & 4            & 8.5             & 10.59             \\
FILE\_TYPE, OUTPUT\_BLOCK                   & 18.2         & 2                                 & 11                           & 25           & 7            & 12              & 13.27             \\
DEVICE, ERROR\_NAME                         & 18.0         & 11                                & 61                           & 25           & 3            & 5               & 6.61              \\
APPLICATION, VERSION                        & 17.9         & 5                                 & 28                           & 25           & 2            & 7               & 8.21              \\
PROGRAMMING\_LANGUAGE, OPERATION\_SYSTEM    & 17.8         & 18                                & 101                          & 25           & 2            & 5               & 5.63              \\
OPERATION\_SYSTEM, ERROR\_NAME              & 17.8         & 13                                & 73                           & 25           & 2            & 5               & 6.12              \\
ERROR\_NAME, VALUE                          & 17.7         & 22                                & 124                          & 25           & 2            & 6               & 6.22              \\
VERSION, LIBRARY\_CLASS                     & 17.6         & 3                                 & 17                           & 25           & 5            & 8               & 11.12             \\
LIBRARY\_FUNCTION, OUTPUT\_BLOCK            & 17.6         & 3                                 & 17                           & 25           & 5            & 10              & 11.00             \\
DEVICE                                      & 17.1         & 19                                & 111                          & 25           & 1            & 4               & 5.64              \\
ERROR\_NAME, LIBRARY                        & 16.9         & 23                                & 136                          & 25           & 2            & 6               & 6.55              \\
ERROR\_NAME, IN\_LINE\_CODE                 & 16.8         & 19                                & 113                          & 25           & 2            & 5               & 6.26              \\
OPERATION\_SYSTEM, DEVICE                   & 16.7         & 5                                 & 30                           & 25           & 3            & 6               & 8.57              \\
DEVICE, LIBRARY\_FUNCTION                   & 16.7         & 3                                 & 18                           & 25           & 3            & 7.5             & 9.67              \\
USER\_NAME, FILE\_TYPE                      & 16.7         & 2                                 & 12                           & 25           & 2            & 6.5             & 10.33             \\
APPLICATION, DEVICE                         & 16.0         & 4                                 & 25                           & 25           & 2            & 5               & 7.32              \\
APPLICATION, LIBRARY                        & 15.8         & 6                                 & 38                           & 25           & 2            & 6               & 6.61              \\
DATA\_STRUCTURE, VALUE                      & 15.8         & 6                                 & 38                           & 25           & 3            & 7               & 8.24              \\
DATA\_TYPE, IN\_LINE\_CODE                  & 15.6         & 5                                 & 32                           & 25           & 3            & 7               & 8.63              \\
USER\_VARIABLE, KEYBOARD\_INPUT             & 15.6         & 5                                 & 32                           & 25           & 2            & 6               & 7.47              \\
VERSION, DATA\_TYPE                         & 15.4         & 2                                 & 13                           & 25           & 3            & 11              & 11.23             \\
DEVICE, VALUE                               & 15.4         & 4                                 & 26                           & 25           & 4            & 8               & 9.77              \\
DATA\_STRUCTURE, IN\_LINE\_CODE             & 15.4         & 6                                 & 39                           & 25           & 4            & 7               & 8.49              \\
USER\_FUNCTION\_NAME, VALUE                 & 15.4         & 10                                & 65                           & 25           & 4            & 6               & 7.68              \\
VALUE, OUTPUT\_BLOCK                        & 15.4         & 2                                 & 13                           & 25           & 3            & 9               & 11.15             \\
VERSION, IN\_LINE\_CODE                     & 15.2         & 5                                 & 33                           & 25           & 3            & 7               & 9.21              \\
WEBSITE                                     & 15.0         & 6                                 & 40                           & 25           & 1            & 4.5             & 5.85              \\
PROGRAMMING\_LANGUAGE, WEBSITE              & 14.8         & 4                                 & 27                           & 25           & 2            & 5               & 7.19              \\
APPLICATION, ERROR\_NAME                    & 14.7         & 11                                & 75                           & 25           & 2            & 5               & 5.75              \\
DATA\_TYPE, LIBRARY                         & 14.6         & 6                                 & 41                           & 25           & 3            & 7               & 8.15              \\
DEVICE, DATA\_STRUCTURE                     & 14.3         & 2                                 & 14                           & 25           & 5            & 7.5             & 11.36             \\
ERROR\_NAME, DATA\_TYPE                     & 14.3         & 6                                 & 42                           & 25           & 2            & 6               & 7.45              \\
USER\_NAME, FILE\_NAME                      & 14.3         & 3                                 & 21                           & 25           & 3            & 5               & 8.05              \\
LIBRARY, KEYBOARD\_INPUT                    & 14.3         & 2                                 & 14                           & 25           & 5            & 9.5             & 10.79             \\
OUTPUT\_BLOCK                               & 13.8         & 4                                 & 29                           & 25           & 2            & 7               & 8.86              \\
DEVICE, USER\_NAME                          & 13.3         & 2                                 & 15                           & 25           & 3            & 5               & 9.00              \\
DATA\_STRUCTURE, KEYBOARD\_INPUT            & 13.3         & 2                                 & 15                           & 25           & 3            & 6               & 9.47              \\
FILE\_NAME, WEBSITE                         & 13.3         & 2                                 & 15                           & 25           & 4            & 7               & 10.00             \\
PROGRAMMING\_LANGUAGE, KEYBOARD\_INPUT      & 13.2         & 7                                 & 53                           & 25           & 2            & 6               & 6.94              \\
KEYBOARD\_INPUT                             & 12.9         & 8                                 & 62                           & 25           & 1            & 5               & 6.27              \\
ALGORITHM, VALUE                            & 12.5         & 2                                 & 16                           & 25           & 2            & 6               & 9.31              \\
OPERATION\_SYSTEM, LIBRARY                  & 12.5         & 4                                 & 32                           & 25           & 3            & 6.5             & 8.38              \\
USER\_FUNCTION\_NAME, IN\_LINE\_CODE        & 12.1         & 4                                 & 33                           & 25           & 3            & 7               & 8.58              \\
PROGRAMMING\_LANGUAGE, OUTPUT\_BLOCK        & 12.0         & 3                                 & 25                           & 25           & 2            & 8               & 9.40              \\
PROGRAMMING\_LANGUAGE, ALGORITHM            & 11.8         & 4                                 & 34                           & 25           & 3            & 6               & 7.38              \\
ERROR\_NAME, WEBSITE                        & 11.8         & 2                                 & 17                           & 25           & 3            & 6               & 8.71              \\
DEVICE, LIBRARY                             & 11.5         & 3                                 & 26                           & 25           & 3            & 8               & 8.92              \\
APPLICATION, IN\_LINE\_CODE                 & 11.1         & 2                                 & 18                           & 25           & 4            & 7               & 8.67              \\
ALGORITHM, USER\_VARIABLE                   & 11.1         & 3                                 & 27                           & 25           & 2            & 6               & 7.19              \\
DEVICE, IN\_LINE\_CODE                      & 11.1         & 2                                 & 18                           & 25           & 4            & 7               & 10.22             \\
ERROR\_NAME, OUTPUT\_BLOCK                  & 11.1         & 2                                 & 18                           & 25           & 4            & 10              & 10.83             \\
DATA\_TYPE, FILE\_NAME                      & 10.5         & 2                                 & 19                           & 25           & 3            & 8               & 10.37             \\
IN\_LINE\_CODE, OUTPUT\_BLOCK               & 10.5         & 2                                 & 19                           & 25           & 2            & 9               & 10.53             \\
VERSION, OPERATION\_SYSTEM                  & 10.3         & 3                                 & 29                           & 25           & 2            & 6               & 8.48              \\
VERSION, KEYBOARD\_INPUT                    & 10.0         & 1                                 & 10                           & 25           & 5            & 11.5            & 13.60             \\
ALGORITHM, DEVICE                           & 10.0         & 1                                 & 10                           & 25           & 3            & 11              & 12.70             \\
ALGORITHM, FILE\_NAME                       & 10.0         & 1                                 & 10                           & 25           & 4            & 11              & 13.00             \\
DEVICE, USER\_FUNCTION\_NAME                & 10.0         & 2                                 & 20                           & 25           & 4            & 9               & 10.85             \\
USER\_CLASS, USER\_VARIABLE                 & 10.0         & 1                                 & 10                           & 25           & 5            & 6.5             & 10.50             \\
USER\_VARIABLE, WEBSITE                     & 10.0         & 1                                 & 10                           & 25           & 4            & 7.5             & 10.70             \\
IN\_LINE\_CODE, KEYBOARD\_INPUT             & 9.5          & 2                                 & 21                           & 25           & 2            & 7               & 9.29              \\
PROGRAMMING\_LANGUAGE, USER\_CLASS          & 9.1          & 1                                 & 11                           & 25           & 3            & 6               & 9.91              \\
ALGORITHM, IN\_LINE\_CODE                   & 9.1          & 1                                 & 11                           & 25           & 6            & 7               & 12.27             \\
ERROR\_NAME, KEYBOARD\_INPUT                & 9.1          & 2                                 & 22                           & 25           & 4            & 6               & 9.18              \\
DATA\_TYPE, FILE\_TYPE                      & 9.1          & 2                                 & 22                           & 25           & 6            & 8.5             & 10.64             \\
USER\_CLASS                                 & 8.3          & 1                                 & 12                           & 25           & 3            & 6               & 9.50              \\
VERSION, ALGORITHM                          & 8.3          & 1                                 & 12                           & 25           & 5            & 9               & 12.08             \\
FILE\_NAME, KEYBOARD\_INPUT                 & 8.3          & 1                                 & 12                           & 25           & 4            & 11.5            & 12.42             \\
ALGORITHM                                   & 8.2          & 4                                 & 49                           & 25           & 1            & 5               & 6.20              \\
APPLICATION, DATA\_TYPE                     & 7.7          & 1                                 & 13                           & 25           & 5            & 7               & 9.54              \\
ALGORITHM, DATA\_STRUCTURE                  & 7.7          & 1                                 & 13                           & 25           & 3            & 6               & 10.08             \\
DEVICE, DATA\_TYPE                          & 7.7          & 1                                 & 13                           & 25           & 4            & 8               & 11.62             \\
ERROR\_NAME, UI\_ELEMENT                    & 7.7          & 1                                 & 13                           & 25           & 4            & 6               & 10.15             \\
FILE\_TYPE, WEBSITE                         & 7.7          & 1                                 & 13                           & 25           & 4            & 7               & 10.77             \\
FILE\_TYPE, KEYBOARD\_INPUT                 & 7.7          & 1                                 & 13                           & 25           & 5            & 12              & 12.77             \\
VERSION, USER\_NAME                         & 7.1          & 1                                 & 14                           & 25           & 2            & 4.5             & 8.57              \\
ALGORITHM, USER\_FUNCTION\_NAME             & 6.7          & 1                                 & 15                           & 25           & 4            & 7               & 10.40             \\
USER\_VARIABLE, UI\_ELEMENT                 & 6.7          & 1                                 & 15                           & 25           & 3            & 6               & 8.73              \\
PROGRAMMING\_LANGUAGE, UI\_ELEMENT          & 6.3          & 1                                 & 16                           & 25           & 3            & 6               & 9.06              \\
OPERATION\_SYSTEM, DATA\_STRUCTURE          & 6.3          & 1                                 & 16                           & 25           & 2            & 7.5             & 10.19             \\
LIBRARY\_FUNCTION, KEYBOARD\_INPUT          & 6.3          & 1                                 & 16                           & 25           & 4            & 7               & 9.69              \\
VALUE, KEYBOARD\_INPUT                      & 5.3          & 1                                 & 19                           & 25           & 2            & 7               & 10.00             \\
ALGORITHM, ERROR\_NAME                      & 4.8          & 1                                 & 21                           & 25           & 3            & 6               & 8.57              \\
UI\_ELEMENT                                 & 4.5          & 1                                 & 22                           & 25           & 2            & 5.5             & 8.05              \\
APPLICATION, OPERATION\_SYSTEM              & 4.5          & 1                                 & 22                           & 25           & 2            & 5               & 7.18              \\
APPLICATION, ALGORITHM                      & 0.0          & 0                                 & 12                           & 25           & 3            & 6               & 9.25              \\
ALGORITHM, OPERATION\_SYSTEM                & 0.0          & 0                                 & 11                           & 25           & 4            & 7               & 12.00             \\
OPERATION\_SYSTEM, DATA\_TYPE               & 0.0          & 0                                 & 14                           & 25           & 3            & 8.5             & 10.93             \\
DATA\_TYPE, VALUE                           & 0.0          & 0                                 & 32                           & 25           & 3            & 7               & 8.50              \\
DATA\_TYPE, KEYBOARD\_INPUT                 & 0.0          & 0                                 & 10                           & 25           & 6            & 10              & 13.00             \\
USER\_FUNCTION\_NAME, KEYBOARD\_INPUT       & 0.0          & 0                                 & 21                           & 25           & 3            & 6               & 8.95              \\
FILE\_NAME, UI\_ELEMENT                     & 0.0          & 0                                 & 11                           & 25           & 5            & 9               & 11.73             \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                  
\end{tabular}
\end{table}

==> tablets/intent_ERRORS_upto2_combinations_success_rate.tex <==
\begin{table}
\centering
\caption{Entity Combinations in ERRORS intent}
\label{tab:intent_ERRORS_upto2_combinations_success_rate}

\begin{tabular}{llllllll}
Entities Combination                        & Success Rate & Number of Successful Combinations & Total Number of Combinations & Max Entities & Min Entities & Median Entities & Average Entities  \\
APPLICATION, FILE\_TYPE                     & 53.33        & 8                                 & 15                           & 13           & 3            & 7               & 6.93              \\
OPERATION\_SYSTEM, USER\_VARIABLE           & 45.83        & 11                                & 24                           & 23           & 3            & 6.5             & 7.88              \\
DATA\_STRUCTURE, LIBRARY\_FUNCTION          & 45.10        & 23                                & 51                           & 23           & 4            & 7               & 7.37              \\
USER\_NAME, VALUE                           & 44.44        & 8                                 & 18                           & 23           & 3            & 6               & 7.56              \\
DATA\_STRUCTURE, USER\_VARIABLE             & 42.65        & 29                                & 68                           & 23           & 3            & 7               & 6.82              \\
DATA\_TYPE, LIBRARY\_FUNCTION               & 42.22        & 19                                & 45                           & 23           & 4            & 7               & 7.38              \\
OPERATION\_SYSTEM, FILE\_NAME               & 41.67        & 5                                 & 12                           & 23           & 6            & 11              & 11.58             \\
LIBRARY\_CLASS, USER\_VARIABLE              & 41.67        & 10                                & 24                           & 23           & 4            & 8               & 9.25              \\
DATA\_STRUCTURE, FILE\_NAME                 & 41.18        & 7                                 & 17                           & 23           & 5            & 8               & 9.41              \\
DATA\_TYPE, USER\_VARIABLE                  & 41.07        & 23                                & 56                           & 23           & 3            & 7               & 6.98              \\
LIBRARY\_CLASS, LIBRARY\_FUNCTION           & 40.00        & 10                                & 25                           & 23           & 4            & 8               & 8.64              \\
DATA\_STRUCTURE, DATA\_TYPE                 & 39.53        & 17                                & 43                           & 23           & 2            & 7               & 7.63              \\
USER\_NAME, USER\_VARIABLE                  & 39.13        & 9                                 & 23                           & 23           & 2            & 5               & 6.22              \\
APPLICATION, DATA\_STRUCTURE                & 38.89        & 7                                 & 18                           & 9            & 2            & 7               & 6.33              \\
APPLICATION, USER\_FUNCTION\_NAME           & 38.46        & 5                                 & 13                           & 11           & 4            & 6               & 6.85              \\
USER\_NAME, LIBRARY\_FUNCTION               & 38.46        & 5                                 & 13                           & 23           & 4            & 7               & 8.46              \\
USER\_FUNCTION\_NAME, FILE\_NAME            & 38.24        & 13                                & 34                           & 23           & 5            & 8               & 8.88              \\
APPLICATION, VALUE                          & 38.10        & 8                                 & 21                           & 11           & 4            & 6               & 6.62              \\
PROGRAMMING\_LANGUAGE, DATA\_STRUCTURE      & 37.37        & 37                                & 99                           & 23           & 2            & 5               & 6.28              \\
DATA\_STRUCTURE                             & 37.29        & 44                                & 118                          & 23           & 1            & 5               & 5.93              \\
OPERATION\_SYSTEM, LIBRARY\_FUNCTION        & 36.84        & 7                                 & 19                           & 23           & 3            & 7               & 8.21              \\
USER\_VARIABLE, LIBRARY\_FUNCTION           & 36.84        & 42                                & 114                          & 23           & 3            & 6.5             & 6.84              \\
ERROR\_NAME, DATA\_STRUCTURE                & 36.00        & 18                                & 50                           & 23           & 3            & 6               & 7.08              \\
DATA\_STRUCTURE, USER\_FUNCTION\_NAME       & 35.90        & 14                                & 39                           & 23           & 3            & 7               & 8.03              \\
ERROR\_NAME, USER\_NAME                     & 35.56        & 16                                & 45                           & 23           & 2            & 5               & 5.51              \\
DATA\_TYPE                                  & 35.29        & 36                                & 102                          & 23           & 2            & 6               & 6.02              \\
APPLICATION, LIBRARY\_FUNCTION              & 35.00        & 7                                 & 20                           & 13           & 6            & 7               & 7.65              \\
USER\_FUNCTION\_NAME, FILE\_TYPE            & 34.38        & 11                                & 32                           & 23           & 5            & 8               & 9.41              \\
VERSION, USER\_VARIABLE                     & 34.29        & 12                                & 35                           & 23           & 3            & 7               & 8.20              \\
APPLICATION, USER\_VARIABLE                 & 33.33        & 11                                & 33                           & 11           & 2            & 6               & 5.94              \\
PROGRAMMING\_LANGUAGE, DATA\_TYPE           & 33.33        & 28                                & 84                           & 23           & 2            & 6               & 6.39              \\
USER\_NAME, LIBRARY                         & 33.33        & 5                                 & 15                           & 23           & 2            & 7               & 8.60              \\
DATA\_TYPE, FILE\_NAME                      & 33.33        & 6                                 & 18                           & 23           & 3            & 7.5             & 8.39              \\
LIBRARY, USER\_VARIABLE                     & 33.33        & 35                                & 105                          & 23           & 3            & 7               & 7.19              \\
LIBRARY\_CLASS, FILE\_TYPE                  & 33.33        & 5                                 & 15                           & 23           & 7            & 10              & 11.33             \\
PROGRAMMING\_LANGUAGE, LIBRARY\_FUNCTION    & 33.16        & 63                                & 190                          & 23           & 2            & 6               & 6.11              \\
LIBRARY\_FUNCTION, VALUE                    & 32.26        & 20                                & 62                           & 23           & 3            & 7               & 7.26              \\
LIBRARY\_FUNCTION                           & 32.06        & 67                                & 209                          & 23           & 2            & 6               & 6.05              \\
DATA\_STRUCTURE, LIBRARY                    & 32.00        & 16                                & 50                           & 23           & 3            & 7               & 7.82              \\
OPERATION\_SYSTEM, VALUE                    & 31.82        & 7                                 & 22                           & 23           & 3            & 7               & 8.59              \\
PROGRAMMING\_LANGUAGE, USER\_NAME           & 31.71        & 13                                & 41                           & 23           & 2            & 5               & 5.49              \\
USER\_VARIABLE, FILE\_NAME                  & 31.67        & 19                                & 60                           & 23           & 3            & 7               & 7.53              \\
LIBRARY\_FUNCTION, FILE\_TYPE               & 31.43        & 11                                & 35                           & 23           & 5            & 8               & 8.89              \\
VERSION, DEVICE                             & 31.25        & 5                                 & 16                           & 23           & 2            & 9.5             & 10.38             \\
ERROR\_NAME, DATA\_TYPE                     & 31.11        & 14                                & 45                           & 23           & 2            & 6               & 6.78              \\
USER\_NAME                                  & 30.86        & 25                                & 81                           & 23           & 1            & 4               & 4.37              \\
VERSION, DATA\_STRUCTURE                    & 30.77        & 4                                 & 13                           & 23           & 5            & 8               & 10.08             \\
OPERATION\_SYSTEM, FILE\_TYPE               & 30.77        & 4                                 & 13                           & 23           & 3            & 10              & 10.92             \\
DEVICE, FILE\_TYPE                          & 30.77        & 4                                 & 13                           & 23           & 4            & 10              & 11.38             \\
LIBRARY\_CLASS, USER\_FUNCTION\_NAME        & 30.77        & 4                                 & 13                           & 23           & 6            & 10              & 11.23             \\
LIBRARY\_FUNCTION, USER\_FUNCTION\_NAME     & 30.51        & 18                                & 59                           & 23           & 4            & 7               & 7.59              \\
DATA\_STRUCTURE, VALUE                      & 30.43        & 7                                 & 23                           & 23           & 3            & 7               & 8.35              \\
APPLICATION, DATA\_TYPE                     & 30.00        & 3                                 & 10                           & 9            & 5            & 7               & 6.90              \\
DEVICE, FILE\_NAME                          & 30.00        & 6                                 & 20                           & 23           & 3            & 8               & 9.70              \\
LIBRARY, FILE\_TYPE                         & 29.63        & 16                                & 54                           & 23           & 3            & 8               & 8.54              \\
VERSION, FILE\_TYPE                         & 29.17        & 7                                 & 24                           & 23           & 4            & 8               & 9.46              \\
APPLICATION                                 & 29.10        & 39                                & 134                          & 13           & 1            & 3               & 4.04              \\
LIBRARY, LIBRARY\_FUNCTION                  & 28.97        & 31                                & 107                          & 23           & 3            & 7               & 7.00              \\
USER\_VARIABLE                              & 28.57        & 102                               & 357                          & 23           & 1            & 5               & 5.20              \\
VERSION, LIBRARY\_CLASS                     & 28.57        & 4                                 & 14                           & 23           & 5            & 9               & 10.57             \\
LIBRARY\_FUNCTION, FILE\_NAME               & 28.57        & 12                                & 42                           & 23           & 3            & 8               & 8.26              \\
APPLICATION, PROGRAMMING\_LANGUAGE          & 28.41        & 25                                & 88                           & 11           & 2            & 4               & 4.50              \\
PROGRAMMING\_LANGUAGE, LIBRARY\_CLASS       & 28.26        & 13                                & 46                           & 23           & 3            & 7               & 8.13              \\
DATA\_TYPE, LIBRARY                         & 28.21        & 11                                & 39                           & 23           & 3            & 7               & 8.03              \\
DATA\_STRUCTURE, FILE\_TYPE                 & 28.00        & 7                                 & 25                           & 23           & 4            & 8               & 9.12              \\
PROGRAMMING\_LANGUAGE, OPERATION\_SYSTEM    & 27.87        & 17                                & 61                           & 23           & 2            & 5               & 5.95              \\
PROGRAMMING\_LANGUAGE, USER\_VARIABLE       & 27.82        & 79                                & 284                          & 23           & 2            & 5               & 5.59              \\
OPERATION\_SYSTEM, DEVICE                   & 27.78        & 5                                 & 18                           & 23           & 3            & 7               & 9.11              \\
ERROR\_NAME, LIBRARY\_FUNCTION              & 27.68        & 31                                & 112                          & 23           & 2            & 6               & 6.58              \\
USER\_VARIABLE, FILE\_TYPE                  & 27.45        & 14                                & 51                           & 23           & 3            & 8               & 8.16              \\
OPERATION\_SYSTEM                           & 27.38        & 23                                & 84                           & 23           & 1            & 5               & 5.33              \\
VERSION, FILE\_NAME                         & 27.27        & 9                                 & 33                           & 23           & 3            & 7               & 8.45              \\
OPERATION\_SYSTEM, USER\_FUNCTION\_NAME     & 27.27        & 3                                 & 11                           & 23           & 5            & 12              & 11.55             \\
DATA\_STRUCTURE, LIBRARY\_CLASS             & 27.27        & 3                                 & 11                           & 23           & 5            & 11              & 11.73             \\
DATA\_TYPE, USER\_FUNCTION\_NAME            & 27.27        & 9                                 & 33                           & 23           & 4            & 7               & 8.18              \\
LIBRARY\_CLASS                              & 27.08        & 13                                & 48                           & 23           & 3            & 7               & 8.04              \\
PROGRAMMING\_LANGUAGE, FILE\_TYPE           & 27.08        & 26                                & 96                           & 23           & 2            & 7               & 6.89              \\
LIBRARY, FILE\_NAME                         & 26.98        & 17                                & 63                           & 23           & 4            & 8               & 8.02              \\
FILE\_TYPE, FILE\_NAME                      & 26.98        & 17                                & 63                           & 23           & 2            & 7               & 7.30              \\
APPLICATION, IN\_LINE\_CODE                 & 26.67        & 4                                 & 15                           & 13           & 4            & 7               & 7.13              \\
VERSION, USER\_FUNCTION\_NAME               & 26.67        & 4                                 & 15                           & 23           & 5            & 10              & 10.80             \\
APPLICATION, FILE\_NAME                     & 26.32        & 5                                 & 19                           & 13           & 3            & 7               & 6.95              \\
PROGRAMMING\_LANGUAGE, FILE\_NAME           & 26.12        & 35                                & 134                          & 23           & 2            & 5               & 6.22              \\
LIBRARY, LIBRARY\_CLASS                     & 26.09        & 12                                & 46                           & 23           & 3            & 7               & 8.09              \\
LIBRARY, USER\_FUNCTION\_NAME               & 25.93        & 14                                & 54                           & 23           & 4            & 8               & 8.31              \\
PROGRAMMING\_LANGUAGE                       & 25.14        & 222                               & 883                          & 23           & 1            & 3               & 3.84              \\
APPLICATION, ERROR\_NAME                    & 25.00        & 15                                & 60                           & 13           & 2            & 5               & 5.13              \\
USER\_NAME, IN\_LINE\_CODE                  & 25.00        & 4                                 & 16                           & 23           & 2            & 6               & 7.81              \\
FILE\_TYPE, IN\_LINE\_CODE                  & 25.00        & 10                                & 40                           & 23           & 4            & 7               & 8.33              \\
PROGRAMMING\_LANGUAGE, LIBRARY              & 24.89        & 58                                & 233                          & 23           & 2            & 5               & 5.91              \\
ERROR\_NAME, USER\_VARIABLE                 & 24.76        & 51                                & 206                          & 23           & 2            & 5               & 5.65              \\
LIBRARY                                     & 24.71        & 65                                & 263                          & 23           & 1            & 5               & 5.77              \\
FILE\_TYPE                                  & 24.58        & 29                                & 118                          & 23           & 2            & 6               & 6.48              \\
OPERATION\_SYSTEM, ERROR\_NAME              & 24.56        & 14                                & 57                           & 23           & 2            & 5               & 6.04              \\
DATA\_TYPE, IN\_LINE\_CODE                  & 24.14        & 7                                 & 29                           & 23           & 3            & 7               & 7.83              \\
PROGRAMMING\_LANGUAGE, VERSION              & 23.91        & 22                                & 92                           & 23           & 2            & 5               & 6.35              \\
OPERATION\_SYSTEM, IN\_LINE\_CODE           & 23.81        & 5                                 & 21                           & 23           & 3            & 6               & 8.10              \\
VERSION, LIBRARY                            & 23.73        & 14                                & 59                           & 23           & 3            & 7               & 7.32              \\
PROGRAMMING\_LANGUAGE, DEVICE               & 23.53        & 12                                & 51                           & 23           & 2            & 6               & 6.94              \\
ERROR\_NAME, LIBRARY\_CLASS                 & 23.53        & 8                                 & 34                           & 23           & 5            & 8               & 9.09              \\
FILE\_NAME                                  & 23.46        & 38                                & 162                          & 23           & 2            & 5               & 5.93              \\
OPERATION\_SYSTEM, LIBRARY                  & 23.08        & 6                                 & 26                           & 23           & 4            & 7               & 8.81              \\
USER\_FUNCTION\_NAME                        & 23.03        & 35                                & 152                          & 23           & 2            & 6               & 6.26              \\
FILE\_TYPE, VALUE                           & 22.86        & 8                                 & 35                           & 23           & 2            & 7               & 8.17              \\
DEVICE                                      & 22.73        & 15                                & 66                           & 23           & 1            & 5               & 6.26              \\
USER\_VARIABLE, USER\_FUNCTION\_NAME        & 22.58        & 28                                & 124                          & 23           & 2            & 6               & 6.39              \\
LIBRARY, VALUE                              & 22.50        & 18                                & 80                           & 23           & 3            & 7               & 7.53              \\
VERSION                                     & 22.41        & 26                                & 116                          & 23           & 1            & 5               & 5.73              \\
PROGRAMMING\_LANGUAGE, USER\_FUNCTION\_NAME & 22.31        & 29                                & 130                          & 23           & 2            & 6               & 6.55              \\
APPLICATION, VERSION                        & 22.22        & 4                                 & 18                           & 13           & 3            & 7               & 7.28              \\
VERSION, ERROR\_NAME                        & 22.08        & 17                                & 77                           & 23           & 2            & 5               & 6.55              \\
LIBRARY\_FUNCTION, IN\_LINE\_CODE           & 22.03        & 13                                & 59                           & 23           & 3            & 7               & 7.53              \\
PROGRAMMING\_LANGUAGE, ERROR\_NAME          & 21.96        & 92                                & 419                          & 23           & 2            & 5               & 4.85              \\
APPLICATION, LIBRARY                        & 21.88        & 7                                 & 32                           & 13           & 3            & 7               & 6.72              \\
VERSION, LIBRARY\_FUNCTION                  & 21.88        & 7                                 & 32                           & 23           & 3            & 7               & 8.00              \\
ERROR\_NAME, FILE\_TYPE                     & 21.74        & 15                                & 69                           & 23           & 2            & 7               & 7.28              \\
USER\_VARIABLE, VALUE                       & 21.74        & 20                                & 92                           & 23           & 3            & 6               & 6.80              \\
ERROR\_NAME                                 & 21.43        & 144                               & 672                          & 23           & 1            & 3               & 3.87              \\
DEVICE, ERROR\_NAME                         & 21.43        & 9                                 & 42                           & 23           & 3            & 5.5             & 7.26              \\
VERSION, OPERATION\_SYSTEM                  & 21.05        & 4                                 & 19                           & 23           & 2            & 7               & 9.00              \\
VERSION, VALUE                              & 21.05        & 4                                 & 19                           & 23           & 4            & 8               & 9.58              \\
HTML\_TAG\_NAME                             & 20.00        & 2                                 & 10                           & 23           & 3            & 11              & 11.20             \\
DEVICE, USER\_VARIABLE                      & 20.00        & 5                                 & 25                           & 23           & 4            & 8               & 8.36              \\
ERROR\_NAME, LIBRARY                        & 20.00        & 31                                & 155                          & 23           & 2            & 6               & 6.45              \\
DATA\_TYPE, FILE\_TYPE                      & 20.00        & 4                                 & 20                           & 23           & 6            & 8.5             & 9.95              \\
LIBRARY\_CLASS, IN\_LINE\_CODE              & 20.00        & 4                                 & 20                           & 23           & 5            & 9               & 10.05             \\
USER\_VARIABLE, IN\_LINE\_CODE              & 19.35        & 18                                & 93                           & 23           & 2            & 6               & 6.48              \\
VALUE                                       & 18.66        & 39                                & 209                          & 23           & 2            & 5               & 5.59              \\
PROGRAMMING\_LANGUAGE, VALUE                & 18.29        & 30                                & 164                          & 23           & 2            & 6               & 5.99              \\
ERROR\_NAME, USER\_FUNCTION\_NAME           & 18.18        & 14                                & 77                           & 23           & 3            & 6               & 6.88              \\
DATA\_STRUCTURE, IN\_LINE\_CODE             & 18.18        & 4                                 & 22                           & 23           & 4            & 7.5             & 8.55              \\
VALUE, IN\_LINE\_CODE                       & 18.06        & 13                                & 72                           & 23           & 3            & 6               & 6.90              \\
LIBRARY\_CLASS, FILE\_NAME                  & 17.65        & 3                                 & 17                           & 23           & 6            & 10              & 10.53             \\
IN\_LINE\_CODE, KEYBOARD\_INPUT             & 17.65        & 3                                 & 17                           & 23           & 4            & 7               & 8.76              \\
ERROR\_NAME, FILE\_NAME                     & 17.59        & 19                                & 108                          & 23           & 2            & 5               & 6.45              \\
ERROR\_NAME, VALUE                          & 17.52        & 24                                & 137                          & 23           & 2            & 6               & 5.91              \\
UI\_ELEMENT                                 & 16.67        & 2                                 & 12                           & 23           & 3            & 6               & 8.25              \\
LIBRARY, KEYBOARD\_INPUT                    & 16.67        & 2                                 & 12                           & 23           & 5            & 10.5            & 11.42             \\
IN\_LINE\_CODE                              & 16.44        & 36                                & 219                          & 23           & 1            & 5               & 5.39              \\
FILE\_NAME, VALUE                           & 16.33        & 8                                 & 49                           & 23           & 3            & 7               & 7.57              \\
VERSION, IN\_LINE\_CODE                     & 16.13        & 5                                 & 31                           & 23           & 3            & 7               & 8.10              \\
USER\_FUNCTION\_NAME, VALUE                 & 15.09        & 8                                 & 53                           & 23           & 3            & 7               & 7.57              \\
DEVICE, LIBRARY\_FUNCTION                   & 15.00        & 3                                 & 20                           & 23           & 3            & 8               & 8.70              \\
DEVICE, VALUE                               & 15.00        & 3                                 & 20                           & 23           & 4            & 8               & 9.50              \\
ERROR\_NAME, IN\_LINE\_CODE                 & 14.89        & 21                                & 141                          & 23           & 2            & 5               & 5.83              \\
PROGRAMMING\_LANGUAGE, IN\_LINE\_CODE       & 14.55        & 24                                & 165                          & 23           & 2            & 5               & 5.84              \\
WEBSITE                                     & 14.29        & 3                                 & 21                           & 23           & 1            & 4               & 5.57              \\
PROGRAMMING\_LANGUAGE, ALGORITHM            & 14.29        & 3                                 & 21                           & 23           & 2            & 6               & 7.05              \\
PROGRAMMING\_LANGUAGE, WEBSITE              & 14.29        & 2                                 & 14                           & 23           & 2            & 5               & 6.71              \\
DEVICE, LIBRARY                             & 14.29        & 3                                 & 21                           & 23           & 5            & 9               & 10.38             \\
LIBRARY\_FUNCTION, OUTPUT\_BLOCK            & 14.29        & 2                                 & 14                           & 23           & 5            & 9               & 10.29             \\
LIBRARY\_FUNCTION, KEYBOARD\_INPUT          & 14.29        & 2                                 & 14                           & 23           & 3            & 6               & 8.29              \\
KEYBOARD\_INPUT                             & 14.04        & 8                                 & 57                           & 23           & 1            & 5               & 5.84              \\
LIBRARY, IN\_LINE\_CODE                     & 13.43        & 9                                 & 67                           & 23           & 2            & 7               & 7.78              \\
LIBRARY\_CLASS, VALUE                       & 13.33        & 2                                 & 15                           & 23           & 5            & 8               & 10.27             \\
PROGRAMMING\_LANGUAGE, KEYBOARD\_INPUT      & 12.50        & 6                                 & 48                           & 23           & 2            & 5.5             & 6.46              \\
ALGORITHM, ERROR\_NAME                      & 12.50        & 2                                 & 16                           & 23           & 2            & 6               & 7.75              \\
DATA\_TYPE, VALUE                           & 12.50        & 3                                 & 24                           & 23           & 4            & 7               & 8.29              \\
USER\_VARIABLE, OUTPUT\_BLOCK               & 12.50        & 2                                 & 16                           & 23           & 6            & 8.5             & 9.94              \\
FILE\_NAME, IN\_LINE\_CODE                  & 12.28        & 7                                 & 57                           & 23           & 3            & 7               & 7.40              \\
DEVICE, USER\_FUNCTION\_NAME                & 11.76        & 2                                 & 17                           & 23           & 4            & 9               & 10.12             \\
ALGORITHM                                   & 11.11        & 3                                 & 27                           & 23           & 2            & 6               & 6.44              \\
USER\_FUNCTION\_NAME, IN\_LINE\_CODE        & 10.26        & 4                                 & 39                           & 23           & 4            & 7               & 7.95              \\
LIBRARY, OUTPUT\_BLOCK                      & 10.00        & 1                                 & 10                           & 23           & 6            & 11.5            & 11.80             \\
FILE\_TYPE, OUTPUT\_BLOCK                   & 10.00        & 1                                 & 10                           & 23           & 5            & 11              & 11.40             \\
FILE\_NAME, OUTPUT\_BLOCK                   & 10.00        & 1                                 & 10                           & 23           & 5            & 10.5            & 11.10             \\
FILE\_NAME, KEYBOARD\_INPUT                 & 10.00        & 1                                 & 10                           & 23           & 4            & 10.5            & 11.30             \\
PROGRAMMING\_LANGUAGE, OUTPUT\_BLOCK        & 9.52         & 2                                 & 21                           & 23           & 5            & 7               & 8.71              \\
ERROR\_NAME, OUTPUT\_BLOCK                  & 9.52         & 2                                 & 21                           & 23           & 3            & 7               & 8.67              \\
IN\_LINE\_CODE, OUTPUT\_BLOCK               & 9.52         & 2                                 & 21                           & 23           & 3            & 7               & 8.48              \\
USER\_VARIABLE, KEYBOARD\_INPUT             & 9.38         & 3                                 & 32                           & 23           & 2            & 6               & 6.69              \\
USER\_NAME, FILE\_NAME                      & 9.09         & 1                                 & 11                           & 23           & 3            & 5               & 9.00              \\
FILE\_TYPE, KEYBOARD\_INPUT                 & 9.09         & 1                                 & 11                           & 23           & 5            & 11              & 11.73             \\
ERROR\_NAME, KEYBOARD\_INPUT                & 8.70         & 2                                 & 23                           & 23           & 2            & 6               & 8.09              \\
OUTPUT\_BLOCK                               & 7.69         & 2                                 & 26                           & 23           & 3            & 7               & 8.42              \\
ERROR\_NAME, WEBSITE                        & 7.69         & 1                                 & 13                           & 23           & 3            & 5               & 7.00              \\
ALGORITHM, USER\_VARIABLE                   & 7.14         & 1                                 & 14                           & 23           & 3            & 6               & 7.14              \\
DEVICE, IN\_LINE\_CODE                      & 6.67         & 1                                 & 15                           & 23           & 4            & 7               & 9.33              \\
VALUE, KEYBOARD\_INPUT                      & 5.56         & 1                                 & 18                           & 23           & 2            & 6.5             & 8.78              \\
USER\_FUNCTION\_NAME, KEYBOARD\_INPUT       & 5.00         & 1                                 & 20                           & 23           & 3            & 6               & 7.95              \\
VALUE, OUTPUT\_BLOCK                        & 0.00         & 0                                 & 10                           & 23           & 5            & 8.5             & 10.20            
\end{tabular}
\end{table}

==> tablets/intent_LEARNING_upto2_combinations_success_rate.tex <==
\begin{table}
\centering

\caption{Entity Combinations in LEARNING intent}
\label{tab:intent_LEARNING_upto2_combinations_success_rate}

\begin{tabular}{llllllll}
Entities Combination                        & Success Rate & Number of Successful Combinations & Total Number of Combinations & Max Entities & Min Entities & Median Entities & Average Entities  \\
DEVICE, LIBRARY\_VARIABLE                   & 40.00        & 4                                 & 10                           & 24           & 4            & 16.5            & 15.50             \\
VERSION, DATA\_STRUCTURE                    & 37.50        & 24                                & 64                           & 25           & 3            & 9.5             & 11.97             \\
UI\_ELEMENT, HTML\_TAG\_NAME                & 36.84        & 14                                & 38                           & 25           & 4            & 17              & 15.26             \\
VERSION, LIBRARY\_FUNCTION                  & 36.62        & 26                                & 71                           & 25           & 3            & 8               & 9.85              \\
PROGRAMMING\_LANGUAGE, DATA\_STRUCTURE      & 36.55        & 303                               & 829                          & 25           & 2            & 4               & 4.92              \\
OPERATION\_SYSTEM, LIBRARY\_FUNCTION        & 36.36        & 20                                & 55                           & 25           & 2            & 7               & 9.22              \\
LIBRARY\_VARIABLE, KEYBOARD\_INPUT          & 36.36        & 4                                 & 11                           & 24           & 11           & 18              & 17.27             \\
USER\_NAME, LIBRARY\_FUNCTION               & 35.42        & 17                                & 48                           & 25           & 3            & 6.5             & 8.58              \\
DATA\_TYPE, LIBRARY\_VARIABLE               & 35.29        & 6                                 & 17                           & 24           & 5            & 14              & 13.53             \\
OPERATION\_SYSTEM, HTML\_TAG\_NAME          & 35.00        & 7                                 & 20                           & 25           & 5            & 20.5            & 19.35             \\
DATA\_STRUCTURE                             & 34.34        & 364                               & 1060                         & 25           & 1            & 4               & 4.49              \\
VERSION, LIBRARY                            & 34.33        & 46                                & 134                          & 25           & 2            & 7               & 8.66              \\
DATA\_TYPE, LIBRARY\_FUNCTION               & 34.22        & 64                                & 187                          & 25           & 3            & 7               & 7.91              \\
VERSION, FILE\_NAME                         & 34.12        & 29                                & 85                           & 25           & 2            & 8               & 10.40             \\
ERROR\_NAME, DATA\_STRUCTURE                & 33.85        & 22                                & 65                           & 25           & 3            & 9               & 11.00             \\
DATA\_STRUCTURE, LIBRARY\_FUNCTION          & 33.82        & 69                                & 204                          & 25           & 2            & 6               & 7.69              \\
PROGRAMMING\_LANGUAGE, LIBRARY\_CLASS       & 33.33        & 68                                & 204                          & 25           & 2            & 6               & 7.96              \\
ERROR\_NAME, LIBRARY\_CLASS                 & 33.33        & 13                                & 39                           & 25           & 4            & 12              & 13.97             \\
ERROR\_NAME, HTML\_TAG\_NAME                & 33.33        & 6                                 & 18                           & 25           & 6            & 21.5            & 19.28             \\
LIBRARY\_VARIABLE, OUTPUT\_BLOCK            & 33.33        & 4                                 & 12                           & 22           & 6            & 15.5            & 15.08             \\
DEVICE, LIBRARY\_FUNCTION                   & 32.79        & 20                                & 61                           & 25           & 3            & 9               & 10.41             \\
DATA\_STRUCTURE, FILE\_NAME                 & 32.41        & 35                                & 108                          & 25           & 3            & 9               & 10.27             \\
APPLICATION, LIBRARY\_CLASS                 & 32.35        & 11                                & 34                           & 25           & 4            & 11              & 12.94             \\
DATA\_STRUCTURE, HTML\_TAG\_NAME            & 32.26        & 10                                & 31                           & 25           & 5            & 18              & 17.10             \\
PROGRAMMING\_LANGUAGE, LIBRARY\_FUNCTION    & 32.08        & 213                               & 664                          & 25           & 2            & 5               & 5.70              \\
LIBRARY\_CLASS                              & 31.96        & 70                                & 219                          & 25           & 1            & 6               & 7.91              \\
VERSION, USER\_VARIABLE                     & 31.96        & 31                                & 97                           & 25           & 2            & 7               & 9.65              \\
DATA\_TYPE, OUTPUT\_BLOCK                   & 31.82        & 14                                & 44                           & 25           & 4            & 14              & 14.41             \\
DATA\_STRUCTURE, OUTPUT\_BLOCK              & 31.71        & 13                                & 41                           & 25           & 3            & 15              & 14.78             \\
LIBRARY, LIBRARY\_CLASS                     & 31.69        & 58                                & 183                          & 25           & 3            & 7               & 8.31              \\
LIBRARY\_FUNCTION                           & 31.65        & 232                               & 733                          & 25           & 1            & 5               & 5.61              \\
DATA\_STRUCTURE, LIBRARY\_VARIABLE          & 31.58        & 6                                 & 19                           & 24           & 4            & 12              & 12.68             \\
DATA\_TYPE, USER\_CLASS                     & 31.58        & 6                                 & 19                           & 25           & 5            & 18              & 17.42             \\
LIBRARY\_CLASS, OUTPUT\_BLOCK               & 31.43        & 11                                & 35                           & 25           & 8            & 17              & 16.89             \\
USER\_NAME, DATA\_STRUCTURE                 & 31.40        & 27                                & 86                           & 25           & 2            & 5               & 7.29              \\
DATA\_STRUCTURE, IN\_LINE\_CODE             & 31.36        & 37                                & 118                          & 25           & 2            & 7               & 9.47              \\
LIBRARY, LIBRARY\_FUNCTION                  & 31.20        & 122                               & 391                          & 25           & 2            & 6               & 6.74              \\
DATA\_STRUCTURE, DATA\_TYPE                 & 31.05        & 86                                & 277                          & 25           & 2            & 6               & 7.31              \\
LIBRARY\_CLASS, WEBSITE                     & 31.03        & 9                                 & 29                           & 25           & 4            & 18              & 17.59             \\
DATA\_STRUCTURE, FILE\_TYPE                 & 30.86        & 50                                & 162                          & 25           & 2            & 7               & 8.81              \\
USER\_CLASS, LIBRARY\_FUNCTION              & 30.77        & 4                                 & 13                           & 25           & 6            & 16              & 14.38             \\
USER\_VARIABLE, HTML\_TAG\_NAME             & 30.77        & 12                                & 39                           & 25           & 2            & 16              & 14.00             \\
ERROR\_NAME, USER\_VARIABLE                 & 30.65        & 57                                & 186                          & 25           & 2            & 5.5             & 6.98              \\
DEVICE, HTML\_TAG\_NAME                     & 30.43        & 7                                 & 23                           & 25           & 5            & 20              & 18.87             \\
LIBRARY\_FUNCTION, HTML\_TAG\_NAME          & 30.43        & 7                                 & 23                           & 25           & 4            & 17              & 15.78             \\
LIBRARY, LIBRARY\_VARIABLE                  & 30.30        & 10                                & 33                           & 24           & 3            & 9               & 10.70             \\
LIBRARY\_CLASS, LIBRARY\_FUNCTION           & 30.28        & 33                                & 109                          & 25           & 2            & 8               & 9.11              \\
VERSION, LIBRARY\_VARIABLE                  & 30.00        & 3                                 & 10                           & 24           & 3            & 16.5            & 15.30             \\
DATA\_STRUCTURE, LIBRARY\_CLASS             & 30.00        & 21                                & 70                           & 25           & 4            & 11              & 12.19             \\
DATA\_TYPE, HTML\_TAG\_NAME                 & 30.00        & 9                                 & 30                           & 25           & 5            & 17.5            & 16.63             \\
LIBRARY\_CLASS, HTML\_TAG\_NAME             & 30.00        & 9                                 & 30                           & 25           & 4            & 18.5            & 17.40             \\
WEBSITE, OUTPUT\_BLOCK                      & 30.00        & 6                                 & 20                           & 25           & 13           & 20.5            & 20.00             \\
DATA\_TYPE, IN\_LINE\_CODE                  & 29.93        & 41                                & 137                          & 25           & 2            & 7               & 9.01              \\
LIBRARY\_FUNCTION, VALUE                    & 29.80        & 45                                & 151                          & 25           & 3            & 7               & 8.09              \\
UI\_ELEMENT, KEYBOARD\_INPUT                & 29.79        & 14                                & 47                           & 25           & 2            & 17              & 14.02             \\
VERSION, KEYBOARD\_INPUT                    & 29.73        & 11                                & 37                           & 25           & 5            & 17              & 15.54             \\
DATA\_TYPE, FILE\_NAME                      & 29.67        & 27                                & 91                           & 25           & 3            & 9               & 10.98             \\
USER\_VARIABLE, LIBRARY\_FUNCTION           & 29.65        & 110                               & 371                          & 25           & 2            & 6               & 6.78              \\
OPERATION\_SYSTEM, LIBRARY\_CLASS           & 29.63        & 8                                 & 27                           & 25           & 8            & 18              & 17.74             \\
ALGORITHM, DEVICE                           & 29.55        & 13                                & 44                           & 25           & 3            & 9               & 12.18             \\
DATA\_STRUCTURE, LIBRARY                    & 29.47        & 84                                & 285                          & 25           & 2            & 6               & 7.41              \\
DEVICE, DATA\_STRUCTURE                     & 29.41        & 20                                & 68                           & 25           & 3            & 10              & 11.68             \\
DATA\_TYPE, WEBSITE                         & 29.41        & 10                                & 34                           & 25           & 3            & 17              & 14.62             \\
PROGRAMMING\_LANGUAGE, DATA\_TYPE           & 29.26        & 187                               & 639                          & 25           & 2            & 4               & 5.36              \\
OPERATION\_SYSTEM, OUTPUT\_BLOCK            & 29.17        & 7                                 & 24                           & 25           & 8            & 18.5            & 17.75             \\
VERSION, OUTPUT\_BLOCK                      & 29.03        & 9                                 & 31                           & 25           & 3            & 18              & 16.26             \\
USER\_NAME, KEYBOARD\_INPUT                 & 29.03        & 9                                 & 31                           & 25           & 3            & 8               & 11.61             \\
LIBRARY\_VARIABLE, LIBRARY\_FUNCTION        & 29.03        & 9                                 & 31                           & 24           & 4            & 9               & 11.26             \\
VERSION, VALUE                              & 28.85        & 15                                & 52                           & 25           & 3            & 12              & 13.35             \\
ERROR\_NAME, DATA\_TYPE                     & 28.79        & 19                                & 66                           & 25           & 3            & 8               & 10.24             \\
ERROR\_NAME, LIBRARY\_FUNCTION              & 28.75        & 23                                & 80                           & 25           & 2            & 7               & 8.59              \\
VALUE, IN\_LINE\_CODE                       & 28.71        & 58                                & 202                          & 25           & 2            & 6               & 7.98              \\
VERSION, FILE\_TYPE                         & 28.57        & 24                                & 84                           & 25           & 2            & 8               & 10.70             \\
VERSION, UI\_ELEMENT                        & 28.57        & 8                                 & 28                           & 25           & 4            & 19              & 17.93             \\
ERROR\_NAME, USER\_NAME                     & 28.57        & 18                                & 63                           & 25           & 2            & 5               & 7.54              \\
LIBRARY, OUTPUT\_BLOCK                      & 28.57        & 14                                & 49                           & 25           & 5            & 15              & 14.76             \\
LIBRARY\_VARIABLE, FILE\_TYPE               & 28.57        & 6                                 & 21                           & 24           & 6            & 9               & 12.00             \\
FILE\_NAME, OUTPUT\_BLOCK                   & 28.57        & 12                                & 42                           & 25           & 6            & 15              & 15.26             \\
WEBSITE, KEYBOARD\_INPUT                    & 28.57        & 8                                 & 28                           & 25           & 2            & 18              & 17.14             \\
DATA\_STRUCTURE, USER\_VARIABLE             & 28.47        & 117                               & 411                          & 25           & 2            & 5               & 6.33              \\
LIBRARY\_CLASS, FILE\_NAME                  & 28.36        & 19                                & 67                           & 25           & 6            & 11              & 13.09             \\
OPERATION\_SYSTEM, IN\_LINE\_CODE           & 28.30        & 15                                & 53                           & 25           & 3            & 8               & 11.47             \\
VERSION, ALGORITHM                          & 28.26        & 13                                & 46                           & 25           & 2            & 7.5             & 11.37             \\
DATA\_STRUCTURE, UI\_ELEMENT                & 28.26        & 13                                & 46                           & 25           & 4            & 16              & 14.80             \\
ERROR\_NAME, USER\_FUNCTION\_NAME           & 28.24        & 24                                & 85                           & 25           & 3            & 7               & 9.09              \\
DATA\_TYPE, FILE\_TYPE                      & 28.23        & 35                                & 124                          & 25           & 2            & 8.5             & 9.77              \\
VERSION, LIBRARY\_CLASS                     & 28.21        & 11                                & 39                           & 25           & 7            & 17              & 15.59             \\
LIBRARY\_CLASS, USER\_FUNCTION\_NAME        & 28.17        & 20                                & 71                           & 25           & 3            & 10              & 11.59             \\
ALGORITHM, ERROR\_NAME                      & 28.13        & 9                                 & 32                           & 25           & 2            & 12.5            & 13.25             \\
ERROR\_NAME, FILE\_TYPE                     & 28.13        & 27                                & 96                           & 25           & 3            & 7               & 9.66              \\
WEBSITE, IN\_LINE\_CODE                     & 28.13        & 9                                 & 32                           & 25           & 4            & 17              & 15.34             \\
PROGRAMMING\_LANGUAGE, IN\_LINE\_CODE       & 28.01        & 149                               & 532                          & 25           & 2            & 5               & 5.72              \\
ALGORITHM, WEBSITE                          & 28.00        & 7                                 & 25                           & 25           & 3            & 16              & 14.36             \\
OPERATION\_SYSTEM, ERROR\_NAME              & 28.00        & 14                                & 50                           & 25           & 2            & 7               & 10.86             \\
OPERATION\_SYSTEM, WEBSITE                  & 28.00        & 7                                 & 25                           & 25           & 5            & 18              & 18.12             \\
HTML\_TAG\_NAME, OUTPUT\_BLOCK              & 28.00        & 7                                 & 25                           & 25           & 8            & 19              & 18.40             \\
DATA\_TYPE                                  & 27.99        & 227                               & 811                          & 25           & 1            & 4               & 4.88              \\
OPERATION\_SYSTEM, DATA\_STRUCTURE          & 27.94        & 19                                & 68                           & 25           & 2            & 7               & 10.29             \\
DATA\_STRUCTURE, WEBSITE                    & 27.91        & 12                                & 43                           & 25           & 3            & 15              & 13.40             \\
DATA\_TYPE, UI\_ELEMENT                     & 27.91        & 12                                & 43                           & 25           & 3            & 17              & 14.88             \\
VERSION, IN\_LINE\_CODE                     & 27.87        & 17                                & 61                           & 25           & 3            & 8               & 11.52             \\
DEVICE, DATA\_TYPE                          & 27.78        & 20                                & 72                           & 25           & 2            & 9               & 11.35             \\
LIBRARY\_VARIABLE, VALUE                    & 27.78        & 5                                 & 18                           & 24           & 4            & 13.5            & 13.39             \\
APPLICATION, LIBRARY\_FUNCTION              & 27.71        & 23                                & 83                           & 25           & 3            & 7               & 8.19              \\
VERSION, DEVICE                             & 27.63        & 21                                & 76                           & 25           & 3            & 8               & 10.84             \\
PROGRAMMING\_LANGUAGE, HTML\_TAG\_NAME      & 27.59        & 16                                & 58                           & 25           & 2            & 9.5             & 11.71             \\
ERROR\_NAME, UI\_ELEMENT                    & 27.59        & 8                                 & 29                           & 25           & 4            & 19              & 15.93             \\
ERROR\_NAME, VALUE                          & 27.52        & 30                                & 109                          & 25           & 2            & 6               & 8.47              \\
FILE\_TYPE, OUTPUT\_BLOCK                   & 27.45        & 14                                & 51                           & 25           & 3            & 12              & 13.78             \\
OPERATION\_SYSTEM, DATA\_TYPE               & 27.42        & 17                                & 62                           & 25           & 3            & 8.5             & 10.94             \\
APPLICATION, DATA\_STRUCTURE                & 27.39        & 43                                & 157                          & 25           & 2            & 5               & 6.59              \\
VERSION, ERROR\_NAME                        & 27.27        & 18                                & 66                           & 25           & 2            & 7.5             & 10.35             \\
LIBRARY\_VARIABLE, UI\_ELEMENT              & 27.27        & 3                                 & 11                           & 24           & 8            & 18              & 16.73             \\
APPLICATION, VERSION                        & 27.18        & 28                                & 103                          & 25           & 2            & 5               & 7.22              \\
IN\_LINE\_CODE                              & 27.15        & 183                               & 674                          & 25           & 1            & 4               & 5.26              \\
LIBRARY\_FUNCTION, USER\_FUNCTION\_NAME     & 27.12        & 48                                & 177                          & 25           & 3            & 7               & 7.90              \\
DATA\_STRUCTURE, USER\_FUNCTION\_NAME       & 27.09        & 55                                & 203                          & 25           & 2            & 6               & 7.65              \\
VERSION, USER\_FUNCTION\_NAME               & 27.08        & 13                                & 48                           & 25           & 3            & 11              & 12.58             \\
PROGRAMMING\_LANGUAGE, VERSION              & 27.06        & 92                                & 340                          & 25           & 2            & 4               & 5.62              \\
DEVICE, LIBRARY\_CLASS                      & 27.03        & 10                                & 37                           & 25           & 3            & 17              & 15.73             \\
LIBRARY\_CLASS, UI\_ELEMENT                 & 27.03        & 10                                & 37                           & 25           & 4            & 18              & 17.00             \\
LIBRARY\_CLASS, KEYBOARD\_INPUT             & 27.03        & 10                                & 37                           & 25           & 5            & 18              & 16.89             \\
LIBRARY\_FUNCTION, FILE\_NAME               & 26.98        & 34                                & 126                          & 25           & 3            & 8.5             & 9.44              \\
ALGORITHM, DATA\_TYPE                       & 26.88        & 25                                & 93                           & 25           & 2            & 5               & 8.13              \\
VERSION, USER\_NAME                         & 26.83        & 11                                & 41                           & 25           & 2            & 7               & 9.76              \\
LIBRARY\_CLASS, FILE\_TYPE                  & 26.83        & 22                                & 82                           & 25           & 4            & 10              & 11.99             \\
PROGRAMMING\_LANGUAGE, ERROR\_NAME          & 26.79        & 112                               & 418                          & 25           & 2            & 4               & 5.25              \\
OPERATION\_SYSTEM, FILE\_NAME               & 26.79        & 15                                & 56                           & 25           & 3            & 10              & 11.84             \\
LIBRARY\_FUNCTION, IN\_LINE\_CODE           & 26.71        & 39                                & 146                          & 25           & 3            & 7               & 8.55              \\
OPERATION\_SYSTEM, USER\_CLASS              & 26.67        & 4                                 & 15                           & 25           & 12           & 21              & 19.67             \\
DEVICE, WEBSITE                             & 26.67        & 8                                 & 30                           & 25           & 3            & 17.5            & 15.70             \\
ERROR\_NAME, WEBSITE                        & 26.67        & 8                                 & 30                           & 25           & 3            & 10.5            & 12.90             \\
LIBRARY\_CLASS, USER\_VARIABLE              & 26.67        & 28                                & 105                          & 25           & 3            & 9               & 10.43             \\
LIBRARY\_CLASS, IN\_LINE\_CODE              & 26.67        & 16                                & 60                           & 25           & 5            & 12              & 13.28             \\
LIBRARY\_VARIABLE, IN\_LINE\_CODE           & 26.67        & 4                                 & 15                           & 24           & 3            & 15              & 14.13             \\
HTML\_TAG\_NAME, KEYBOARD\_INPUT            & 26.67        & 8                                 & 30                           & 25           & 4            & 18.5            & 16.93             \\
DEVICE, OUTPUT\_BLOCK                       & 26.47        & 9                                 & 34                           & 25           & 6            & 17              & 15.85             \\
HTML\_TAG\_NAME, IN\_LINE\_CODE             & 26.47        & 9                                 & 34                           & 25           & 2            & 17              & 15.91             \\
OUTPUT\_BLOCK, KEYBOARD\_INPUT              & 26.42        & 14                                & 53                           & 25           & 4            & 14              & 13.70             \\
DATA\_STRUCTURE, KEYBOARD\_INPUT            & 26.32        & 15                                & 57                           & 25           & 3            & 12              & 12.46             \\
LIBRARY\_VARIABLE, USER\_FUNCTION\_NAME     & 26.32        & 5                                 & 19                           & 24           & 4            & 11              & 12.05             \\
VERSION, DATA\_TYPE                         & 26.23        & 16                                & 61                           & 25           & 3            & 10              & 12.08             \\
DATA\_STRUCTURE, VALUE                      & 26.21        & 38                                & 145                          & 25           & 2            & 7               & 8.78              \\
DEVICE, KEYBOARD\_INPUT                     & 26.19        & 11                                & 42                           & 25           & 3            & 16              & 14.50             \\
VERSION                                     & 26.18        & 111                               & 424                          & 25           & 1            & 3.5             & 5.08              \\
HTML\_TAG\_NAME                             & 26.14        & 23                                & 88                           & 25           & 1            & 5.5             & 8.75              \\
LIBRARY, VALUE                              & 25.95        & 48                                & 185                          & 25           & 2            & 7               & 8.72              \\
LIBRARY\_FUNCTION, FILE\_TYPE               & 25.88        & 44                                & 170                          & 25           & 3            & 7.5             & 8.55              \\
OPERATION\_SYSTEM, DEVICE                   & 25.86        & 30                                & 116                          & 25           & 2            & 5               & 8.29              \\
DATA\_TYPE, LIBRARY\_CLASS                  & 25.76        & 17                                & 66                           & 25           & 3            & 10.5            & 12.42             \\
DATA\_TYPE, LIBRARY                         & 25.74        & 52                                & 202                          & 25           & 3            & 7               & 8.42              \\
DATA\_TYPE, USER\_VARIABLE                  & 25.70        & 83                                & 323                          & 25           & 2            & 5               & 6.69              \\
FILE\_TYPE, FILE\_NAME                      & 25.70        & 83                                & 323                          & 25           & 2            & 6               & 7.36              \\
USER\_VARIABLE, OUTPUT\_BLOCK               & 25.68        & 19                                & 74                           & 25           & 3            & 9               & 11.16             \\
PROGRAMMING\_LANGUAGE, LIBRARY\_VARIABLE    & 25.64        & 10                                & 39                           & 24           & 3            & 8               & 10.15             \\
DATA\_TYPE, VALUE                           & 25.62        & 41                                & 160                          & 25           & 2            & 6               & 8.26              \\
USER\_VARIABLE, IN\_LINE\_CODE              & 25.55        & 81                                & 317                          & 25           & 2            & 6               & 6.75              \\
PROGRAMMING\_LANGUAGE, VALUE                & 25.44        & 160                               & 629                          & 25           & 2            & 5               & 5.62              \\
DEVICE, USER\_NAME                          & 25.42        & 15                                & 59                           & 25           & 2            & 5               & 8.24              \\
PROGRAMMING\_LANGUAGE, KEYBOARD\_INPUT      & 25.33        & 57                                & 225                          & 25           & 2            & 5               & 7.02              \\
ERROR\_NAME                                 & 25.04        & 147                               & 587                          & 25           & 1            & 3               & 4.45              \\
ALGORITHM, DATA\_STRUCTURE                  & 25.00        & 30                                & 120                          & 25           & 2            & 5               & 7.49              \\
ALGORITHM, FILE\_NAME                       & 25.00        & 6                                 & 24                           & 25           & 5            & 19              & 16.54             \\
OPERATION\_SYSTEM, USER\_NAME               & 25.00        & 10                                & 40                           & 25           & 2            & 5.5             & 9.35              \\
OPERATION\_SYSTEM, LIBRARY                  & 25.00        & 23                                & 92                           & 25           & 2            & 6               & 8.95              \\
OPERATION\_SYSTEM, FILE\_TYPE               & 25.00        & 18                                & 72                           & 25           & 2            & 7               & 9.74              \\
ERROR\_NAME, LIBRARY                        & 25.00        & 36                                & 144                          & 25           & 2            & 6               & 8.09              \\
USER\_NAME, HTML\_TAG\_NAME                 & 25.00        & 3                                 & 12                           & 25           & 2            & 22.5            & 19.25             \\
USER\_CLASS, IN\_LINE\_CODE                 & 25.00        & 5                                 & 20                           & 25           & 6            & 19              & 18.10             \\
USER\_FUNCTION\_NAME, HTML\_TAG\_NAME       & 25.00        & 6                                 & 24                           & 25           & 5            & 17              & 17.13             \\
FILE\_NAME, HTML\_TAG\_NAME                 & 25.00        & 8                                 & 32                           & 25           & 3            & 17              & 16.16             \\
USER\_VARIABLE, VALUE                       & 24.73        & 91                                & 368                          & 25           & 2            & 5               & 6.68              \\
LIBRARY\_CLASS, VALUE                       & 24.59        & 15                                & 61                           & 25           & 4            & 11              & 13.08             \\
KEYBOARD\_INPUT                             & 24.57        & 71                                & 289                          & 25           & 1            & 5               & 6.26              \\
ALGORITHM, OPERATION\_SYSTEM                & 24.56        & 14                                & 57                           & 25           & 2            & 6               & 9.75              \\
LIBRARY, FILE\_NAME                         & 24.54        & 53                                & 216                          & 25           & 2            & 7               & 8.65              \\
LIBRARY\_FUNCTION, OUTPUT\_BLOCK            & 24.44        & 11                                & 45                           & 25           & 5            & 11              & 12.11             \\
UI\_ELEMENT, WEBSITE                        & 24.44        & 11                                & 45                           & 25           & 3            & 16              & 13.27             \\
ALGORITHM, LIBRARY                          & 24.32        & 18                                & 74                           & 25           & 2            & 6               & 9.41              \\
VALUE                                       & 24.31        & 195                               & 802                          & 25           & 1            & 4               & 5.16              \\
LIBRARY, FILE\_TYPE                         & 24.22        & 70                                & 289                          & 25           & 2            & 7               & 7.88              \\
DATA\_TYPE, KEYBOARD\_INPUT                 & 24.14        & 14                                & 58                           & 25           & 3            & 11              & 12.53             \\
FILE\_TYPE, HTML\_TAG\_NAME                 & 24.14        & 7                                 & 29                           & 25           & 5            & 17              & 16.90             \\
ERROR\_NAME, FILE\_NAME                     & 24.07        & 26                                & 108                          & 25           & 2            & 7               & 9.04              \\
USER\_NAME, IN\_LINE\_CODE                  & 24.07        & 13                                & 54                           & 25           & 2            & 6               & 8.41              \\
USER\_FUNCTION\_NAME, OUTPUT\_BLOCK         & 24.07        & 13                                & 54                           & 25           & 3            & 9.5             & 12.04             \\
FILE\_NAME, KEYBOARD\_INPUT                 & 24.07        & 13                                & 54                           & 25           & 3            & 12              & 13.41             \\
LIBRARY\_CLASS, LIBRARY\_VARIABLE           & 24.00        & 6                                 & 25                           & 24           & 6            & 12              & 12.96             \\
UI\_ELEMENT, IN\_LINE\_CODE                 & 24.00        & 12                                & 50                           & 25           & 4            & 15.5            & 13.90             \\
PROGRAMMING\_LANGUAGE, LIBRARY              & 23.94        & 323                               & 1349                         & 25           & 2            & 4               & 4.69              \\
PROGRAMMING\_LANGUAGE, OPERATION\_SYSTEM    & 23.91        & 88                                & 368                          & 25           & 2            & 4               & 5.04              \\
VERSION, OPERATION\_SYSTEM                  & 23.75        & 19                                & 80                           & 25           & 2            & 7               & 9.48              \\
LIBRARY, HTML\_TAG\_NAME                    & 23.68        & 9                                 & 38                           & 25           & 2            & 17              & 15.03             \\
LIBRARY                                     & 23.64        & 360                               & 1523                         & 25           & 1            & 4               & 4.52              \\
IN\_LINE\_CODE, OUTPUT\_BLOCK               & 23.61        & 17                                & 72                           & 25           & 2            & 10              & 11.89             \\
DEVICE, USER\_CLASS                         & 23.53        & 4                                 & 17                           & 25           & 12           & 20              & 19.18             \\
LIBRARY\_VARIABLE, FILE\_NAME               & 23.53        & 4                                 & 17                           & 24           & 6            & 12              & 13.00             \\
LIBRARY, KEYBOARD\_INPUT                    & 23.38        & 18                                & 77                           & 25           & 3            & 10              & 11.73             \\
PROGRAMMING\_LANGUAGE, FILE\_NAME           & 23.33        & 133                               & 570                          & 25           & 2            & 5               & 5.76              \\
WEBSITE, HTML\_TAG\_NAME                    & 23.33        & 7                                 & 30                           & 25           & 2            & 17              & 16.03             \\
LIBRARY, IN\_LINE\_CODE                     & 23.30        & 41                                & 176                          & 25           & 3            & 7               & 8.83              \\
PROGRAMMING\_LANGUAGE, FILE\_TYPE           & 23.25        & 179                               & 770                          & 25           & 2            & 4               & 5.41              \\
PROGRAMMING\_LANGUAGE, OUTPUT\_BLOCK        & 23.16        & 22                                & 95                           & 25           & 2            & 8               & 10.34             \\
USER\_FUNCTION\_NAME, FILE\_NAME            & 23.14        & 28                                & 121                          & 25           & 3            & 8               & 9.76              \\
ALGORITHM, USER\_CLASS                      & 23.08        & 3                                 & 13                           & 25           & 4            & 21              & 19.46             \\
LIBRARY\_FUNCTION, WEBSITE                  & 23.08        & 6                                 & 26                           & 25           & 3            & 15.5            & 13.58             \\
FILE\_TYPE                                  & 22.99        & 206                               & 896                          & 25           & 1            & 4               & 5.15              \\
FILE\_TYPE, IN\_LINE\_CODE                  & 22.97        & 34                                & 148                          & 25           & 2            & 7               & 9.14              \\
FILE\_NAME, VALUE                           & 22.95        & 28                                & 122                          & 25           & 3            & 9               & 10.21             \\
FILE\_NAME                                  & 22.87        & 148                               & 647                          & 25           & 1            & 4               & 5.58              \\
APPLICATION, DATA\_TYPE                     & 22.86        & 24                                & 105                          & 25           & 2            & 6               & 7.79              \\
LIBRARY\_FUNCTION, UI\_ELEMENT              & 22.86        & 8                                 & 35                           & 25           & 2            & 14              & 13.66             \\
FILE\_TYPE, VALUE                           & 22.86        & 32                                & 140                          & 25           & 2            & 8               & 9.81              \\
UI\_ELEMENT, OUTPUT\_BLOCK                  & 22.86        & 8                                 & 35                           & 25           & 4            & 17              & 16.20             \\
OUTPUT\_BLOCK                               & 22.81        & 26                                & 114                          & 25           & 1            & 8               & 9.82              \\
VALUE, OUTPUT\_BLOCK                        & 22.81        & 13                                & 57                           & 25           & 5            & 13              & 13.68             \\
LIBRARY\_VARIABLE                           & 22.73        & 10                                & 44                           & 24           & 3            & 8               & 9.82              \\
DEVICE, UI\_ELEMENT                         & 22.73        & 10                                & 44                           & 25           & 3            & 16.5            & 13.50             \\
APPLICATION, ALGORITHM                      & 22.45        & 22                                & 98                           & 25           & 2            & 5               & 6.53              \\
PROGRAMMING\_LANGUAGE                       & 22.42        & 2399                              & 10699                        & 25           & 1            & 2               & 2.35              \\
USER\_NAME, VALUE                           & 22.41        & 26                                & 116                          & 25           & 2            & 5               & 6.33              \\
ALGORITHM, VALUE                            & 22.22        & 14                                & 63                           & 25           & 2            & 6               & 9.44              \\
USER\_CLASS, OUTPUT\_BLOCK                  & 22.22        & 4                                 & 18                           & 25           & 6            & 20              & 18.89             \\
USER\_VARIABLE, FILE\_NAME                  & 22.17        & 49                                & 221                          & 25           & 2            & 7               & 8.37              \\
OPERATION\_SYSTEM                           & 22.16        & 119                               & 537                          & 25           & 1            & 3               & 4.25              \\
OPERATION\_SYSTEM, VALUE                    & 22.08        & 17                                & 77                           & 25           & 2            & 7               & 9.40              \\
FILE\_NAME, UI\_ELEMENT                     & 22.00        & 11                                & 50                           & 25           & 3            & 14.5            & 13.76             \\
DEVICE, LIBRARY                             & 21.97        & 29                                & 132                          & 25           & 3            & 6.5             & 8.77              \\
FILE\_NAME, IN\_LINE\_CODE                  & 21.90        & 30                                & 137                          & 25           & 3            & 7               & 9.20              \\
DEVICE, USER\_FUNCTION\_NAME                & 21.84        & 19                                & 87                           & 25           & 3            & 7               & 9.54              \\
ALGORITHM                                   & 21.76        & 99                                & 455                          & 25           & 1            & 4               & 4.43              \\
PROGRAMMING\_LANGUAGE, ALGORITHM            & 21.70        & 74                                & 341                          & 25           & 2            & 4               & 4.95              \\
USER\_VARIABLE, KEYBOARD\_INPUT             & 21.62        & 32                                & 148                          & 25           & 2            & 6               & 8.17              \\
DATA\_TYPE, USER\_FUNCTION\_NAME            & 21.56        & 36                                & 167                          & 25           & 2            & 6               & 8.20              \\
LIBRARY, USER\_VARIABLE                     & 21.56        & 108                               & 501                          & 25           & 2            & 6               & 6.56              \\
ALGORITHM, HTML\_TAG\_NAME                  & 21.43        & 3                                 & 14                           & 25           & 15           & 22.5            & 21.36             \\
FILE\_TYPE, KEYBOARD\_INPUT                 & 21.33        & 16                                & 75                           & 25           & 2            & 10              & 11.80             \\
OPERATION\_SYSTEM, USER\_VARIABLE           & 21.19        & 25                                & 118                          & 25           & 2            & 6               & 7.84              \\
APPLICATION, VALUE                          & 21.10        & 23                                & 109                          & 25           & 2            & 6               & 7.93              \\
APPLICATION, FILE\_TYPE                     & 21.05        & 36                                & 171                          & 25           & 2            & 5               & 6.65              \\
OPERATION\_SYSTEM, KEYBOARD\_INPUT          & 21.05        & 8                                 & 38                           & 25           & 3            & 14              & 14.03             \\
USER\_CLASS, WEBSITE                        & 21.05        & 4                                 & 19                           & 25           & 12           & 18              & 19.21             \\
PROGRAMMING\_LANGUAGE, USER\_VARIABLE       & 20.72        & 389                               & 1877                         & 25           & 2            & 4               & 4.48              \\
LIBRARY, USER\_FUNCTION\_NAME               & 20.70        & 53                                & 256                          & 25           & 3            & 6               & 7.71              \\
APPLICATION, IN\_LINE\_CODE                 & 20.63        & 13                                & 63                           & 25           & 3            & 8               & 9.84              \\
DEVICE, ERROR\_NAME                         & 20.55        & 15                                & 73                           & 25           & 3            & 8               & 10.05             \\
ALGORITHM, FILE\_TYPE                       & 20.51        & 8                                 & 39                           & 25           & 3            & 10              & 12.21             \\
OPERATION\_SYSTEM, UI\_ELEMENT              & 20.51        & 8                                 & 39                           & 25           & 2            & 16              & 12.95             \\
USER\_VARIABLE                              & 20.45        & 460                               & 2249                         & 25           & 1            & 4               & 4.26              \\
PROGRAMMING\_LANGUAGE, USER\_CLASS          & 20.37        & 11                                & 54                           & 25           & 2            & 6               & 9.78              \\
USER\_NAME, DATA\_TYPE                      & 20.29        & 14                                & 69                           & 25           & 2            & 5               & 7.84              \\
USER\_NAME, WEBSITE                         & 20.20        & 20                                & 99                           & 25           & 2            & 4               & 6.07              \\
PROGRAMMING\_LANGUAGE, DEVICE               & 20.09        & 85                                & 423                          & 25           & 2            & 4               & 5.33              \\
APPLICATION, KEYBOARD\_INPUT                & 20.00        & 8                                 & 40                           & 25           & 2            & 8               & 10.63             \\
ALGORITHM, IN\_LINE\_CODE                   & 20.00        & 8                                 & 40                           & 25           & 3            & 7.5             & 12.15             \\
USER\_NAME, OUTPUT\_BLOCK                   & 20.00        & 4                                 & 20                           & 25           & 3            & 12              & 13.90             \\
DATA\_STRUCTURE, USER\_CLASS                & 20.00        & 5                                 & 25                           & 25           & 4            & 17              & 15.24             \\
LIBRARY, USER\_CLASS                        & 20.00        & 5                                 & 25                           & 25           & 6            & 17              & 16.36             \\
LIBRARY\_CLASS, USER\_CLASS                 & 20.00        & 4                                 & 20                           & 25           & 10           & 19              & 19.10             \\
USER\_CLASS, USER\_VARIABLE                 & 20.00        & 9                                 & 45                           & 25           & 3            & 8               & 10.89             \\
USER\_CLASS, UI\_ELEMENT                    & 20.00        & 4                                 & 20                           & 25           & 7            & 19              & 18.75             \\
USER\_CLASS, HTML\_TAG\_NAME                & 20.00        & 3                                 & 15                           & 25           & 16           & 20              & 20.20             \\
APPLICATION, LIBRARY                        & 19.92        & 47                                & 236                          & 25           & 2            & 5               & 5.89              \\
DEVICE, FILE\_NAME                          & 19.74        & 15                                & 76                           & 25           & 3            & 9               & 11.49             \\
DEVICE, VALUE                               & 19.74        & 15                                & 76                           & 25           & 3            & 8               & 10.59             \\
ERROR\_NAME, IN\_LINE\_CODE                 & 19.59        & 19                                & 97                           & 25           & 2            & 7               & 9.02              \\
ERROR\_NAME, KEYBOARD\_INPUT                & 19.51        & 8                                 & 41                           & 25           & 4            & 10              & 12.85             \\
HTML\_TAG\_NAME, VALUE                      & 19.51        & 8                                 & 41                           & 25           & 2            & 16              & 14.12             \\
VERSION, WEBSITE                            & 19.44        & 7                                 & 36                           & 25           & 2            & 16              & 13.97             \\
DEVICE                                      & 19.44        & 97                                & 499                          & 25           & 1            & 4               & 5.03              \\
USER\_FUNCTION\_NAME, FILE\_TYPE            & 19.41        & 33                                & 170                          & 25           & 3            & 7               & 8.75              \\
USER\_NAME, FILE\_TYPE                      & 19.35        & 18                                & 93                           & 25           & 2            & 6               & 7.33              \\
LIBRARY\_VARIABLE, USER\_VARIABLE           & 19.23        & 5                                 & 26                           & 24           & 3            & 10              & 11.19             \\
DEVICE, USER\_VARIABLE                      & 19.20        & 24                                & 125                          & 25           & 2            & 7               & 8.70              \\
DEVICE, FILE\_TYPE                          & 19.15        & 18                                & 94                           & 25           & 2            & 8               & 10.31             \\
VERSION, HTML\_TAG\_NAME                    & 19.05        & 4                                 & 21                           & 25           & 3            & 20              & 19.05             \\
ALGORITHM, OUTPUT\_BLOCK                    & 19.05        & 4                                 & 21                           & 25           & 5            & 20              & 16.86             \\
DEVICE, IN\_LINE\_CODE                      & 19.05        & 12                                & 63                           & 25           & 3            & 10              & 12.13             \\
USER\_CLASS, KEYBOARD\_INPUT                & 19.05        & 4                                 & 21                           & 25           & 6            & 18              & 17.71             \\
VALUE, KEYBOARD\_INPUT                      & 18.99        & 15                                & 79                           & 25           & 2            & 8               & 11.42             \\
APPLICATION, DEVICE                         & 18.90        & 24                                & 127                          & 25           & 2            & 4               & 6.31              \\
USER\_NAME                                  & 18.88        & 304                               & 1610                         & 25           & 1            & 2               & 2.82              \\
APPLICATION                                 & 18.63        & 420                               & 2254                         & 25           & 1            & 2               & 2.88              \\
APPLICATION, PROGRAMMING\_LANGUAGE          & 18.60        & 297                               & 1597                         & 25           & 2            & 3               & 3.28              \\
USER\_CLASS                                 & 18.33        & 11                                & 60                           & 25           & 1            & 6               & 9.70              \\
USER\_FUNCTION\_NAME, IN\_LINE\_CODE        & 18.30        & 28                                & 153                          & 25           & 3            & 7               & 8.58              \\
USER\_VARIABLE, FILE\_TYPE                  & 17.97        & 62                                & 345                          & 25           & 2            & 6               & 7.02              \\
ALGORITHM, LIBRARY\_FUNCTION                & 17.95        & 7                                 & 39                           & 25           & 3            & 7               & 9.74              \\
USER\_NAME, FILE\_NAME                      & 17.95        & 14                                & 78                           & 25           & 2            & 5               & 7.29              \\
ERROR\_NAME, OUTPUT\_BLOCK                  & 17.86        & 5                                 & 28                           & 25           & 7            & 18.5            & 16.68             \\
LIBRARY, UI\_ELEMENT                        & 17.81        & 13                                & 73                           & 25           & 3            & 10              & 11.60             \\
USER\_FUNCTION\_NAME, VALUE                 & 17.78        & 40                                & 225                          & 25           & 2            & 6               & 7.69              \\
VERSION, USER\_CLASS                        & 17.65        & 3                                 & 17                           & 25           & 10           & 20              & 19.35             \\
ALGORITHM, LIBRARY\_CLASS                   & 17.39        & 4                                 & 23                           & 25           & 5            & 20              & 17.70             \\
OPERATION\_SYSTEM, USER\_FUNCTION\_NAME     & 17.39        & 12                                & 69                           & 25           & 2            & 6               & 9.38              \\
UI\_ELEMENT, VALUE                          & 17.33        & 13                                & 75                           & 25           & 2            & 10              & 11.69             \\
USER\_NAME, LIBRARY                         & 17.27        & 24                                & 139                          & 25           & 2            & 5               & 6.32              \\
WEBSITE, VALUE                              & 17.24        & 10                                & 58                           & 25           & 2            & 8               & 11.00             \\
USER\_NAME, UI\_ELEMENT                     & 17.14        & 12                                & 70                           & 25           & 2            & 4               & 7.13              \\
LIBRARY\_FUNCTION, KEYBOARD\_INPUT          & 17.14        & 12                                & 70                           & 25           & 4            & 8               & 10.09             \\
USER\_NAME, USER\_VARIABLE                  & 16.81        & 40                                & 238                          & 25           & 2            & 4               & 5.26              \\
USER\_NAME, USER\_CLASS                     & 16.67        & 2                                 & 12                           & 25           & 3            & 18              & 14.50             \\
IN\_LINE\_CODE, KEYBOARD\_INPUT             & 16.67        & 15                                & 90                           & 25           & 2            & 8               & 10.60             \\
PROGRAMMING\_LANGUAGE, USER\_NAME           & 16.40        & 165                               & 1006                         & 25           & 2            & 3               & 3.48              \\
APPLICATION, OPERATION\_SYSTEM              & 16.38        & 19                                & 116                          & 25           & 2            & 4               & 5.66              \\
USER\_FUNCTION\_NAME, KEYBOARD\_INPUT       & 16.30        & 15                                & 92                           & 25           & 3            & 7               & 9.68              \\
APPLICATION, UI\_ELEMENT                    & 16.22        & 12                                & 74                           & 25           & 2            & 5               & 7.59              \\
PROGRAMMING\_LANGUAGE, WEBSITE              & 16.12        & 54                                & 335                          & 25           & 2            & 3               & 4.82              \\
ALGORITHM, USER\_NAME                       & 16.07        & 9                                 & 56                           & 25           & 2            & 5               & 7.36              \\
ALGORITHM, UI\_ELEMENT                      & 16.00        & 4                                 & 25                           & 25           & 3            & 19              & 15.36             \\
PROGRAMMING\_LANGUAGE, USER\_FUNCTION\_NAME & 15.86        & 137                               & 864                          & 25           & 2            & 5               & 5.37              \\
USER\_FUNCTION\_NAME                        & 15.83        & 158                               & 998                          & 25           & 1            & 5               & 5.21              \\
USER\_VARIABLE, USER\_FUNCTION\_NAME        & 15.80        & 119                               & 753                          & 25           & 2            & 5               & 5.57              \\
WEBSITE                                     & 15.63        & 65                                & 416                          & 25           & 1            & 3               & 4.39              \\
APPLICATION, OUTPUT\_BLOCK                  & 15.38        & 4                                 & 26                           & 25           & 3            & 12              & 13.27             \\
ERROR\_NAME, USER\_CLASS                    & 15.38        & 2                                 & 13                           & 25           & 5            & 21              & 19.31             \\
LIBRARY, WEBSITE                            & 15.38        & 12                                & 78                           & 25           & 2            & 6               & 9.65              \\
FILE\_TYPE, UI\_ELEMENT                     & 15.38        & 12                                & 78                           & 25           & 3            & 8               & 11.00             \\
APPLICATION, FILE\_NAME                     & 15.27        & 20                                & 131                          & 25           & 2            & 5               & 6.98              \\
PROGRAMMING\_LANGUAGE, UI\_ELEMENT          & 14.47        & 33                                & 228                          & 25           & 2            & 4               & 6.42              \\
APPLICATION, WEBSITE                        & 14.44        & 13                                & 90                           & 25           & 2            & 4               & 6.54              \\
USER\_CLASS, FILE\_NAME                     & 14.29        & 3                                 & 21                           & 25           & 8            & 18              & 18.43             \\
USER\_FUNCTION\_NAME, WEBSITE               & 14.29        & 7                                 & 49                           & 25           & 3            & 8               & 11.53             \\
UI\_ELEMENT                                 & 13.99        & 41                                & 293                          & 25           & 1            & 4               & 5.84              \\
APPLICATION, USER\_NAME                     & 13.85        & 41                                & 296                          & 25           & 2            & 3               & 4.21              \\
USER\_VARIABLE, WEBSITE                     & 13.75        & 11                                & 80                           & 25           & 3            & 6               & 9.16              \\
APPLICATION, ERROR\_NAME                    & 13.58        & 11                                & 81                           & 25           & 2            & 5               & 7.17              \\
USER\_NAME, USER\_FUNCTION\_NAME            & 13.33        & 22                                & 165                          & 25           & 2            & 4               & 5.50              \\
USER\_NAME, LIBRARY\_CLASS                  & 13.04        & 3                                 & 23                           & 25           & 3            & 11              & 14.39             \\
FILE\_TYPE, WEBSITE                         & 13.04        & 9                                 & 69                           & 25           & 2            & 7               & 10.10             \\
ALGORITHM, USER\_VARIABLE                   & 12.84        & 19                                & 148                          & 25           & 2            & 5               & 6.88              \\
APPLICATION, USER\_VARIABLE                 & 12.58        & 38                                & 302                          & 25           & 2            & 5               & 5.69              \\
APPLICATION, USER\_CLASS                    & 12.50        & 2                                 & 16                           & 25           & 4            & 14.5            & 14.31             \\
USER\_FUNCTION\_NAME, UI\_ELEMENT           & 12.00        & 9                                 & 75                           & 25           & 3            & 7               & 10.23             \\
ALGORITHM, USER\_FUNCTION\_NAME             & 11.90        & 10                                & 84                           & 25           & 2            & 6               & 8.55              \\
USER\_CLASS, USER\_FUNCTION\_NAME           & 11.43        & 4                                 & 35                           & 25           & 3            & 12              & 12.46             \\
USER\_CLASS, FILE\_TYPE                     & 11.11        & 3                                 & 27                           & 25           & 4            & 17              & 15.48             \\
APPLICATION, HTML\_TAG\_NAME                & 10.53        & 2                                 & 19                           & 25           & 2            & 17              & 15.68             \\
ALGORITHM, KEYBOARD\_INPUT                  & 10.53        & 4                                 & 38                           & 25           & 2            & 9               & 12.61             \\
USER\_CLASS, VALUE                          & 10.53        & 2                                 & 19                           & 25           & 7            & 20              & 18.26             \\
FILE\_NAME, WEBSITE                         & 10.00        & 9                                 & 90                           & 25           & 2            & 6               & 9.00              \\
APPLICATION, USER\_FUNCTION\_NAME           & 9.09         & 14                                & 154                          & 25           & 2            & 6               & 6.89              \\
USER\_VARIABLE, UI\_ELEMENT                 & 8.87         & 11                                & 124                          & 25           & 2            & 5               & 8.08              \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                   \\
                                            &              &                                   &                              &              &              &                 &                  
\end{tabular}
\end{table}

==> tablets/intent_REVIEW_upto2_combinations_success_rate.tex <==
\begin{table}
\centering
\caption{Entity Combinations in REVIEW intent}
\label{tab:intent_REVIEW_upto2_combinations_success_rate}
\setlength{\tabcolsep}{2pt} 

\begin{tabular}{llllllll}
Entities Combination                        & Success Rate & Number of Successful Combinations & Total Number of Combinations & Max Entities & Min Entities & Median Entities & Average Entities  \\
LIBRARY\_FUNCTION                           & 70.00        & 7                                 & 10                           & 13           & 3            & 5               & 6.10              \\
LIBRARY                                     & 53.85        & 7                                 & 13                           & 13           & 2            & 5               & 5.69              \\
PROGRAMMING\_LANGUAGE, LIBRARY              & 53.85        & 7                                 & 13                           & 13           & 2            & 5               & 5.69              \\
USER\_VARIABLE, USER\_FUNCTION\_NAME        & 50.00        & 5                                 & 10                           & 13           & 4            & 5               & 6.10              \\
PROGRAMMING\_LANGUAGE, USER\_FUNCTION\_NAME & 46.15        & 6                                 & 13                           & 13           & 2            & 5               & 5.54              \\
USER\_FUNCTION\_NAME                        & 43.75        & 7                                 & 16                           & 13           & 1            & 4               & 4.88              \\
PROGRAMMING\_LANGUAGE, FILE\_TYPE           & 41.67        & 5                                 & 12                           & 13           & 3            & 4               & 5.08              \\
PROGRAMMING\_LANGUAGE, USER\_VARIABLE       & 39.13        & 9                                 & 23                           & 13           & 2            & 4               & 4.57              \\
USER\_VARIABLE                              & 38.46        & 10                                & 26                           & 13           & 2            & 4               & 4.46              \\
FILE\_TYPE                                  & 35.71        & 5                                 & 14                           & 13           & 3            & 4               & 4.79              \\
PROGRAMMING\_LANGUAGE, FILE\_NAME           & 22.22        & 4                                 & 18                           & 13           & 2            & 4               & 4.50              \\
PROGRAMMING\_LANGUAGE                       & 21.98        & 20                                & 91                           & 13           & 1            & 2               & 2.82              \\
FILE\_NAME                                  & 21.05        & 4                                 & 19                           & 13           & 2            & 4               & 4.42              \\
APPLICATION                                 & 16.67        & 4                                 & 24                           & 9            & 1            & 2.5             & 3.08              \\
WEBSITE                                     & 15.38        & 2                                 & 13                           & 7            & 2            & 4               & 3.77              \\
APPLICATION, PROGRAMMING\_LANGUAGE          & 15.38        & 2                                 & 13                           & 9            & 2            & 3               & 3.85              \\
PROGRAMMING\_LANGUAGE, WEBSITE              & 10.00        & 1                                 & 10                           & 7            & 2            & 4               & 4.10              \\
USER\_NAME                                  & 0.00         & 0                                 & 15                           & 5            & 1            & 3               & 2.87              \\
PROGRAMMING\_LANGUAGE, USER\_NAME           & 0.00         & 0                                 & 10                           & 5            & 2            & 3.5             & 3.30             
\end{tabular}
\end{table}

==> tablets/overall_intent_entity_best-worst_3.tex <==
\begin{table*}[!th]
\centering
\caption{Entity Pair Results (Top 3 and Bottom 3 by \% Success).}
\label{tab:overall_intent_entity_combinations_success_rate}
\scriptsize
\begin{tabular}{lllrrr}
\toprule
Intent & \multicolumn{2}{l}{Entity Pair (Ranked by \% Success)} & \% Success & \# Success & \# Total \\ \midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Aggregate \\ Results\\ (All Intents)\end{tabular}} & \multirow{3}{*}{Top 3} & \entity{Device, Library Variable} & 45.5 & 5 & 11 \\
 &  & \entity{Version, Library Variable} & 41.7 & 5 & 12 \\
 &  & \entity{Data Type, Library Variable} & 36.4 & 8 & 22 \\ \cmidrule(l){2-6} 
 & \multirow{3}{*}{Bottom 3} & \entity{Application, User Class} & 10.0 & 2 & 20 \\
 &  & \entity{User Variable, UI Element} & 8.4 & 13 & 154 \\
 &  & \entity{User Class, Value} & 6.9 & 2 & 29 \\ \midrule
\multicolumn{6}{l}{\textit{The following rows present entity pair results broken down by intent.}} \\ \midrule
\multirow{6}{*}{\intent{API Usage}} & \multirow{3}{*}{Top 3} & \entity{Application, File Type} & 53.3 & 8 & 15 \\
 &  & \entity{Operation System, User Variable} & 45.8 & 11 & 24 \\
 &  & \entity{Data Structure, Library Function} & 45.1 & 23 & 51 \\ \cmidrule(l){2-6} 
 & \multirow{3}{*}{Bottom 3} & \entity{Value, Keyboard Input} & 5.6 & 1 & 18 \\
 &  & \entity{User Function Name, Keyboard Input} & 5.0 & 1 & 20 \\
 &  & \entity{Value, Output Block} & 0.0 & 0 & 10 \\ \midrule
\multirow{6}{*}{\intent{Conceptual}} & \multirow{3}{*}{Top 3} & \entity{Data Structure, Library Variable} & 42.1 & 8 & 19 \\
 &  & \entity{User Name, HTML/XML Tag Name} & 41.7 & 5 & 12 \\
 &  & \entity{Version, Library Variable} & 41.7 & 5 & 12 \\ \cmidrule(l){2-6} 
 & \multirow{3}{*}{Bottom 3} & \entity{User Function Name, Website} & 6.9 & 2 & 29 \\
 &  & \entity{Algorithm, UI Element} & 6.3 & 1 & 16 \\
 &  & \entity{User Variable, Website} & 5.6 & 2 & 36 \\ \midrule
\multirow{6}{*}{\intent{Discrepancy}} & \multirow{3}{*}{Top 3} & \entity{User Variable, Library Function} & 39.1 & 45 & 115 \\
 &  & \entity{Library Class, Library Function} & 38.7 & 12 & 31 \\
 &  & \entity{Application, File Type} & 38.5 & 10 & 26 \\ \cmidrule(l){2-6} 
 & \multirow{3}{*}{Bottom 3} & \entity{Data Type, Keyboard Input} & 0.0 & 0 & 10 \\
 &  & \entity{File Name, UI Element} & 0.0 & 0 & 11 \\
 &  & \entity{User Function Name, Keyboard Input} & 0.0 & 0 & 21 \\ \midrule
\multirow{6}{*}{\intent{Errors}} & \multirow{3}{*}{Top 3} & \entity{Programming Language, Library Function} & 63.6 & 7 & 11 \\
 &  & \entity{Programming Language, File Name} & 41.2 & 7 & 17 \\
 &  & \entity{Programming Language, File Type} & 33.3 & 4 & 12 \\ \cmidrule(l){2-6} 
 & \multirow{3}{*}{Bottom 3} & \entity{Programming Language, Error Name} & 27.3 & 3 & 11 \\
 &  & \entity{Programming Language, Version} & 14.3 & 2 & 14 \\
 &  & \entity{Programming Language, User Name} & 0.0 & 0 & 10 \\ \midrule
\multirow{6}{*}{\intent{Learning}} & \multirow{3}{*}{Top 3} & \entity{Programming Language, Library} & 53.9 & 7 & 13 \\
 &  & \entity{User Variable, User Function Name} & 50.0 & 5 & 10 \\
 &  & \entity{Programming Language, User Function Name} & 46.2 & 6 & 13 \\ \cmidrule(l){2-6} 
 & \multirow{3}{*}{Bottom 3} & \entity{Programming Language, Application} & 15.4 & 2 & 13 \\
 &  & \entity{Programming Language, Website} & 10.0 & 1 & 10 \\
 &  & \entity{Programming Language, User Name} & 0.0 & 0 & 10 \\ \midrule
\multirow{6}{*}{\intent{Review}} & \multirow{3}{*}{Top 3} & \entity{Device, Library Variable} & 40.0 & 4 & 10 \\
 &  & \entity{Version, Data Structure} & 37.5 & 24 & 64 \\
 &  & \entity{UI Element, HTML/XML Tag Name} & 36.8 & 14 & 38 \\ \cmidrule(l){2-6} 
 & \multirow{3}{*}{Bottom 3} & \entity{File Name, Website} & 10.0 & 9 & 90 \\
 &  & \entity{Application, User Function Name} & 9.1 & 14 & 154 \\
 &  & \entity{User Variable, UI Element} & 8.9 & 11 & 124 \\ \midrule
\multirow{6}{*}{\intent{API Change}} & \multirow{3}{*}{Top 3} & \entity{Data Structure, Output Block} & 75.0 & 9 & 12 \\
 &  & \entity{Algorithm, Error Name} & 66.7 & 8 & 12 \\
 &  & \entity{Data Type, UI Element} & 63.6 & 7 & 11 \\ \cmidrule(l){2-6} 
 & \multirow{3}{*}{Bottom 3} & \entity{File Type, Keyboard Input} & 17.7 & 6 & 34 \\
 &  & \entity{Library, Website} & 17.1 & 6 & 35 \\
 &  & \entity{Application, User Function Name} & 17.0 & 10 & 59 \\ \bottomrule
\end{tabular}
\vspace*{-1em}
\end{table*}



==> tablets/overall_intent_entity_best-worst_3_subtable.tex <==

\begin{table*}[!th]
\centering
\caption{Entity Pair Results (Top 3 and Bottom 3 by \% Success).}
\label{tab:entity_pair_results}
% Requires the subcaption package
\begin{subtable}[t]{0.47\textwidth}
  \centering
  \caption{Aggregate Results (All Intents)}
  \begin{tabular}{p{5.5cm}rr}
    \toprule
    Entity Pair & \% Success & \# Total \\
    \midrule
    \entity{Device, Library Variable} & 45.5 & 11 \\
    \entity{Version, Library Variable}  & 41.7 & 12 \\
    \entity{Data Type, Library Variable} & 36.4 & 22 \\
    \midrule
    \entity{Application, User Class}     & 10.0 & 20 \\
    \entity{User Variable, UI Element}    & 8.4  & 154 \\
    \entity{User Class, Value}            & 6.9  & 29 \\
    \bottomrule
  \end{tabular}
\end{subtable}
\hspace{0.5cm}
\begin{subtable}[t]{0.47\textwidth}
  \centering
  \caption{API Usage}
  \begin{tabular}{p{5.5cm}rr}
    \toprule
    Entity Pair & \% Success & \# Total \\
    \midrule
    \entity{Application, File Type}          & 53.3 & 15 \\
    \entity{Operation System, User Variable} & 45.8 & 24 \\
    \entity{Data Structure, Library Function}& 45.1 & 51 \\
    \midrule
    \entity{Value, Keyboard Input}            & 5.6  & 18 \\
    \entity{User Func Name, Keyboard Input}& 5.0 & 20 \\
    \entity{Value, Output Block}               & 0.0  & 10 \\
    \bottomrule
  \end{tabular}
\end{subtable}

\vspace{0.5em}

\begin{subtable}[t]{0.47\textwidth}
  \centering
  \caption{Conceptual}
  \begin{tabular}{p{5.5cm}rr}
    \toprule
    Entity Pair & \% Success & \# Total \\
    \midrule
    \entity{Data Structure, Library Variable}  & 42.1 & 19 \\
    \entity{User Name, HTML/XML Tag Name}        & 41.7 & 12 \\
    \entity{Version, Library Variable}           & 41.7 & 12 \\
    \midrule
    \entity{User Func Name, Website}         & 6.9  & 29 \\
    \entity{Algorithm, UI Element}               & 6.3  & 16 \\
    \entity{User Variable, Website}              & 5.6  & 36 \\
    \bottomrule
  \end{tabular}
\end{subtable}
\hspace{0.5cm}
\begin{subtable}[t]{0.47\textwidth}
  \centering
  \caption{Discrepancy}
  \begin{tabular}{p{5.5cm}rr}
    \toprule
    Entity Pair & \% Success & \# Total \\
    \midrule
    \entity{User Variable, Library Function}  & 39.1 & 115 \\
    \entity{Library Class, Library Function}    & 38.7 & 31 \\
    \entity{Application, File Type}               & 38.5 & 26 \\
    \midrule
    \entity{Data Type, Keyboard Input}            & 0.0  & 10 \\
    \entity{File Name, UI Element}                & 0.0  & 11 \\
    \entity{User Func Name, Keyboard Input}   & 0.0  & 21 \\
    \bottomrule
  \end{tabular}
\end{subtable}

\vspace{0.5em}

\begin{subtable}[t]{0.47\textwidth}
  \centering
  \caption{Errors}
  \begin{tabular}{p{5.5cm}rr}
    \toprule
    Entity Pair & \% Success & \# Total \\
    \midrule
    \entity{Prog Lang, Library Function} & 63.6 & 11 \\
    \entity{Prog Lang, File Name}        & 41.2 & 17 \\
    \entity{Prog Lang, File Type}        & 33.3 & 12 \\
    \midrule
    \entity{Prog Lang, Error Name}       & 27.3 & 11 \\
    \entity{Prog Lang, Version}          & 14.3 & 14 \\
    \entity{Prog Lang, User Name}        & 0.0  & 10 \\
    \bottomrule
  \end{tabular}
\end{subtable}
\hspace{0.5cm}
\begin{subtable}[t]{0.47\textwidth}
  \centering
  \caption{Learning}
  \begin{tabular}{p{5.5cm}rr}
    \toprule
    Entity Pair & \% Success & \# Total \\
    \midrule
    \entity{Prog Lang, Library}         & 53.9 & 13 \\
    \entity{User Variable, User Func Name}       & 50.0 & 10 \\
    \entity{Prog Lang, User Func Name}& 46.2 & 13 \\
    \midrule
    \entity{Prog Lang, Application}      & 15.4 & 13 \\
    \entity{Prog Lang, Website}          & 10.0 & 10 \\
    \entity{Prog Lang, User Name}        & 0.0  & 10 \\
    \bottomrule
  \end{tabular}
\end{subtable}

\vspace{0.5em}

\begin{subtable}[t]{0.47\textwidth}
  \centering
  \caption{Review}
  \begin{tabular}{p{5.5cm}rr}
    \toprule
    Entity Pair & \% Success & \# Total \\
    \midrule
    \entity{Device, Library Variable}     & 40.0 & 10 \\
    \entity{Version, Data Structure}        & 37.5 & 64 \\
    \entity{UI Element, HTML/XML Tag Name}  & 36.8 & 38 \\
    \midrule
    \entity{File Name, Website}             & 10.0 & 90 \\
    \entity{Application, User Func Name}& 9.1  & 154 \\
    \entity{User Variable, UI Element}       & 8.9  & 124 \\
    \bottomrule
  \end{tabular}
\end{subtable}
\hspace{0.5cm}
\begin{subtable}[t]{0.47\textwidth}
  \centering
  \caption{API Change}
  \begin{tabular}{p{5.5cm}rr}
    \toprule
    Entity Pair & \% Success & \# Total \\
    \midrule
    \entity{Data Structure, Output Block} & 75.0 & 12 \\
    \entity{Algorithm, Error Name}        & 66.7 & 12 \\
    \entity{Data Type, UI Element}          & 63.6 & 11 \\
    \midrule
    \entity{File Type, Keyboard Input}      & 17.7 & 34 \\
    \entity{Library, Website}               & 17.1 & 35 \\
    \entity{Application, User Func Name}& 17.0 & 59 \\
    \bottomrule
  \end{tabular}
\end{subtable}
\end{table*}

==> tablets/overall_upto2_best_combinations_success_rate.tex <==
\begin{table}
\centering
\caption{Best Entity Combinations Overall}
\label{tab:overall_upto2_best_combinations_success_rate}



\begin{tabular}{llllllll}
Entities Combination                     & Success Rate & Number of Successful Combinations & Total Number of Combinations & Max Entities & Min Entities & Median Entities & Average Entities  \\
DEVICE, LIBRARY\_VARIABLE                & 45.45        & 5                                 & 11                           & 24           & 4            & 15              & 14.82             \\
VERSION, LIBRARY\_VARIABLE               & 41.67        & 5                                 & 12                           & 24           & 3            & 15              & 14.17             \\
ERROR\_NAME, LIBRARY\_VARIABLE           & 36.36        & 4                                 & 11                           & 24           & 5            & 11              & 13.00             \\
DATA\_TYPE, LIBRARY\_VARIABLE            & 36.36        & 8                                 & 22                           & 24           & 2            & 9               & 11.73             \\
LIBRARY\_VARIABLE, KEYBOARD\_INPUT       & 36.36        & 4                                 & 11                           & 24           & 11           & 18              & 17.27             \\
DATA\_STRUCTURE, LIBRARY\_VARIABLE       & 36.00        & 9                                 & 25                           & 24           & 4            & 9               & 11.44             \\
LIBRARY\_VARIABLE, FILE\_TYPE            & 34.78        & 8                                 & 23                           & 24           & 6            & 9               & 11.70             \\
PROGRAMMING\_LANGUAGE, DATA\_STRUCTURE   & 33.55        & 416                               & 1240                         & 25           & 2            & 4               & 4.97              \\
USER\_NAME, DATA\_STRUCTURE              & 33.33        & 40                                & 120                          & 25           & 2            & 5               & 7.52              \\
LIBRARY, LIBRARY\_VARIABLE               & 33.33        & 13                                & 39                           & 24           & 3            & 8               & 10.15             \\
LIBRARY\_VARIABLE, OUTPUT\_BLOCK         & 33.33        & 4                                 & 12                           & 22           & 6            & 15.5            & 15.08             \\
LIBRARY\_FUNCTION, HTML\_TAG\_NAME       & 33.33        & 10                                & 30                           & 25           & 4            & 16              & 15.37             \\
UI\_ELEMENT, HTML\_TAG\_NAME             & 33.33        & 15                                & 45                           & 25           & 3            & 17              & 15.84             \\
VERSION, DATA\_STRUCTURE                 & 33.00        & 33                                & 100                          & 25           & 3            & 8               & 10.96             \\
USER\_NAME, LIBRARY\_FUNCTION            & 32.84        & 22                                & 67                           & 25           & 3            & 7               & 8.54              \\
DATA\_TYPE, LIBRARY\_FUNCTION            & 32.16        & 91                                & 283                          & 25           & 3            & 7               & 7.60              \\
VERSION, FILE\_NAME                      & 31.82        & 42                                & 132                          & 25           & 2            & 8               & 9.92              \\
LIBRARY\_VARIABLE, FILE\_NAME            & 31.58        & 6                                 & 19                           & 24           & 6            & 11              & 12.53             \\
PROGRAMMING\_LANGUAGE, LIBRARY\_CLASS    & 31.13        & 99                                & 318                          & 25           & 2            & 6.5             & 7.85              \\
LIBRARY\_CLASS, LIBRARY\_FUNCTION        & 31.06        & 50                                & 161                          & 25           & 2            & 8               & 8.82              \\
OPERATION\_SYSTEM, LIBRARY\_FUNCTION     & 30.77        & 28                                & 91                           & 25           & 2            & 6               & 8.31              \\
DEVICE, LIBRARY\_FUNCTION                & 30.59        & 26                                & 85                           & 25           & 3            & 8               & 9.82              \\
DATA\_STRUCTURE, LIBRARY\_FUNCTION       & 30.48        & 96                                & 315                          & 25           & 2            & 7               & 7.48              \\
VERSION, LIBRARY                         & 30.41        & 66                                & 217                          & 25           & 2            & 7               & 8.21              \\
DATA\_STRUCTURE, FILE\_NAME              & 30.07        & 46                                & 153                          & 25           & 2            & 8               & 9.84              \\
PROGRAMMING\_LANGUAGE, LIBRARY\_VARIABLE & 30.00        & 15                                & 50                           & 24           & 2            & 8               & 9.34              \\
ERROR\_NAME, DATA\_STRUCTURE             & 30.00        & 39                                & 130                          & 25           & 3            & 7               & 9.51             
\end{tabular}
\end{table}

==> tablets/overall_upto2_worst_combinations_success_rate.tex <==
\begin{table}
\centering
\caption{Worst Entity Combinations Overall}
\label{tab:overall_upto2_worst_combinations_success_rate}


\begin{tabular}{llllllll}
Entities Combination                        & Success Rate & Number of Successful Combinations & Total Number of Combinations & Max Entities & Min Entities & Median Entities & Average Entities  \\
APPLICATION, PROGRAMMING\_LANGUAGE          & 19.07        & 359                               & 1883                         & 25           & 2            & 3               & 3.43              \\
PROGRAMMING\_LANGUAGE, USER\_NAME           & 17.64        & 217                               & 1230                         & 25           & 2            & 3               & 3.59              \\
PROGRAMMING\_LANGUAGE, USER\_FUNCTION\_NAME & 16.44        & 203                               & 1235                         & 25           & 2            & 5               & 5.45              \\
USER\_VARIABLE, USER\_FUNCTION\_NAME        & 15.26        & 166                               & 1088                         & 25           & 2            & 5               & 5.64              \\
APPLICATION, OPERATION\_SYSTEM              & 14.81        & 24                                & 162                          & 25           & 2            & 4               & 5.57              \\
IN\_LINE\_CODE, KEYBOARD\_INPUT             & 14.69        & 21                                & 143                          & 25           & 2            & 7               & 9.72              \\
USER\_NAME, UI\_ELEMENT                     & 14.61        & 13                                & 89                           & 25           & 2            & 4               & 7.52              \\
USER\_NAME, USER\_FUNCTION\_NAME            & 14.22        & 31                                & 218                          & 25           & 2            & 5               & 5.79              \\
LIBRARY, WEBSITE                            & 14.14        & 14                                & 99                           & 25           & 2            & 6               & 9.82              \\
PROGRAMMING\_LANGUAGE, UI\_ELEMENT          & 13.89        & 40                                & 288                          & 25           & 2            & 4               & 6.40              \\
USER\_FUNCTION\_NAME, KEYBOARD\_INPUT       & 13.64        & 18                                & 132                          & 25           & 3            & 7               & 9.48              \\
UI\_ELEMENT, VALUE                          & 13.54        & 13                                & 96                           & 25           & 2            & 9               & 11.51             \\
USER\_CLASS, USER\_FUNCTION\_NAME           & 13.46        & 7                                 & 52                           & 25           & 3            & 9               & 11.90             \\
FILE\_TYPE, UI\_ELEMENT                     & 13.40        & 13                                & 97                           & 25           & 3            & 9               & 11.30             \\
APPLICATION, USER\_FUNCTION\_NAME           & 13.04        & 27                                & 207                          & 25           & 2            & 5               & 6.90              \\
ERROR\_NAME, OUTPUT\_BLOCK                  & 12.96        & 7                                 & 54                           & 25           & 3            & 12              & 13.72             \\
FILE\_TYPE, WEBSITE                         & 12.94        & 11                                & 85                           & 25           & 2            & 7               & 10.61             \\
ALGORITHM, USER\_VARIABLE                   & 12.56        & 27                                & 215                          & 25           & 2            & 5               & 6.91              \\
ALGORITHM, UI\_ELEMENT                      & 12.50        & 4                                 & 32                           & 25           & 3            & 20              & 15.97             \\
USER\_NAME, USER\_CLASS                     & 12.50        & 2                                 & 16                           & 25           & 3            & 20              & 15.69             \\
USER\_FUNCTION\_NAME, WEBSITE               & 12.31        & 8                                 & 65                           & 25           & 3            & 8               & 11.69             \\
USER\_VARIABLE, WEBSITE                     & 12.12        & 12                                & 99                           & 25           & 3            & 6               & 9.55              \\
ALGORITHM, USER\_FUNCTION\_NAME             & 12.07        & 14                                & 116                          & 25           & 2            & 6.5             & 8.83              \\
APPLICATION, HTML\_TAG\_NAME                & 12.00        & 3                                 & 25                           & 25           & 2            & 17              & 16.28             \\
ALGORITHM, KEYBOARD\_INPUT                  & 11.11        & 6                                 & 54                           & 25           & 2            & 9               & 12.50             \\
USER\_CLASS, FILE\_NAME                     & 11.11        & 3                                 & 27                           & 25           & 5            & 18              & 18.26             \\
USER\_FUNCTION\_NAME, UI\_ELEMENT           & 10.99        & 10                                & 91                           & 25           & 3            & 7               & 10.43             \\
FILE\_NAME, WEBSITE                         & 10.91        & 12                                & 110                          & 25           & 2            & 6               & 9.34              \\
USER\_CLASS, FILE\_TYPE                     & 10.81        & 4                                 & 37                           & 25           & 3            & 17              & 15.05             \\
APPLICATION, USER\_CLASS                    & 10.00        & 2                                 & 20                           & 25           & 3            & 16              & 15.20             \\
USER\_VARIABLE, UI\_ELEMENT                 & 8.44         & 13                                & 154                          & 25           & 2            & 5               & 8.21              \\
USER\_CLASS, VALUE                          & 6.90         & 2                                 & 29                           & 25           & 5            & 17              & 16.00            
\end{tabular}
\end{table}

==> tablets/performance_comparison.tex <==
\begin{table}[htbp]
\centering
\caption{Performance metrics comparison between the mixed-effect model with and without \ourmethod features, before and after stepwise}

\label{tab:performance_comparison}
\begin{tabular}{lrrr}
\toprule
\textbf{Metric} & \textbf{Baseline with standard features} & \textbf{ \ourmethod with 52 features } & \textbf{ \ourmethod with 26 features} \\ \midrule
AUC            & 0.75                  & \textbf{0.76} (1\% $\uparrow$)                       & \textbf{0.78} (3\% $\uparrow$)               \\
PR-AUC         & 0.43                  & \textbf{0.51} (8\% $\uparrow$)                       & \textbf{0.46} (3\% $\uparrow$)               \\
MCC            & 0.07                  & \textbf{0.25} (18\% $\uparrow$)                       & \textbf{0.21} (15\% $\uparrow$)               \\ \bottomrule
\end{tabular}
\end{table}


==> tablets/performance_comparison_after_stepwise.tex <==
\begin{table}[htbp]
\centering
\caption{Performance metrics comparison between the mixed-effect model with and without\ourmethod features after stepwise.}
\label{tab:performance_comparison_stepwise}
\begin{tabular}{lrrr}
\toprule
\textbf{Metric} & \textbf{Without \ourmethod} & \textbf{With \ourmethod} & \textbf{Improvement} \\ \midrule
AUC            & 0.75                  & \textbf{0.78}                       & 3\% $\uparrow$               \\
PR-AUC         & 0.43                  & \textbf{0.46}                       & 3\% $\uparrow$               \\
MCC            & 0.06                  & \textbf{0.21}                       & 15\% $\uparrow$               \\ \bottomrule
\end{tabular}
\end{table}

